Deep Reinforcement Learning-Aided Random Access

We consider a system model comprised of an access point (AP) and K Internet of Things (IoT) nodes that sporadically become active in order to send data to the AP. The AP is assumed to have N time-frequency resource blocks that it can allocate to the IoT nodes that wish to send data, where N < K. The main problem is how to allocate the N time-frequency resource blocks to the IoT nodes in each time slot such that the average packet rate is maximized. For this problem, we propose a deep reinforcement learning (DRL)-aided random access (RA) scheme, where an intelligent DRL agent at the AP learns to predict the activity of the IoT nodes in each time slot and grants time-frequency resource blocks to the IoT nodes predicted as active. Next, the IoT nodes that are missclassified as non-active by the DRL agent, as well as unseen or newly arrived nodes in the cell, employ the standard RA scheme in order to obtain time-frequency resource blocks. We leverage expert knowledge for faster training of the DRL agent. Our numerical results show significant improvements in terms of average packet rate when the proposed DRL-aided RA scheme is implemented compared to the existing solution used in practice, the standard RA scheme.

==> litdab.tex <==
@STRING{com = {IEEE Trans. Commun.} }
@STRING{cma = {IEEE Commun. Magazine} }
@STRING{inf = {IEEE Trans. Inf. Theory} }
@STRING{veh = {IEEE Trans. Veh. Technol.} }
@STRING{sel = {IEEE J. Select. Areas Commun.} }
@STRING{sip = {IEEE Trans. Signal Proces.} }
@STRING{siplett = {IEEE Signal Processing Letters} }
@STRING{ac  = {IEEE Trans. on Automatic Control} }
@STRING{neu = {IEEE Trans. on Neural Networks} }
@STRING{csi = {IEEE Trans. on Circuits and Systems I: Fundamental Theory
          and Applications} }
@STRING{ple = {Plenum Press} }
@STRING{bel = {Bell System Technical Journal} }
@STRING{pre = {Prentice--Hall, Inc.} }
@STRING{old = {Oldenbourg Verlag} }
@STRING{spr = {Springer Verlag} }
@STRING{teu = {B.G. Teubner} }
@STRING{wil = {John Wiley \& Sons, Inc.} }
@STRING{ntz = {Nachrichtentechnische Zeitschrift (ntz)} }
@STRING{wc = {IEEE Trans. Wireless Commun.}}


@INPROCEEDINGS{7037459,
author={N. Zlatanov and V. Jamali and R. Schober},
booktitle={2014 IEEE Global Communications Conference},
title={Achievable rates for the fading half-duplex single relay selection network using buffer-aided relaying},
year={2014},
pages={4156-4161},
keywords={AWGN;fading channels;protocols;relay networks (telecommunication);AWGN;additive white Gaussian noise;buffer-aided relaying protocol;fading half-duplex single relay selection network;independent time-continuous fading;Barium;Delays;Fading;Protocols;Relays;Switches;Wireless communication},
doi={10.1109/GLOCOM.2014.7037459},
ISSN={1930-529X},
month={Dec},}

@book{mir2010computer,
  title={Computer and Communication Networks},
  author={Mir, N.F.},
  isbn={9780131389106},
  lccn={2006025914},
  year={2010},
  publisher={Prentice Hall}
}

@INPROCEEDINGS{6283743,
author={I. Shomorony and A. S. Avestimehr},
booktitle={IEEE Intern. Sym. on Inform. Theory (ISIT)},
title={{Is Gaussian Noise the Worst-case Additive Noise in Wireless Networks?}},
year={2012},
pages={214-218},
month={July}}

@ARTICLE{6807959,
author={N. Zlatanov and A. Ikhlef and T. Islam and R. Schober},
journal={IEEE Communications Magazine},
title={Buffer-aided cooperative communications: opportunities and challenges},
year={2014},
volume={52},
number={4},
pages={146-153},
keywords={buffer storage;cooperative communication;protocols;relay networks (telecommunication);buffer aided cooperative communication;buffer aided protocols;half duplex relays;network topology;one way multirelay network;one way single network;relaying protocols;relays buffer;two way single relay network;Buffer storage;Delays;Relays;Signal to noise ratio;Telecommunication network management;Telecommunication traffic;Throughput},
doi={10.1109/MCOM.2014.6807959},
ISSN={0163-6804},
month={April},}

@ARTICLE{6742713,
author={L. J. Rodriguez and N. H. Tran and T. Le-Ngoc},
journal={IEEE Wireless Commun. Lett.},
title={{Optimal Power Allocation and Capacity of Full-Duplex AF Relaying under Residual Self-Interference}},
year={2014},
volume={3},
number={2},
pages={233-236},
month={April}}

@ARTICLE{6423757,
author={N. Zlatanov and R. Schober},
journal={IEEE Communications Letters},
title={Buffer-Aided Half-Duplex Relaying Can Outperform Ideal Full-Duplex Relaying},
year={2013},
volume={17},
number={3},
pages={479-482},
month={March}}

@ARTICLE{4927468,
author={A. D. Coso and C. Ibars},
journal={IEEE Transactions on Wireless Communications},
title={Achievable rates for the AWGN channel with multiple parallel relays},
year={2009},
volume={8},
number={5},
pages={2524-2534},
keywords={AWGN channels;Rayleigh channels;antenna arrays;channel coding;data compression;decoding;multiplexing;radio networks;relays;AWGN channel;Rayleigh fading channel;Wyner-Ziv compression;additive white Gaussian noise channel;amplify-and-forward scheme;antenna array;compress-and-forward technique;decode-and-forward technique;frequency-flat fading channel;full-duplex operation;linear relaying function;multiple parallel relay technology;signal regeneration scheme;time-invariant system;wireless network;AWGN channels;Antenna arrays;Broadcasting;Decoding;Fading;Frequency;Rayleigh channels;Relays;Transmitting antennas;Wireless networks;Multiple relay channel;achievable rate;compress-and-forward;decode-and-forward;linear relaying;partial decoding},
doi={10.1109/TWC.2009.080288},
ISSN={1536-1276},
month={May},}

@article{Bharadia,
 author = {Bharadia, Dinesh and McMilin, Emily and Katti, Sachin},
 title = {{Full Duplex Radios}},
 journal = {SIGCOMM Comput. Commun. Rev.},
 issue_date = {October 2013},
 volume = {43},
 number = {4},
 month = aug,
 year = {2013},
 issn = {0146-4833},
 pages = {375--386},
 numpages = {12},
 doi = {10.1145/2534169.2486033},
 acmid = {2486033},
 publisher = {ACM},
 address = {New York, NY, USA},
 keywords = {full duplex, interference cancellation, non-linear cancellation},
}

@Article{     abend:70,
  author    = {K.~Abend and B.D.~Fritchman},
  title     = {{S}tatistical {D}etection for {C}ommunication {C}hannels
          with {I}ntersymbol {I}nterference},
  journal   = {Proceedings of the {IEEE}},
  volume    = {58},
  pages     = {779-785},
  month     = may,
  year      = 1970
}

@Article{     Ada92,
  author    = {F.~Adachi and M.~Sawahashi},
  title     = {Performance {A}nalysis of {V}arious 16 {L}evel
          {M}odulation {S}chemes {U}nder {R}ayleigh {F}ading},
  journal   = {Electronics Letters},
  volume    = {28},
  pages     = {1579-1581},
  number    = {17},
  year      = 1992
}

@Article{     Ada93,
  author    = {F.~Adachi and M.~Sawahashi},
  title     = {Decision {F}eedback {M}ultiple--{S}ymbol {D}ifferential
          {D}etection for {M}--ary {DPSK}},
  journal   = {Electronics Letters},
  volume    = {29},
  pages     = {1385-1387},
  number    = {15},
  year      = 1993
}

@Article{     Ada96,
  author    = {F.~Adachi and M.~Sawahashi},
  title     = {{D}ecision {F}eedback {D}ifferential {D}etection of
          {D}ifferentially {E}ncoded {16APSK} {S}ignals},
  journal   = com,
  volume    = {COM-44},
  pages     = {416-418},
  month     = aug,
  year      = 1996
}

@Article{     Ada96a,
  author    = {F.~Adachi},
  title     = {Adaptive differential detection for {M}-ary {DPSK}},
  journal   = {Proceedings of the {IEEE}},
  volume    = {143},
  pages     = {21-28},
  month     = feb,
  year      = 1996
}

@Article{     Ada96b,
  author    = {F.~Adachi},
  title     = {Error {R}ate {A}nalysis of {D}ifferentially {E}ncoded and
          {D}etected {16APSK} {U}nder {R}ician {F}ading},
  journal   = veh,
  volume    = {45},
  pages     = {1-11},
  month     = feb,
  year      = 1996
}

@Article{     Ada98,
  author    = {F.~Adachi},
  title     = {Adaptive {D}ifferential {D}etection {U}sing {L}inear
          {P}rediction for {M}-ary {DPSK}},
  journal   = veh,
  volume    = {47},
  pages     = {909-918},
  month     = oct,
  year      = 1998
}

@Book{        Ada95,
  author    = {R.A.~Adams},
  title     = {{Single-Variable Calculus}},
  publisher = {Addison-Wesley},
  year      = 1995
}

@InProceedings{   adam:72,
  author    = {McAdam, P.L. and Welch, L.R. and Weber, C.L.},
  title     = {{M.A.P.} bit decoding of convolutional codes},
  booktitle = {Int. Symp. Inf. Theory},
  address   = {Asilomar, CA},
  month     = jan,
  year      = 1972
}

@Article{     Ala98,
  author    = {S.M.~Alamouti},
  title     = {{A Simple Transmitter Diversity Scheme for Wireless Communications}},
  journal   = sel,
  volume    = {16},
  pages     = {1451-1458},
  month     = oct,
  year      = 1998
}

@Article{     aldhahir:96,
  author    = {N.~{Al-Dhahir} and J.M.~Cioffi},
  title     = {{B}lock {T}ransmission over {D}ispersive {C}hannels:
          {T}ransmit {F}ilter {O}ptimization and {R}ealization, and
          {MMSE}-{DFE} {R}eceiver {P}erformance},
  journal   = inf,
  volume    = {42},
  pages     = {137-160},
  month     = jan,
  year      = 1996
}

@Article{     AD01,
  author    = {N.~{Al-Dhahir}},
  title     = {{Single--Carrier Frequency--Domain Equalization for Space--Time Block--Coded Transmission Over Frequency--Selective Fading Channels}},
  journal   = {IEEE Commun. Letters},
  volume    = {5},
  pages     = {304-306},
  month     = jul,
  year      = 2001
}

@Article{     AD02,
  author    = {N.~{Al-Dhahir}},
  title     = {{Overview and Comparison of Equalization Schemes for Space--Time--Coded Signals With Application to EDGE}},
  journal   = sip,
  volume    = {50},
  pages     = {2477-2488},
  month     = oct,
  year      = 2002
}

@Article{     aman:91,
  author    = {A.K. Aman and R.L. Cupo and N.A. Zervos},
  title     = {{C}ombined {T}rellis {C}oding and {D}{F}{E} Through
          {T}omlinson {P}recoding},
  journal   = sel,
  volume    = {SAC-9},
  pages     = {876-884},
  month     = aug,
  year      = 1991
}

@Book{        ammon:74,
  author    = {U.v. {Ammon, K. Tr"ondle}},
  title     = {{M}athematische {G}rundlagen der {C}odierung},
  publisher = {Oldenbourg Verlag},
  address   = {M"unchen, Wien},
  year      = 1974
}

@Article{     andersen:73,
  author    = {I.N. Andersen},
  title     = {{Sample--Whitened Matched Filters}},
  journal   = inf,
  volume    = {IT-19},
  pages     = {653-660},
  year      = 1973
}

@Article{     anderson:75,
  author    = {Anderson, J.B. and Bodie, J.B.},
  title     = {Tree encoding of speech},
  journal   = inf,
  volume    = {IT-21},
  pages     = {379-387},
  year      = 1975
}

@Article{     anderson:78,
  author    = {J.B. Anderson and D.P. Taylor},
  title     = {A Bandwidth--Efficient Class of Signal Space Codes},
  journal   = inf,
  volume    = {IT-24},
  pages     = {703-712},
  month     = nov,
  year      = 1978
}

@Article{     anderson:84,
  author    = {J.B.~Anderson and S.~Mohan},
  title     = {{S}equential {C}oding {A}lgorithms: {A} {S}urvey and
          {C}ost {A}nalysis},
  journal   = com,
  volume    = {COM-32},
  pages     = {169-176},
  month     = feb,
  year      = 1984
}

@InProceedings{   anderson:86,
  author    = {Anderson, J.B. and Lin, C.F.},
  title     = {{M}-Algorithm decoding of Channel Convolutional Codes},
  booktitle = {20th Ann. Conf. Inform. Science},
  pages     = {19-21},
  address   = {Princeton University, NJ},
  note      = {Conf. Rec.},
  year      = 1986
}

@Book{        anderson:86b,
  author    = {J.B. Anderson and T. Aulin and C.-E. Sundberg},
  title     = {Digital Phase Modulation},
  publisher = ple,
  address   = {New York},
  year      = 1986
}

@Book{        andexser:77,
  author    = {W. Andexser},
  title     = {{U}ntersuchung von {D}aten"ubertragungssystemen mit
          adaptiver quantisierter {R}"uckkopplung},
  publisher = {Dissertation, TU Stuttgart},
  year      = 1977
}

@Article{     andfo:75,
  author    = {R.R.~Anderson and G.J.~Foschini},
  title     = {{T}he {M}inimum {D}istance for {MLSE} {D}igital {D}ata
          {S}ystems of {L}imited {C}omplexity},
  journal   = inf,
  volume    = {IT-21},
  pages     = {544-551},
  month     = sep,
  year      = 1975
}

@Article{     AT01,
  author    = {A.~Annamalai and C.~Tellambura},
  title     = {{Error Rates for Nakagami-$m$ Fading Multichannel Reception of Binary and $M$-ary Signals}},
  journal   = com,
  volume    = {COM-49},
  pages     = {58-68},
  month     = jan,
  year      = 2001
}

@Article{     ATB05,
  author    = {A.~Annamalai and C.~Tellambura and V.K.~Bhargava},
  title     = {{A General Method for Calculating Error Probabilities Over Fading Channels}},
  journal   = com,
  volume    = {COM-53},
  pages     = {841-852},
  month     = may,
  year      = 2005
}

@Article{     Arn66,
  author    = {L.~Arnold},
  title     = {{\"Uber die Nullstellenverteilung zuf\"alliger Polynome (\it in German)}},
  journal   = {Math.~Zeitschrift},
  volume    = {92},
  pages     = {12-18},
  month     = {},
  year      = 1966
}

@Book{        ascheid:84,
  author    = {G. Ascheid},
  title     = {{O}ptimale {D}etektion und {S}ynchronisation mit digitaler
          {S}ignalverarbeitung},
  publisher = {Dissertation, Rheinisch--Westf"alische Technische
          Hochschule Aachen},
  year      = 1984
}

@Article{     aulin:81a,
  author    = {T. Aulin and C.-E. Sundberg},
  title     = {Continous Phase Modulation -- Part {I}: Full Response
          Signalling},
  journal   = com,
  volume    = {COM-29},
  pages     = {196-209},
  month     = mar,
  year      = 1981
}

@Article{     aulin:81b,
  author    = {T. Aulin and C.-E. Sundberg and N. Rydbeck},
  title     = {Continous Phase Modulation -- Part {II}: Partial Response
          Signalling},
  journal   = com,
  volume    = {COM-29},
  pages     = {210-225},
  month     = mar,
  year      = 1981
}

@Article{     aulin:81c,
  author    = {T. Aulin},
  title     = {Symbol Error Probability Bounds for Coherently Viterbi
          Detected Continuous Phase Modulated Signals},
  journal   = com,
  volume    = {COM-29},
  pages     = {1707-1715},
  month     = nov,
  year      = 1981
}

@Article{     aulin:82,
  author    = {T. Aulin and C.-E. Sundberg},
  title     = {Exact asymptotic Behaviour of Digital {FM}--Spektra},
  journal   = com,
  volume    = {COM-30},
  pages     = {2438-2449},
  year      = 1982
}

@Article{     aulin:83,
  author    = {T. Aulin and C.-E. Sundberg},
  title     = {An easy way to calculate power spectrum for digital {FM}},
  journal   = {IEE Proc. -- F Commun.},
  volume    = {},
  pages     = {519-525},
  month     = {},
  year      = 1983
}

@Book{        azizi:88,
  author    = {S.A. Azizi},
  title     = {{E}ntwurf und {R}ealisierung digitaler {F}ilter},
  publisher = old,
  address   = {M"unchen, Wien},
  year      = 1988
}

@Article{     baccala:94,
  author    = {L.A.~Baccala and S.~Roy},
  title     = {{A} {N}ew {B}lind {T}ime--{D}omain {C}hannel
          {I}dentification {M}ethod {B}ased on {C}yclostationarity},
  journal   = siplett,
  volume    = {1},
  pages     = {89-91},
  month     = jun,
  year      = 1994
}

@InProceedings{   BM99,
  author    = {K.E.~Baddour and P.J.~McLane},
  title     = {{Analysis of Optimum Diversity Combining and Decision Feedback Equalization in Dispersive Rayleigh Fading}},
  booktitle = {Proc. of IEEE Intern. Commun. Conf.},
  pages     = {21-26},
  adrress   = {Vancouver},
  month     = jun,
  year      = 1999
}

@Article{     bahl:74,
  author    = {Bahl, L.R. and Cocke, J. and Jelinek, F. and Raviv, J.},
  title     = {{Optimal Decoding of Linear Codes for Minimizing Symbol
          Error Rate}},
  journal   = inf,
  volume    = {IT-20},
  pages     = {284-287},
  year      = 1974
}

@Article{     bahlcull:72,
  author    = {L.R.~Bahl and C.D.~Cullum and W.D.~Frazer and F.~Jelinek},
  title     = {{A}n {E}fficient {A}lgorithm for {C}omputing {F}ree
          {D}istance},
  journal   = inf,
  volume    = {IT-18},
  pages     = {437-439},
  month     = may,
  year      = 1972
}

@Article{     baker:74,
  author    = {T.J. Baker},
  title     = {Asymptotic Behaviour of Digital {FM}--Spektra},
  journal   = com,
  volume    = {COM-22},
  pages     = {1585-1594},
  year      = 1974
}

@Article{     BS92,
  author    = {P.~Balaban and J.~Salz},
  title     = {{Optimum Diversity Combining and Equalization in Digital Data Transmission with Applications to Cellular Mobile Radio -- Part I and II}},
  journal   = com,
  volume    = {40},
  pages     = {885--907},
  month     = may,
  year      = 1992
}

@Article{     barbosa:89,
  author    = {L.C.~Barbosa},
  title     = {{M}aximum {L}ikelihood {S}equence {E}stimators: {A}
          {G}eometric {V}iew},
  journal   = inf,
  volume    = {IT-35},
  pages     = {419-427},
  month     = mar,
  year      = 1989
}

@Article{     battail:87,
  author    = {Battail, G.},
  title     = {Pond\'eration des symboles d\'ecode\'es par l'algorithme
          de Viterbi},
  journal   = {Annales des Telecommunications},
  volume    = {tome 42},
  pages     = {31-38},
  year      = 1987
}

@Book{        bauer:91,
  author    = {D.~Bauer},
  title     = {{E}inheitliche {B}eschreibung und vergleichende {A}nalyse
          suboptimaler sequentieller {D}etektionsalgorithmen f"ur die
          {E}ntscheidung verzerrter und gest"orter {D}atensignale},
  publisher = {Dissertation, Universit"at Kaiserslautern},
  month     = jan,
  year      = 1991
}

@Article{     Bea78,
  author    = {C.~T.~Beare},
  title     = {{The Choice of the Desired Impulse Response in Combined Linear--Viterbi Algorithm Equalizers}},
  journal   = com,
  volume    = {COM-26},
  pages     = {1301-1327},
  month     = aug,
  year      = 1978
}

@Article{     beaulieu:93,
  author    = {S.A.~Altekar and N.C.~Beaulieu},
  title     = {{U}pper {B}ounds to the {E}rror {P}robability of
          {D}ecision {F}eedback {E}qualization},
  journal   = inf,
  volume    = {IT-39},
  pages     = {145-156},
  month     = jan,
  year      = 1993
}

@Book{        beck:88,
  author    = {H. Beckmann},
  title     = {{L}eistungsspektrum und {S}ynchronisation bei codierten
          und modulierten {D}igitalsignalen und ihre {A}nwendung bei
          {CPM}},
  publisher = {Dissertation, Universit"at der Bundeswehr M"unchen},
  year      = 1989
}

@Article{     BP79,
  author    = {C.~A.~Belfiore and J.~H.~Park},
  title     = {{Decision--Feedback Equalization}},
  journal   = {Proceedings of the {IEEE}},
  volume    = {67},
  pages     = {1143-1156},
  month     = aug,
  year      = 1979
}

@InCollection{    bellini:86,
  author    = {S.~Bellini and F.~Rocca},
  title     = {{B}lind {D}econvolution: {P}olyspectra or {B}ussgang
          {T}echniques?},
  booktitle = {{D}igital {C}ommunications},
  publisher = {North--Holland},
  year      = {1986},
  editor    = {E.~Biglieri and G.~Prati},
  pages     = {251-263},
  address   = {Amsterdam}
}

@Book{        bellman:57,
  author    = {Bellman, R.E.},
  title     = {Dynamic Programming},
  publisher = {Princeton University Press},
  address   = {Princeton, NJ},
  year      = 1957
}

@Article{     Bel62,
  author    = {P.~A.~Bello, B.~D.~Nelin},
  title     = {{T}he {I}nfluence of {F}ading {S}pectrum on the {B}inary
          {E}rror {P}robabilities of {I}ncoherent and {D}ifferentially {C}oherent {M}atched {F}ilter {R}eceivers},
  journal   = {{IRE} {T}ransactions on {C}ommunication {S}ystems},
  volume    = {CS-10},
  pages     = {160-168},
  month     = jun,
  year      = 1962
}

@Article{     benelli:94,
  author    = {G.~Benelli and A.~Fioravanti and A.~Garzelli and
          P.~Matteini},
  title     = {{S}ome digital receivers for the {GSM} pan-{E}uropean
          cellular communication system},
  journal   = {IEE Proc.-Commun.},
  volume    = {Vol.141},
  pages     = {168-176},
  month     = jun,
  year      = 1994
}

@Article{     benveniste:80,
  author    = {A.~Benveniste and M.~Goursat and G.~Rouget},
  title     = {{R}obust {I}dentification of a {N}onminimum {P}hase
          {S}ystem: {B}lind {A}djustment of a {L}inear {E}qualizer in
          {D}ata {C}ommunications},
  journal   = ac,
  volume    = {AC-25},
  pages     = {385-399},
  month     = jun,
  year      = 1980
}

@Article{     benveniste:84,
  author    = {A.~Benveniste},
  title     = {{B}lind {E}qualizers},
  journal   = com,
  volume    = {COM-32},
  pages     = {871-883},
  month     = aug,
  year      = 1984
}

@Article{     benvenuto:96,
  author    = {N.~Benvenuto and R.~Marchesani},
  title     = {{T}he {V}iterbi {A}lgorithm for {S}parse {C}hannels},
  journal   = com,
  volume    = {COM-44},
  pages     = {287-289},
  month     = mar,
  year      = 1996
}

@Article{     berger:67,
  author    = {Berger, T. and Tufts, D.W.},
  title     = {{Optimum Pulse Amplitude Modulation, Part {I}:
          Transmitter-Receiver Design and Bounds from Information
          Theory}},
  journal   = inf,
  volume    = {IT-13},
  pages     = {196-208},
  year      = 1967
}

@Book{        bergmans:87,
  author    = {J.W.M.~Bergmans},
  title     = {{Partial Response Techniques and Robustness in Data
          Equalization}},
  publisher = {Dissertation, Technische Universit"at Eindhoven},
  month     = sep,
  year      = 1987
}

@Book{        berle:68,
  author    = {E.R. Berlekamp},
  title     = {Algebraic Coding Theory},
  publisher = {McGraw-Hill},
  address   = {New York},
  year      = 1968
}

@InProceedings{   berrou:93,
  author    = {Berrou and Glavieux and Thitimajshima},
  title     = {{N}ear {S}hannon {L}imit {E}rror-{C}orrecting {C}oding and
          {D}ecoding: {T}urbo-{C}odes (1)},
  booktitle = {Proceedings of the International Conference on
          Communications ({ICC}'93)},
  note      = {Conf. Record},
  pages     = {1064-1070},
  adrress   = {Geneva},
  month     = may,
  year      = 1993
}

@InProceedings{   bertelsmeier:86a,
  author    = {M. Bertelsmeier},
  title     = {Digital signal transmission with trellis--coded phase
          shift keyed signals},
  booktitle = {Proceedings of the {ICDSC}-7},
  address   = {Munich},
  pages     = {323-330},
  month     = may,
  year      = 1986
}

@InProceedings{   bertelsmeier:86b,
  author    = {M. Bertelsmeier},
  title     = {Modified coded octal phase--shift keying with improved
          carrier--phase tracking ability},
  booktitle = {Proceedings of the GLOBECOM'86},
  address   = {Houston},
  pages     = {1356-1360},
  month     = nov,
  year      = 1986
}

@Article{     bertelsmeier:89a,
  author    = {M. Bertelsmeier and G. Komp},
  title     = {Trellis--coded {8PSK} with Embedded {QPSK}},
  journal   = sel,
  volume    = {SAC-7},
  pages     = {1296-1306},
  month     = dec,
  year      = 1989
}

@InProceedings{   bertelsmeier:89b,
  author    = {M. Bertelsmeier and G. Komp},
  title     = {Coded Phase--Shift Keying with Time--Varying Signal Sets},
  booktitle = {Proceedings of the {ICDSC}-8},
  address   = {Guadeloupe},
  month     = apr,
  year      = 1989
}

@Book{        bhargava:81,
  author    = {V.K. Bhargava and D. Haccoun and R. Matyes and P.P.
          Nuspl},
  title     = {Digital Communications by Satellite},
  publisher = wil,
  address   = {New York},
  year      = 1981
}

@Article{     biglieri:84,
  author    = {E. Biglieri},
  title     = {High--level modulation and coding for nonlinear satellite
          channels},
  journal   = com,
  volume    = {COM--32},
  pages     = {616-626},
  month     = {},
  year      = {1984}
}

@Article{     biglieri:86,
  author    = {E.~Biglieri},
  title     = {{Ungerboeck Codes Do Not Shape the Signal Power
          Spectrum}},
  journal   = inf,
  volume    = {IT-32},
  pages     = {595-596},
  month     = jul,
  year      = 1986
}

@Book{        biglieri:87,
  author    = {S. Benedetto and E. Biglieri and V. Castellani},
  title     = {Digital Transmission Theory},
  publisher = {Prentice--Hall},
  address   = {Englewood Cliffs, N.J.},
  year      = {1987}
}

@Book{        biglieri:91,
  author    = {E. {Biglieri e.a.}},
  title     = {Introduction to Trellis--Coded Modulation with
          Applications},
  publisher = {Macmillan},
  address   = {New York},
  year      = {1991}
}

@Article{     BCTV98,
  author    = {E.~Biglieri and G.~Caire and G.~Taricco and J.~Ventura--Traveset},
  title     = {{Computing Error Probabilities over Fading Channels: a Unified Approach}},
  journal   = {European Transactions on Telecommunications},
  volume    = {9},
  pages     = {15-25},
  month     = {January-Feburary},
  year      = 1998
}

@InProceedings{   Bin97,
  author    = {L.~Bin and P.~Ho},
  title     = {{A} {N}ew {D}ecision--{F}eedback {DPSK} {R}eceiver with {B}lind
          {P}hase {P}rediction},
  booktitle = {Proceedings of Globecom'97},
  pages     = {337-341},
  month     = nov,
  address   = {Phoenix, Arizona, USA},
  year      = 1997
}

@Book{        bingham:88,
  author    = {J.A.C.~Bingham},
  title     = {The Theory and Practice of Modem Design},
  publisher = {J. Wiley \& Sons},
  address   = {New York},
  year      = 1988
}

@Book{rappaport02,
  author    = {T.~S.~Rappaport},
  title     = {Wireless Communications : Principles and Practice},
  publisher = {Prentice Hall},
  address   = {New York},
  year      = 2002
}

@Book{TSE05,
  author    = {D.~Tse and P.~Viswanath},
  title     = {Fundamentals of Wireless Communication},
  publisher = {Cambridge University Press},
  year      = 2005
}

@Book{        blahut:83,
  author    = {Richard E. Blahut},
  title     = {Theory and Practice of Error Control Codes},
  publisher = {Addison--Wesley},
  address   = {Reading, Massachusetts},
  year      = 1983
}

@Book{        blahut:87,
  author    = {Richard E. Blahut},
  title     = {Principles and Practice of Infomation Theory},
  publisher = {Addison--Wesley},
  address   = {Reading, Mass.},
  year      = 1987
}

@Book{        blahut:90,
  author    = {R.E. Blahut},
  title     = {Digital Transmission of Information},
  publisher = {Addison--Wesley},
  address   = {Reading, Mass.},
  year      = {1990}
}

@Book{        bocker:76,
  author    = {P. Bocker},
  title     = {Daten"ubertragung},
  note      = {B"ande {I} und {II}},
  publisher = spr,
  address   = {Berlin},
  year      = {1976,1977}
}

@InProceedings{   BP00,
  author    = {H.~B\"olcskei and A.J.~Paulraj},
  title     = {{Space--Frequency Coded Broadband OFDM Systems}},
  booktitle = {Proceedings of IEEE Wireless Commun.~and Networking Conf.~(WCNC)},
  address   = {Chicago (IL)},
  pages     = {1-6},
  month     = sep,
  year      = 2000
}

@InProceedings{   BP00a,
  author    = {H.~B\"olcskei and A.J.~Paulraj},
  title     = {{Performance of Space-Time Codes in the Presence of Spatial Fading Correlation}},
  booktitle = {Proceedings of 34th Asilomar Conf.~on Signals, Systems and Computers},
  address   = {Pacific Grove},
  pages     = {686-693},
  month     = nov,
  year      = 2000
}

@Article{     Bol06,
  author    = {H.~B\"olcskei},
  title     = {{MIMO--OFDM Wireless Systems: Basics, Perspectives, and Challenges}},
  journal   = {IEEE Wireless Commun.},
  volume    = {13},
  pages     = {31-37},
  month     = aug,
  year      = 2006
}

@Book{        Bor91,
  author    = {E.~J.~Borowski and J.~M.Borwein},
  title     = {The {H}arper {C}ollins {D}ictionary of {M}athematics},
  publisher = {Harper {P}erennial},
  address   = {New York},
  year      = 1991
}

@Book{        bossert:92,
  author    = {M. Bossert},
  title     = {{K}analcodierung},
  publisher = teu,
  address   = {Stuttgart},
  year      = 1992
}

@Article{     BFY04,
  author    = {J.~Boyer and D.D.~Falconer and H.~Yanikomeroglu},
  title     = {{Multihop Diversity in Wireless Relaying Channels}},
  journal   = com,
  volume    = {COM-52},
  pages     = {1820-1830},
  month     = oct,
  year      = 2004
}

@Article{     bune:91,
  author    = {P.A.M.~Bun\'e},
  title     = {{A} {F}ast {C}oefficient {C}omputation {A}lgorithm for
          {T}ransversal and {D}ecision--{F}eedback {E}qualizers},
  journal   = {European Transactions on Telecommunications},
  volume    = {2},
  pages     = {251-258},
  month     = mar # "-"  # apr,
  year      = 1991
}

@Article{     cain:79,
  author    = {J.B. Cain and G.C. Clark and J.M. Geist},
  title     = {Punctured convolutional codes of rate $(n-1)/n$ and
          simplified maximum likelihood decoding},
  journal   = inf,
  volume    = {IT-25},
  pages     = {97-100},
  month     = jan,
  year      = 1979
}

@Article{     calderbank:84,
  author    = {A.R. Calderbank and J.E. Mazo},
  title     = {A new description of trellis codes},
  journal   = inf,
  volume    = {IT-30},
  pages     = {784-791},
  month     = nov,
  year      = 1984
}

@Article{     calderbank:85,
  author    = {A.R. Calderbank and N.J.A. Sloane},
  title     = {Four--dimensional modulation with an eight--state trellis
          code},
  journal   = {AT{\rm\&}T Tech. J.},
  volume    = {64},
  pages     = {1005-1018},
  month     = may # "-"  # jun,
  year      = 1985
}

@Article{     calderbank:86,
  author    = {A.R. Calderbank and N.J.A. Sloane},
  title     = {An Eight--Dimensional Trellis Code},
  journal   = {Proceedings of the {IEEE}},
  volume    = {74},
  pages     = {757-759},
  month     = may,
  year      = 1986
}

@Article{     calderbank:87,
  author    = {A.R. Calderbank and N.J. Sloane},
  title     = {New trellis codes based on lattices and cosets},
  journal   = inf,
  volume    = {IT-33},
  pages     = {177-195},
  year      = 1987
}

@Article{     calderbank:89,
  author    = {A.R. Calderbank},
  title     = {{M}ultilevel {C}odes and {M}ultistage {D}ecoding},
  journal   = com,
  volume    = {COM-37},
  pages     = {222-229},
  month     = mar,
  year      = {1989}
}

@Article{     calderbank:89a,
  author    = {A.R.~Calderbank and J.E.~Mazo},
  title     = {{B}aseband {L}ine {C}odes {V}ia {S}pectral
          {F}actorization},
  journal   = sel,
  volume    = {SAC-7},
  pages     = {914-928},
  month     = aug,
  year      = 1989
}

@Article{     cariolaro:74,
  author    = {G.L. Cariolaro and G.P. Tronca},
  title     = {Spectra of block coded digital signals},
  journal   = com,
  volume    = {COM-22},
  pages     = {1555-1564},
  month     = {},
  year      = {1974}
}

@Article{     cariolaro:75,
  author    = {G.L. Cariolaro and S. Pupolin},
  title     = {Moments of correlated digital signals for error
          probability evaluation},
  journal   = inf,
  volume    = {IT-21},
  pages     = {558-568},
  month     = {},
  year      = {1975}
}

@Article{     CH92,
  author    = {J.K.~Cavers and P.~Ho},
  title     = {{Analysis of the Error Performance of Trellis--Coded Modulations in Rayleigh--Fading Channels}},
  journal   = com,
  volume    = {COM-40},
  pages     = {74-83},
  month     = jan,
  year      = {1992}
}

@InProceedings{   CER05,
  author    = {C.A.~Corral and S.~Emami and G.~Rasor},
  title     = {{Model of Multi-Band OFDM Interference on Broadband QPSK Receivers}},
  booktitle = {Proceedings of the IEEE International Conference on Acoustics, Speech, and Signal Processing (ICASSP)},
  address   = {Philadelphia},
  pages     = {629-632},
  month     = nov,
  year      = 2005
}

@InProceedings{   CC99,
  author    = {W.--J.~Choi and J.M.~Cioffi},
  title     = {{Space--Time Block Codes over Frequency Selective Rayleigh Fading Channels}},
  booktitle = {IEEE Veh.~Technol.~Conf.},
  address   = {},
  pages     = {2541-2545},
  month     = nov,
  year      = 1999
}

@Article{     chang:66,
  author    = {Chang, R.W. and Hancock, J.C.},
  title     = {On receiver structures for channels having memmory},
  journal   = inf,
  volume    = {IT-12},
  pages     = {463-468},
  year      = 1966
}

@InProceedings{   chang:95,
  author    = {K.-H.~Chang and C.N.~Georghiades},
  title     = {{I}terative {J}oint {S}equence and {C}hannel {E}stimation
          for {F}ast {T}ime--{V}arying {I}ntersymbol {I}nterference
          {C}hannels},
  booktitle = {Proceedings of the International Conference on
          Communications ({ICC}'95)},
  pages     = {357-361},
  address   = {Seattle},
  month     = jun,
  year      = 1995
}

@Article{     chev:89,
  author    = {P.R. Chevillat and E. Eleftheriou},
  title     = {{Decoding of Trellis--Encoded Signals in the Presence of
          Intersymbol Interference and Noise}},
  journal   = com,
  volume    = {COM-37},
  pages     = {669-676},
  month     = jul,
  year      = 1989
}

@Article{     Cho92,
  author    = {Y.~C.~Chow and A.~R.~Nix and J.~P.~McGeehan},
  title     = {Analysis of 16--{APSK} {M}odulation in {AWGN} and {R}ayleigh {F}ading {C}hannel},
  journal   = {Electronics Letters},
  volume    = {28},
  pages     = {1608-1610},
  number    = {17},
  year      = 1992
}

@Article{     Cho93,
  author    = {Y.~C.~Chow and A.~R.~Nix and J.~P.~McGeehan},
  title     = {Diversity improvement for 16--{DAPSK} in {R}ayleigh fading channel},
  journal   = {Electronics Letters},
  volume    = {29},
  pages     = {387-389},
  number    = {4},
  year      = 1993
}

@Book{        chung:67,
  author    = {Chung, K. L.},
  title     = {Markov chains with stationary transition probabilities},
  publisher = {Springer Verlag},
  address   = {Berlin},
  editon    = {second},
  year      = {1967}
}

@Article{     cioffi:84,
  author    = {J.M.~Cioffi and T.~Kailath},
  title     = {Fast recursive--least--squares transversal filters for
          adaptive filtering},
  journal   = assp,
  volume    = {ASSP-32},
  pages     = {304-337},
  year      = 1984
}

@InProceedings{   cioffi:86,
  author    = {J.M.~Cioffi},
  title     = {{A}n error event length conjecture},
  booktitle = {Proceedings of the Conference on Specific Problems in
          Communication and Computation},
  address   = {Palo Alto, CA},
  month     = sep,
  year      = 1986
}

@InProceedings{   cioffi:90,
  author    = {J.M.~Cioffi and P.H.~Algoet and P.S.~Chow},
  title     = {{C}ombined {E}qualization and {C}oding with
          {F}inite-{L}ength {D}ecision {F}eedback {E}qualization},
  booktitle = {Proceedings of the IEEE Global Telecommunication
          Conference (GLOBECOM'90)},
  pages     = {1664-1668},
  address   = {San Diego},
  month     = nov,
  year      = 1990
}

@InProceedings{   cioffi:92,
  author    = {N.M.W.~{Al-Dhahir} and J.M.~Cioffi},
  title     = {{F}ast {A}lgorithms for the {C}omputation of the {F}inite
          {L}ength {D}ecision {F}eedback {E}qualizer},
  booktitle = {Proceedings of ICASSP'92},
  pages     = {IV-533-IV-536},
  month     = mar,
  year      = 1992
}

@Article{     cioffi:95,
  author    = {N.~{Al-Dhahir} and J.~M.~Cioffi},
  title     = {{MMSE} {D}ecision-{F}eedback {E}qualizers:
          {F}inite-{L}ength {R}esults},
  journal   = inf,
  volume    = {IT-41},
  pages     = {961-975},
  month     = jul,
  year      = 1995
}

@Article{     cioffi:95b,
  author    = {N.~{Al-Dhahir} and J.M.~Cioffi},
  title     = {{F}ast {C}omputation of {C}hannel-{E}stimate {B}ased
          {E}qualizers in {P}acket {D}ata {T}ransmission},
  journal   = sip,
  volume    = {43},
  pages     = {2462-2473},
  month     = nov,
  year      = 1995
}

@Article{     cioffi:95c,
  author    = {I.~Lee and J.M.~Cioffi},
  title     = {{A} {F}ast {C}omputation {A}lgorithm for the {D}ecision
          {F}eedback {E}qualizer},
  journal   = com,
  volume    = {COM-43},
  pages     = {2742-2749},
  month     = nov,
  year      = 1995
}

@Article{     CDEF95,
  author    = {J.~M.~Cioffi and G.~P.~Dudevoir and M.~V.~Eyuboglu
          and G.~D.~Forney Jr.},
  title     = {{MMSE} {D}ecision--{F}eedback {E}qualizers and {C}oding -- {P}art {I}: {E}qualization {R}esults},
  journal   = com,
  volume    = {43},
  pages     = {2582-2594},
  month     = oct,
  year      = 1995
}

@Book{        clark:82,
  author    = {G.C. Clark and J.B. Cain},
  title     = {Error-Correction Coding for Digital Communications},
  publisher = {Plenum Press},
  edition   = {second},
  address   = {New York},
  year      = 1982
}

@Article{     CGKS92,
  author    = {M.~Clark and L.~Greenstein and W.~Kennedy and M.~Shafi},
  title     = {{Matched Filter Performance Bounds for Diversity Combining Receivers in Digital Mobile Radio}},
  journal   = veh,
  volume    = {41},
  pages     = {356-362},
  month     = nov,
  year      = 1992
}

@Article{     CGKS94,
  author    = {M.V.~Clark and L.J.~Greenstein and W.K.~Kennedy and M.~Shafi},
  title     = {{Optimum Linear Diversity Receivers for Mobile Communications}},
  journal   = veh,
  volume    = {43},
  pages     = {47-56},
  month     = feb,
  year      = 1994
}

@Article{     Col98,
  author    = {G.~Colavolpe and P.~Castoldi and R.~Raheli},
  title     = {{Linear predictive receivers for fading channels}},
  journal   = {Electronics Letters},
  volume    = {34},
  pages     = {1289-1290},
  month     = jun,
  year      = 1998
}

@Book{        conrads:89,
  author    = {D. Conrads},
  title     = {{D}atenkommunikation ({V}erfahren, {N}etze, {D}ienste)},
  publisher = {Friedr. Vieweg \& Sohn},
  address   = {Braunschweig / Wiesbaden},
  year      = 1989
}

@Book{        conway:87,
  author    = {J.H. Conway and N.J.A. Sloane},
  title     = {Sphere Packings, Lattices and Groups},
  publisher = {Springer Verlag},
  address   = {New York},
  year      = 1987
}

@Article{     costello:96,
  author    = {L.C. Perez and J. Seghers and D.J. {Costello, Jr.}},
  title     = {{A} {D}istance {S}pectrum {I}nterpretation of {T}urbo
          {C}odes},
  journal   = inf,
  volume    = {IT-42},
  pages     = {1698-1722},
  month     = nov,
  year      = 1996
}

@INPROCEEDINGS{7343304,
author={K. T. Phan and T. Le-Ngoc},
booktitle={Personal, Indoor, and Mobile Radio Communications (PIMRC), 2015 IEEE 26th Annual International Symposium on},
title={{Buffer-Aided Full-Duplex Relaying with Residual Self-Interference and Statistical Delay Provisioning}},
year={2015},
pages={250-255},
month={Aug}}

@ARTICLE{BA-relaying-adaptive-rate,
  author={N. Zlatanov and R. Schober and P. Popovski},
journal=sel,
title={{Buffer-Aided Relaying with Adaptive Link Selection}},
year={2013},
volume={31},
number={8},
pages={1530-1542},
month=aug}


@ARTICLE{cover,
  author    = {T.M.~Cover and A.A.~{El Gamal}},
  title     = {{Capacity Theorems for the Relay Channel}},
  journal   = inf,
  volume    = {25},
  pages     = {572-584},
  month     = sep,
  year      = 1979
}

@Article{     CFM91,
  author    = {S.N.~Crozier and D.D.~Falconer and S.A.~Mahmoud},
  title     = {{Least sum of squared errors (LSSE) channel estimation}},
  journal   = {IEE Proceedings-F},
  volume    = {138},
  pages     = {371-378},
  month     = aug,
  year      = 1991
}

 @Article{    Dam94,
  author    = {W.~C.~Dam and D.~P.~Taylor},
  title     = {{A}n {A}daptive {M}aximum {L}ikelihood {R}eceiver for
          {C}orrelated {R}ayleigh--{F}ading {C}hannels},
  journal   = com,
  volume    = {COM-42},
  pages     = {2684-2692},
  month     = sep,
  year      = 1994
}

@Article{     daut:82,
  author    = {D.G. Daut and J.W. Modestino and L.D. Wismer},
  title     = {New Short Constraint Length Convolutional Code
          Constructions for Selected Rates},
  journal   = inf,
  volume    = {IT-28},
  nmber     = {No.5},
  pages     = {794-800},
  month     = sep,
  year      = 1982
}

@Article{     DBV04,
  author    = {P.~Dayal and M.~Brehler and M.K.~Varanasi},
  title     = {{Leveraging Coherent Space-Time Codes for Noncoherent Communications via Training}},
  journal   = inf,
  volume    = {IT-50},
  pages     = {2058-2080},
  month     = sep,
  year      = 2004
}

@Article{     ding:93,
  author    = {Z.~Ding and R.A.~Kennedy and B.D.O.~Anderson and
          C.R.~{Johnson, Jr.}},
  title     = {{L}ocal {C}onvergence of the {S}ato {B}lind {E}qualizer
          and {G}eneralizations {U}nder {P}ractical {C}onstraints},
  journal   = inf,
  volume    = {IT-39},
  pages     = {129-144},
  month     = jan,
  year      = 1993
}

@InProceedings{   divsalar:86,
  author    = {Divsalar, D. and Simon, M.K.},
  title     = {Multiple Trellis Coded Modulation ({MTCM})},
  booktitle = {Proceedings of the GLOBECOM '86},
  address   = {Houston},
  pages     = {30.8.1-30.8.7},
  month     = {},
  year      = 1986
}

@Article{     divsalar:88,
  author    = {Divsalar, D. and Simon, M.K.},
  title     = {Multiple Trellis Coded Modulation ({MTCM})},
  journal   = com,
  volume    = {COM-36},
  pages     = {410-419},
  month     = {},
  year      = 1988
}

@Article{     Div90a,
  author    = {D. Divsalar and M.K. Simon and M. Shahshahani},
  title     = {The Performance of Trellis--Coded {MDPSK} with Multiple
          Symbol Detection},
  journal   = com,
  volume    = {COM-38},
  pages     = {1391-1403},
  month     = sep,
  year      = 1990
}

@Article{     Div90,
  author    = {D.~Divsalar and M.K.~Simon},
  title     = {{M}ultiple--{S}ymbol {D}ifferential {D}etection of
          {MPSK}},
  journal   = com,
  volume    = {COM-38},
  pages     = {300-308},
  month     = mar,
  year      = 1990
}

@Article{     Div94,
  author    = {D.~Divsalar and M.K.~Simon},
  title     = {{M}aximum--{L}ikelihood {D}ifferential {D}etection of
          {U}ncoded and {T}rellis {C}oded {A}mplitude {P}hase {M}odulation
          over {AWGN} and {F}ading {C}hannels -- {M}etrics and {P}erformance},
  journal   = com,
  volume    = {COM-94},
  pages     = {76-89},
  month     = jan,
  year      = 1994
}

@Article{     dollard:64,
  author    = {P.M. Dollard},
  title     = {On the Time--Bandwidth Concentration of Signal Functions
          Forming Given Geometric Vector Configuration},
  journal   = inf,
  volume    = {IT-10},
  pages     = {328-338},
  month     = oct,
  year      = 1964
}

@Article{     Don98,
  author    = {X.~Dong and T.~T.~.Tjhung and F.~Adachi},
  title     = {Error {P}robability {A}nalysis for 16 {STAR}--{QAM} in
          {F}requency--{S}elective {R}ician {F}ading with {D}iversity {R}eception},
  journal   = veh,
  volume    = {47},
  pages     = {924-935},
  month     = aug,
  year      = 1998
}

@InProceedings{   dorsch:83,
  author    = {B. Dorsch},
  title     = {Successive Check Digits Rather than Information
          Repetition},
  booktitle = {Proceedings of the Int. Comm. Conference ({ICC}'83),
          Boston},
  pages     = {323-327},
  month     = jun,
  year      = 1983
}

@InProceedings{   duel:85,
  author    = {A. Duel and C. Heegard},
  title     = {{Delayed decision--feedback sequence estimation}},
  booktitle = {Proceedings of the 23rd. Annual Allerton Conference
          Commun., Contr. Comput.},
  month     = oct,
  address   = {Allerton},
  year      = 1985
}

@Article{     DH89,
  author    = {A.~{Duel-Hallen} and A. C.~Heegard},
  title     = {{Delayed Decision--Feedback Sequence Estimation}},
  journal   = com,
  volume    = {37},
  pages     = {428-436},
  month     = {},
  year      = 1989
}

@Article{     duttweiler:74,
  author    = {D.L.~Duttweiler and J.E.~Mazo and D.G.~Messerschmitt},
  title     = {{A}n {U}pper {B}ound on the {E}rror {P}robability in
          {D}ecision-{F}eedback {E}qualization},
  journal   = inf,
  volume    = {IT-20},
  pages     = {490-497},
  month     = jul,
  year      = 1974
}

@InProceedings{   edbauer:87,
  author    = {F. Edbauer},
  title     = {Coded 8--{DPSK} modulation with differentially coherent
          detection --- An efficient modulation scheme for fading
          channels},
  booktitle = {Conference Record of the {GLOBECOM}'87},
  volume    = {3},
  pages     = {42.2.1-42.2.4},
  address   = {Tokyo},
  month     = nov,
  year      = 1987
}

@Article{     edbauer:89,
  author    = {F. Edbauer},
  title     = {Performance of Interleaved Trellis--Coded Differential
          8--{PSK} Modulation Over Fading Channels},
  journal   = sel,
  volume    = {SAC-7},
  pages     = {1340-1346},
  month     = dec,
  year      = 1989
}

@Article{     Edb92,
  author    = {F.~Edbauer},
  title     = {{B}it {E}rror {R}ate of {B}inary and {Q}uaternary {DPSK}
          {S}ignals with {M}ultiple {D}ifferential {F}eedback {D}etection},
  journal   = com,
  volume    = {COM-40},
  pages     = {457-460},
  month     = mar,
  year      = 1992
}

@Article{     Edb92,
  author    = {F.~Edbauer},
  title     = {{B}it {E}rror {R}ate of {B}inary and {Q}uaternary {DPSK}
          {S}ignals with {M}ultiple {D}ifferential {F}eedback {D}etection},
  journal   = com,
  volume    = {COM-40},
  pages     = {457-460},
  month     = mar,
  year      = 1992
}

@Article{     Ede95,
  author    = {A.~Edelman and E.~Kostlan},
  title     = {{How Many Zeros of a Random Polynomial are Real}},
  journal   = {Bulletin of the American Mathematical Society},
  volume    = {32},
  pages     = {1-37},
  month     = jan,
  year      = 1995
}

@Article{     elias:55,
  author    = {P. Elias},
  title     = {Coding for Noisy Channels},
  journal   = {IRE Conv. Rec.},
  volume    = {Part 4},
  pages     = {37-47},
  year      = 1955
}

@Article{     ericson:71,
  author    = {T.~Ericson},
  title     = {{S}tructure of {O}ptimum {R}eceiving {F}ilters in {D}ata
          {T}ransmission {S}ystems},
  journal   = inf,
  volume    = {IT-17},
  pages     = {352-353},
  month     = may,
  year      = 1971
}

@Manual{      etsi98,
  title     = {"Tdoc SMG2 WPB 325/98," ETSI, Nov.~1998}
}

@InProceedings{   eyu:86,
  author    = {Eyubo\v{g}lu, M.V. and Qureshi, S.U.},
  title     = {{Reduced State Sequence Estimation with Set Partioning and
          Decision Feedback}},
  booktitle = {Proceedings of the IEEE Global Telecommunication
          Conference (GLOBECOM'86)},
  address   = {Houston},
  pages     = {1023-1028},
  year      = 1986
}

@Article{     Eyu88,
  author    = {Eyubo\v{g}lu, M.V. and Qureshi, S.U.},
  title     = {Reduced--state sequence estimation with set partitioning
          and decision feedback},
  journal   = com,
  volume    = {COM-36},
  pages     = {13-20},
  month     = jan,
  year      = 1988
}

@Article{     Eyu88a,
  author    = {M.V.~Eyubo\v{g}lu},
  title     = {{D}etection of {C}oded {M}odulation {S}ignals on {L}inear,
          {S}everely {D}istorted {C}hannels {U}sing
          {D}ecision-{F}eedback {N}oise {P}rediction with
          {I}nterleaving},
  journal   = com,
  volume    = {COM-36},
  pages     = {401-409},
  month     = apr,
  year      = 1988
}

@Article{     Eyu89,
  author    = {M.V. Eyubo\v{g}lu and S.U. Qureshi},
  title     = {Reduced--state sequence estimation for coded modulation on
          intersymbol interference channels},
  journal   = sel,
  volume    = {SAC-7},
  pages     = {989-995},
  month     = aug,
  year      = 1989
}

@Article{     eyu:92,
  author    = {M.V. Eyubo\v{g}lu and G.D. {Forney, Jr.}},
  title     = {{T}rellis {P}recoding: {C}ombined {C}oding, {P}recoding
          and {S}haping for {I}ntersymbol {I}nterference {C}hannels},
  journal   = inf,
  volume    = {IT-38},
  pages     = {301-314},
  month     = mar,
  year      = {1992}
}

@Article{     Fal91,
  author    = {A.~Falahati and B.~Woodward and S.~C.~Bateman},
  title     = {{Underwater Acoustic Channel Models For 4800 b/s QDPSK Signals}},
  journal   = {{IEEE Journal of Oceanic Engineering}},
  volume    = {16},
  pages     = {12-20},
  month     = jan,
  year      = 1991
}

@Article{     Fal73,
  author    = {D.~D.~Falconer and F.~R.~Magee, Jr.},
  title     = {{Adaptive Channel Memory Truncation for Maximum--Likelihood Sequence Estimation}},
  journal   = {{Bell Syst.~Tech.~Journal}},
  volume    = {52},
  pages     = {1541-1562},
  month     = nov,
  year      = 1973
}

@Book{        fano:61,
  author    = {R.M. Fano},
  title     = {Transmission of Information. {D}eutsche {"U}bersetzung:
          {I}nformations{"u}bertragung},
  publisher = {Oldenbourg},
  address   = {M\"unchen, Wien},
  year      = 1961
}

@Article{     fano:63,
  author    = {Fano, R.M.},
  title     = {A heuristic discussion of probabilistic coding},
  journal   = inf,
  volume    = {IT-9},
  pages     = {64-74},
  year      = 1963
}

@Book{        fano:66,
  author    = {R.M. Fano},
  title     = {Informations"ubertragung --- Eine statistische Theorie der
          Nachrichten"ubertragung},
  publisher = old,
  address   = {M"unchen Wien},
  year      = {1966}
}

@Article{     FFLV01,
  author    = {{F.R.~Farrokhi and G.J.~Foschini and A.~Lozano and R.A.~Valenzuela}},
  title     = {{Link-Optimal Space-Time Processing with Multiple Transmit and Receive Antennas}},
  journal   = {{IEEE Communictions Letters}},
  volume    = {5},
  pages     = {85-87},
  month     = mar,
  year      = 2001
}

@InProceedings{   fazel:93,
  author    = {K. Fazel and M. J. Ruf},
  title     = {{C}ombined multilevel coding and multiresolution
          modulation},
  booktitle = {Proceedings of the International Conference on
          Communications ({ICC}'93)},
  note      = {Conf. Record},
  pages     = {1081-1085},
  adrress   = {Geneva},
  month     = may,
  year      = 1993
}

@Article{     fettweis:89,
  author    = {Fettweis, G. and Meyr, H.},
  title     = {Parallel Viterbi Algorithm Implementation: Breaking the
          {ACS}--Bottleneck},
  journal   = com,
  volume    = {COM-37},
  pages     = {785-790},
  month     = {},
  year      = 1989
}

@Book{        fettweis:90,
  author    = {A. Fettweis},
  title     = {{E}lemente nachrichtentechnischer {S}ysteme},
  publisher = teu,
  address   = {Stuttgart},
  year      = 1990
}

@Book{        fi:96,
  author    = {R. Fischer},
  title     = {{M}ehrkanal- und {M}ehrtr\"agerverfahren f\"ur die
          schnelle digitale {\"U}bertragung im
          {O}rtsanschlu{\ss}leitungsnetz},
  publisher = {Shaker Verlag},
  address   = {Aachen},
  year      = 1997
}

@Article{     figehu:94,
  author    = {R.~Fischer and W.~Gerstacker and J.~Huber},
  title     = {{D}ynamics {L}imited {P}recoding, {S}haping, and {B}lind
          {E}qualization for {F}ast {D}igital {T}ransmission over
          {T}wisted {P}air {L}ines},
  journal   = sel,
  volume    = {SAC-13},
  pages     = {1622-1633},
  month     = dec,
  year      = 1995
}

@TechReport{      figehuschr:95,
  author    = {R.~Fischer and W.~Gerstacker and J.~Huber and P.~Schramm},
  title     = {{E}ntzerrung von {I}mpulsinterferenzen infolge
          {M}ehrwegeausbreitung beim {M}obilfunk nach dem
          {GSM}-{S}tandard mittels zustandsreduzierter
          {S}equenzsch\"atzung},
  institution   = {Lehrstuhl f\"ur Nachrichtentechnik, Universit\"at
          Erlangen-N\"urnberg},
  type      = {Research Report},
  note      = {(in German)},
  year      = 1995
}

@InProceedings{   fihu:94,
  author    = {R.~Fischer and J.~Huber},
  title     = {{D}ynamics {L}imited {S}haping for {F}ast {D}igital
          {T}ransmission},
  booktitle = {Proceedings of the International Conference on
          Communications ({ICC}'95)},
  pages     = {22-26},
  address   = {Seattle},
  month     = jun,
  year      = 1995
}

@InProceedings{   fihu:94b,
  author    = {R.~Fischer and J.~Huber},
  title     = {{S}ignalformung zur {B}egrenzung der {D}ynamik bei der
          {T}omlinson--{H}arashima--{V}orcodierung},
  booktitle = {ITG--Fachbericht 130},
  note      = {Codierung f\"ur Quelle, Kanal und \"Ubertragung},
  publisher = {VDE--Verlag},
  pages     = {457-466},
  year      = 1994
}

@Book{        fihu:94c,
  author    = {R.~Fischer and J.~Huber},
  title     = {{Erh\"ohung der St\"orresistenz bei der schnellen
          digitalen \"Ubertragung \"uber Ortsanschlu\ss leitungen
          (HDSL) durch koordinierte Mehrfach--Duplex \"Ubertragung}},
  publisher = {Forschungsbericht f\"ur die Deutsche Telekom AG, Lehrstuhl
          f\"ur Nachrichtentechnik der Universit\"at
          Erlangen-N\"urnberg},
  month     = mar,
  year      = 1994
}

@InProceedings{   fihu:96,
  author    = {R. Fischer and J. Huber},
  title     = {{A} {N}ew {L}oading {A}lgorithm for {D}iscrete {M}ultitone
          {T}ransmission},
  booktitle = {Proceedings of the IEEE Global Telecommunication
          Conference (GLOBECOM'96)},
  address   = {London},
  pages     = {724-728},
  month     = nov,
  year      = 1996
}

@Article{     fihu:97a,
  author    = {R. Fischer and J. Huber},
  title     = {{F}inite--{W}ord--{L}ength and {N}onrecursive
          {I}mplementation of {T}omlinson--{H}arashima {P}recoding},
  journal   = {International Journal of Electronics and Communications
          (AE\"U)},
  volume    = {51},
  pages     = {187-195},
  number    = {4},
  year      = {1997}
}

@InProceedings{   fihu:97b,
  author    = {R. Fischer and J. Huber},
  title     = {{O}n {T}he {E}quivalence of {S}ingle- and {M}ulticarrier
          {M}odulation: {A} {N}ew {V}iew},
  booktitle = {International Symposium on Information Theory (ISIT'97)},
  address   = {Ulm},
  note      = {Accepted for presentation},
  year      = 1997
}

@InProceedings{   fijalkow:94,
  author    = {I.~Fijalkow and F.~{{L}opez de {V}ictoria} and
          C.R.~{Johnson, Jr.}},
  title     = {{A}daptive {F}ractionally {S}paced {B}lind
          {E}qualization},
  booktitle = {Proceedings of IEEE DSP Workshop},
  pages     = {257-260},
  address   = {Yosemite NP},
  year      = 1994
}

@InProceedings{   fijalkow:95,
  author    = {I.~Fijalkow and J.R.~Treichler and C.R.~{Johnson, Jr.}},
  title     = {{F}ractionally {S}paced {B}lind {E}qualization: {L}oss of
          {C}hannel {D}isparity},
  booktitle = {Proceedings of ICASSP'95},
  pages     = {1988-1991},
  month     = may,
  address   = {Detroit},
  year      = 1995
}

@InProceedings{   fink:79,
  author    = {A.J. Vinck},
  title     = {On the implementation of a reduced state Viterbi decoder},
  booktitle = {Kurzfassungen zum 4. Aachener Kolloquium},
  pages     = {116-117},
  month     = {},
  year      = 1981
}

@InProceedings{   Foe02,
  author    = {J.R.~Foerster},
  title     = {{Interference Modeling of Pulse-based UWB Waveforms on Narrowband Systems}},
  booktitle = {Proceedings of IEEE Vehicular Technology Conference (VTC)},
  address   = {Birmingham, Al.},
  pages     = {1931-1935},
  month     = may,
  year      = 2002
}

@Article{     forney:70,
  author    = {G.D. {Forney, Jr.}},
  title     = {Convolutional Codes {I}: Algebraic Structure},
  journal   = inf,
  volume    = {IT-16},
  pages     = {720-738},
  month     = nov,
  year      = 1970
}

@Article{     forney:71,
  author    = {G.D. {Forney, Jr.}},
  title     = {{B}urst--{C}orrecting {C}odes for the {C}lassical {B}ursty
          {C}hannel},
  journal   = com,
  volume    = {COM-19},
  pages     = {772-781},
  month     = may,
  year      = {1971}
}

@Article{     For72,
  author    = {G.D. {Forney, Jr.}},
  title     = {{M}aximum--{L}ikelihood {S}equence {E}stimation of
          {D}igital {S}equences in the {P}resence of {I}ntersymbol
          {I}nterference},
  journal   = inf,
  volume    = {18},
  pages     = {363-378},
  year      = 1972
}

@Article{     forney:72b,
  author    = {G.D. {Forney, Jr.}},
  title     = {{L}ower {B}ounds on {E}rror {P}robability in the
          {P}resence of {L}arge {I}ntersymbol {I}nterference},
  journal   = com,
  volume    = {COM-20},
  pages     = {76-78},
  month     = feb,
  year      = 1972
}

@Article{     For73,
  author    = {Forney, Jr., G.D.},
  title     = {The {V}iterbi {A}lgorithm},
  journal   = {IEEE Proceedings},
  volume    = {61},
  pages     = {268-278},
  year      = 1973
}

@Article{     forney:73b,
  author    = {G.D. {Forney, Jr.}},
  title     = {Structural Analysis of Convolutional Codes via Dual
          Codes},
  journal   = inf,
  volume    = {IT-19},
  pages     = {512-518},
  year      = 1973
}

@Article{     forney:74,
  author    = {Forney, Jr., G.D.},
  title     = {Convolutional codes {III}: Sequential decoding},
  journal   = {Information and Control},
  volume    = {25},
  pages     = {267-297},
  year      = 1974
}

@Article{     forney:84,
  author    = {G.D. {Forney, Jr.} and R.G. Gallager and G.R. Lang and
          F.M. Longstaff and S.U. Qureshi},
  title     = {Efficient modulation for band--limited channels},
  journal   = {IEEE J. Select. Areas Commun.},
  volume    = {SAC-2},
  pages     = {632-647},
  year      = 1984
}

@Article{     forney:88a,
  author    = {G.D. {Forney, Jr.}},
  title     = {{Coset codes -- Part {I}: Introduction and geometrical
          classification}},
  journal   = inf,
  volume    = {IT-34},
  pages     = {1123-1151},
  month     = sep,
  year      = 1988
}

@Article{     forney:88b,
  author    = {G.D. {Forney, Jr.}},
  title     = {{Coset codes -- Part {II}: Binary Lattices and Related
          Codes}},
  journal   = inf,
  volume    = {IT-34},
  pages     = {1152-1187},
  month     = sep,
  year      = 1988
}

@Article{     forney:89a,
  author    = {G.D. {Forney, Jr.} and L.-F. Wei},
  title     = {{Multidimensional Constellations---Part {I}: Introduction,
          Figures of Merit, and Generalized Cross Constellations}},
  journal   = sel,
  volume    = {SAC-7},
  pages     = {877-892},
  month     = aug,
  year      = 1989
}

@Article{     forney:89b,
  author    = {G.D. {Forney, Jr.}},
  title     = {{Multidimensional Constellations---Part {II}: Voronoi
          Constellations}},
  journal   = sel,
  volume    = {SAC-7},
  pages     = {941-958},
  month     = aug,
  year      = 1989
}

@Article{     forney:90,
  author    = {J.M.~Cioffi and G.P.~Dudevoir and M.V~Eyuboglu and
          G.D.~{Forney, Jr.}},
  title     = {{MMSE} {D}ecision-{F}eedback {E}qualization and
          {C}oding---Part {I}: {G}eneral {R}esults},
  journal   = com,
  year      = {to appear}
}

@Article{     forney:92,
  author    = {G.D. {Forney, Jr.} and M.V. Eyubo\v{g}lu},
  title     = {{C}ombined {E}qualization and {C}oding Using {P}recoding},
  journal   = cma,
  volume    = {29},
  month     = dec,
  year      = 1991
}

@Article{     forney:95,
  author    = {J.~Cioffi and G.~Dudevoir and M.~Eyuboglu and
          G.~D.~{Forney, Jr.}},
  title     = {{MMSE} {D}ecision-{F}eedback {E}qualizers and {C}oding --
          {P}arts {I} and {II}},
  journal   = com,
  volume    = {COM-43},
  pages     = {2582-2604},
  month     = oct,
  year      = 1995
}

@Book{        fraleigh:76,
  author    = {J.B. Fraleigh},
  title     = {A First Course in Abstract Algebra},
  publisher = {Addison Wesley},
  address   = {Reading, Mass.},
  edition   = {second},
  year      = 1976
}

@Book{        franks:69,
  author    = {L.E. Franks},
  title     = {Signal Theory},
  publisher = {Prentice--Hall},
  address   = {Englewood Cliffs, NJ},
  year      = 1969
}

@Article{     franks:80,
  author    = {L.E. Franks},
  title     = {Carrier and Bit Synchronization in Data Communication--A
          Tutorial Review},
  journal   = com,
  pages     = {1107--1121},
  volume    = {COM--28},
  number    = {NO.8},
  month     = aug,
  year      = 1980
}

@InProceedings{   friedrichs:89,
  author    = {K.-J. Friedrichs and K.D. Kahn},
  title     = {Modulation Matched Coding for Microwave Digital Radio},
  booktitle = {{ITG}--Fachbericht 107},
  pages     = {271-276},
  month     = apr,
  year      = 1989
}

@Book{        fritz:79,
  author    = {F.J. {Fritz, B. Huppert, W. Willems}},
  title     = {{S}tochastische {M}atrizen},
  publisher = {Springer--Verlag},
  address   = {Berlin},
  year      = {1979}
}

@Book{        furrer:81,
  author    = {F.J. Furrer},
  title     = {{F}ehlerkorrigierende {B}lock--{C}odierung f"ur die
          {D}aten"ubertragung},
  publisher = {Birkh"auser Verlag},
  address   = {Basel, Switzerland},
  year      = 1981
}

@Article{     FMMO99,
  author    = {A.~Furusk\"ar and S.~Mazur and F.~M\"uller and H.~Olofsson},
  title     = {{EDGE: Enhanced Data Rates for GSM and TDMA/136 Evolution}},
  journal   = {IEEE Personal Communications Magazine},
  pages     = {56-66},
  volume    = {},
  number    = {},
  month     = jun,
  year      = 1999
}

@Article{     Gag97,
  author    = {M.~Gagnaire},
  title     = {{An Overview of Broad--Band Access Technologies}},
  journal   = {Proceedings of the {IEEE}},
  volume    = {85},
  number    = {12},
  pages     = {1958-1972},
  month     = dec,
  year      = 1997
}

@Book{        galiardi:84,
  author    = {R.M. Gagliardi},
  title     = {Satellite Communication},
  publisher = {Van Nostrand Reinhold},
  address   = {New York},
  year      = 1984
}

@Article{     galko:81,
  author    = {P. Galko and S. Pasupathy},
  title     = {The mean power spectral density of Markov chain driven
          signals},
  journal   = inf,
  volume    = {IT-11},
  pages     = {3-18},
  month     = {},
  year      = {1981}
}

@Book{        gallager:68,
  author    = {Robert G. Gallager},
  title     = {Information Theory and Reliable Communication},
  publisher = {John Wiley \& Sons, Inc.},
  address   = {New York},
  year      = 1968
}

@InProceedings{   GA03,
  author    = {H.~{El Gamal} and Aktas},
  title     = {{Distributed Space--Time Filtering for Cooperative Wireless Networks}},
  booktitle = {Proceedings of the IEEE Global Telecommunication
          Conference (GLOBECOM)},
  address   = {San Francisco},
  pages     = {1826-1830},
  year      = 2003
}

@Book{        gantmacher:59,
  author    = {Gantmacher, F.R.},
  title     = {The Theory of Matrices},
  publisher = {Chelsea Publishing Co.},
  address   = {New York},
  year      = {1959}
}

@Article{     gard:75,
  author    = {W.A. Gardner and L.E. Franks},
  title     = {Characterization of cyclostationary random signal
          processes},
  journal   = inf,
  volume    = {IT-21},
  pages     = {4-14},
  month     = {},
  year      = 1975
}

@Article{     gardner:91,
  author    = {W.~Gardner},
  title     = {{A new method of channel identification}},
  journal   = com,
  volume    = {COM-39},
  pages     = {813-817},
  month     = jun,
  year      = 1991
}

@Article{     ge:96,
  author    = {W.~Gerstacker},
  title     = {{A}n {A}lternative {A}pproach to {M}inimum
          {M}ean-{S}quared {E}rror {DFE} with {F}inite {L}ength
          {C}onstraints},
  journal   = {International Journal of Electronics and Communications
          (AE\"U)},
  volume    = {50},
  pages     = {27-31},
  number    = {1},
  year      = 1996
}

@InProceedings{   gefihu:94,
  author    = {W.~Gerstacker and R.~Fischer and J.~Huber},
  title     = {{B}lind {E}qualization for {D}igital {C}able
          {T}ransmission with {T}omlinson-{H}arashima {P}recoding and
          {S}haping},
  booktitle = {Proceedings of the International Conference on
          Communications ({ICC}'95)},
  pages     = {493-497},
  address   = {Seattle},
  month     = jun,
  year      = 1995
}

@InProceedings{   gefihu:97a,
  author    = {W. Gerstacker and R. Fischer and J. Huber},
  title     = {{A} {T}ransmission {S}cheme for {T}wisted {P}air {L}ines
          with {C}oding, {P}recoding, and {B}lind {E}qualization},
  booktitle = {Proceedings of the IEEE Global Telecommunication
          Conference (GLOBECOM'97)},
  pages     = {52-56},
  address   = {Phoenix},
  year      = 1997
}

@InProceedings{   gefihu:98,
  author    = {W.~Gerstacker and R.~Fischer and J.~Huber},
  title     = {{Blinde Entzerrung f\"ur digitale \"Ubertragung \"uber
          Zweidrahtleitungen mit Codierung und Vorcodierung}},
  booktitle = {ITG--Fachbericht 146, Codierung f\"ur Quelle, Kanal und
          \"Ubertragung},
  publisher = {VDE--Verlag},
  pages     = {239-244},
  year      = 1998
}

@InProceedings{   GH96,
  author    = {W.~Gerstacker and J.~Huber},
  title     = {{I}mproved {E}qualization for {GSM} {M}obile
          {C}ommunications},
  booktitle = {Proceedings of International Conference on Telecommunications (ICT)},
  address   = {Istanbul},
  month     = apr,
  year      = 1996
}

@InProceedings{   gehu:96b,
  author    = {W.~Gerstacker and J.~Huber},
  title = {{M}aximum {SNR} {D}ecision-{F}eedback {E}qualization with
          {FIR} {F}ilters: {F}ilter {O}ptimization and a {S}ignal
          {P}rocessing {A}pplication},
  booktitle = {Proceedings of the International Conference on
          Communications ({ICC}'96)},
  pages     = {1188-1192},
  address   = {Dallas},
  month     = jun,
  year      = 1996
}

@InProceedings{   Ger98,
  author    = {W.~Gerstacker and R.~Schober and J.~Huber},
  title     = {{N}oncoherent {E}qualization {A}lgorithms {B}ased on
          {S}equence {E}stimation},
  booktitle = {Proceedings of Globecom'98},
  address   = {Sydney},
  month = nov,
  year  = 1998
}

@Article{     GS02,
  author    = {W.~H.~Gerstacker and R.~Schober},
  title     = {{Equalization Concepts for EDGE}},
  journal   = {IEEE Transactions on Wireless Communications},
  volume    = {1},
  pages = {190-199},
  month = jan,
  year  = 2002
}

@Article{     Ger01,
  author    = {W.H.~Gerstacker and F.~Obernosterer and R.~Schober and A.~Lehmann and A.~Lampe and P.~Gunreben},
  title = {{Receiver Concepts for Space--Time Block--Coded Transmission over Frequency--Selective Fading Channels}},
  journal   = {In Revision: IEEE Transactions on Communications},
  volume    = {},
  pages = {},
  month = {},
  year  = 2002
}

@InProceedings{   GOS02,
  author    = {W.H.~Gerstacker and F.~Obernosterer and R.~Schober and A.~Lehmann and A.~Lampe
and P.~Gunreben},
  title     = {{Symbol--by--Symbol and Trellis--Based Equalization with Widely Linear Processing for Space--Time Block--Coded Transmission over Frequency Selective Channels}},
  booktitle = {Proceedings of the IEEE Global Telecommunications Conference (GLOBECOM)},
  pages     = {365-369},
  month     = dec,
  address   = {Taipei, Taiwan},
  year      = 2002
}

@InProceedings{   giannakis:95,
  author    = {G.B.~Giannakis and S.D.~Halford},
  title     = {{B}lind {F}ractionally--{S}paced {E}qualization of {N}oisy
          {FIR} {C}hannels: {A}daptive and {O}ptimal {S}olutions},
  booktitle = {Proceedings of ICASSP'95},
  pages     = {1972-1975},
  month     = may,
  address   = {Detroit},
  year      = 1995
}

@Article{     ginzburg:84,
  author    = {V.V. Ginzburg},
  title     = {Multidimensional Signals for a Continuous Channel},
  journal   = {Probl. Inf. Transmission},
  volume    = {23},
  pages     = {20-34},
  note      = {({T}ranslation from {P}robl. {P}eredachi {I}nf., pp.28-46,
          1984)},
  year      = 1984
}

@Article{     gitlin:79,
  author    = {R.D.~Gitlin and S.B.~Weinstein},
  title     = {{O}n the {R}equired {T}ap--{W}eight {P}recision for
          {D}igitally {I}mplemented, {A}daptive, {M}ean--{S}quared
          {E}qualizers},
  journal   = {Bell Syst. Tech. J.},
  volume    = {58},
  pages     = {301-321},
  month     = feb,
  year      = 1979
}

@Article{     gitlin:81,
  author    = {R.D.~Gitlin and S.B.~Weinstein},
  title     = {{F}ractionally--{S}paced {E}qualization: {A}n {I}mproved
          {D}igital {T}ransversal {E}qualizer},
  journal   = {Bell Syst. Tech. J.},
  volume    = {60},
  pages     = {275-296},
  month     = feb,
  year      = 1981
}

@Article{     GM05,
  author    = {R.~Giuliano and F.~Mazzenga},
  title     = {{On the Coexistence of Power Controlled Ultrawide-Band Systems with UMTS, GPS, DCS1800, and Fixed Wireless Systems}},
  journal   = veh,
  volume    = {VT-54},
  pages     = {62-81},
  month     = jan,
  year      = 2005
}


@InProceedings{   glauner:86,
  author    = {M. Glauner and S. Rasmussen and H. Wetzel},
  title     = {Simulation Program {SIM}: Structure and Application to
          Fixed and Mobile Digital Satellite Channels},
  booktitle = {Proceedings of the {ICDSC}'86},
  address   = {Munich},
  pages     = {611-618},
  year      = 1986
}

@Article{     godard:80,
  author    = {D.N.~Godard},
  title     = {{S}elf--{R}ecovering {E}qualization and {C}arrier
          {T}racking in {T}wo--{D}imensional {D}ata {C}ommunication
          {S}ystems},
  journal   = com,
  volume    = {COM-28},
  pages     = {1867-1875},
  month     = nov,
  year      = 1980
}

@Article{     goldfeld:95,
  author    = {L.~Goldfeld and D.~Wulich},
  title     = {{A calculation of the capacity of a twisted--wire pair}},
  journal   = {Elsevier Signal Processing},
  volume    = {41},
  pages     = {391-393},
  year      = 1995
}

@Article{     GL00,
  author    = {Y.~Gong and K.B.~Letaief},
  title     = {{Performance Evaluation and Analysis of Space--Time Coding in Unequalized Multipath Fading Links}},
  journal   = com,
  volume    = {COM-48},
  pages     = {1778-1782},
  month     = nov,
  year      = 2000
}

@InProceedings{  GSP02,
  author    = {D.~Gore and S.~Sandhu and A.~Paulraj},
  title     = {{Delay Diversity Codes for Frequency Selective Channels}},
  booktitle = {Proceedings of the IEEE Inter.~Conf.~Commun.~(ICC)},
  address   = {New York},
  pages     = {1949-1953},
  month     = may,
  year      = 2002
}

@Book{        Gra65,
  author    = {I.~S.~Gradshteyn and I.~M~.Ryzhik},
  title     = {{T}able of {I}ntegrals, {S}eries, and {P}roducts},
  publisher = {Academic {P}ress},
  address   = {New York},
  year      = 1965
}

@Book{        graf:90,
  author    = {K. Graf},
  title     = {{N}ahezu optimale, adaptive {E}mpf"anger f"ur digitale
          {B}asisbandsysteme},
  publisher = {Dissertation, Universit"at der Bundeswehr M"unchen,
          Fakult"at f"ur Elektrotechnik},
  year      = 1990
}

@Article{     graf:90a,
  author    = {K. {Graf, J. Huber, K. Tr"ondle}},
  title     = {{D}igitale {B}asisband"ubertragung "uber
          {B}andpa\3kan"ale},
  journal   = {Frequenz},
  volume    = {Band 44},
  pages     = {S.42-51},
  month     = feb,
  year      = 1990
}

@InProceedings{   grafhu:89,
  author    = {K.P.~Graf and J.~Huber},
  title     = {{D}esign and {P}erformance of an {A}ll-{D}igital
          {A}daptive 2.048 {M}bit/s {D}ata {T}ransmission {S}ystem
          {U}sing {N}oise {P}rediction},
  booktitle = {Proceedings of the International Symposium on Circuits and
          Systems ({ISCAS}'89)},
  pages     = {1808-1812},
  year      = 1989
}

@Article{     greenstein:97a,
  author    = {S.~Ariyavisitakul and L.J.~Greenstein},
  title     = {{R}educed-{C}omplexity {E}qualization {T}echniques for
          {B}roadband {W}ireless {C}hannels},
  journal   = sel,
  volume    = {SAC-15},
  pages     = {5-15},
  month     = jan,
  year      = 1997
}

@InProceedings{   greenstein:97b,
  author    = {S.~Ariyavisitakul and N.R.~Sollenberger and
          L.J.~Greenstein},
  title     = {{T}ap-{S}electable {D}ecision {F}eedback {E}qualization},
  booktitle = {Proceedings of the International Conference on
          Communications ({ICC}'97)},
  address   = {Montreal},
  month     = jun,
  year      = 1997
}

@Book{        gregg:77,
  author    = {W.D. Gregg},
  title     = {Analog and Digital Communication},
  publisher = wil,
  address   = {New York},
  year      = 1977
}

@Article{     grettenberg:65,
  author    = {T.L. Grettenberg},
  title     = {A representation theorem for complex normal processes},
  journal   = inf,
  volume    = {IT-11},
  pages     = {305-306},
  year      = 1965
}

@Manual{      gsmrec,
  title     = {{ETSI}/{GSM} {R}ecommendations {S}eries 05: ``{P}hysical
          {L}ayer on the {R}adio {P}ath''}
}

@Manual{      GSM,
  title     = {{GSM} {R}ecommendation 05.05: ``{P}ropagation {C}onditions'', {V}ers.~5.3.0, {R}elease 1996}}
}

@InProceedings{   gu:94,
  author    = {Y.-M.~Gu and B.-S.~Seo and Ch.-W.~Lee},
  title     = {{C}onvergence {A}nalysis of {S}ato {B}lind {E}qualizer
          with {D}iscrete {C}hannel {I}nput},
  booktitle = {Proceedings of the International Symposium on Information
          Theory (ISIT'94)},
  address   = {Trondheim},
  month     = jun # "/"  # jul,
  page      = {355},
  year      = 1994
}

@Article{     guba:95,
  author    = {W.~Guba},
  title     = {{HDSL--Mehrpaarsysteme im technischen und wirtschaftlichen
          Vergleich}},
  journal   = ntz,
  number    = {4},
  pages     = {36-41},
  year      = 1995
}

@InProceedings{   GFBK96,
  author    = {J.--C.~Guey and M.P.~Fitz and M.R.~Bell and W.--Y.~Kuo},
  title     = {{Signal Design for Transmitter Diversity Wireless Communication Systems Over Rayleigh Fading Channels}},
  booktitle = {Proceedings of IEEE Veh.~Technol.~Conf.},
  address   = {Atlanta},
  month     = {},
  pages     = {136-140},
  year      = 1996
}

@Article{     GFBK99,
  author    = {J.--C.~Guey and M.P.~Fitz and M.R.~Bell and W.--Y.~Kuo},
  title     = {{Signal Design for Transmitter Diversity Wireless Communication Systems Over Rayleigh Fading Channels}},
  journal   = com,
  volume    = {47},
  pages     = {527-537},
  month     = apr,
  year      = 1999
}

@Article{     haensler:71,
  author    = {E.~H{\"a}nsler},
  title     = {{S}ome {P}roperties of {T}ransmission {S}ystems with
          {M}inimum {M}ean-{S}quare {E}rror},
  journal   = com,
  volume    = {COM-19},
  pages     = {576-579},
  month     = aug,
  year      = 1971
}

@Book{        haensler:83,
  author    = {E. H"ansler},
  title     = {{G}rundlagen der {T}heorie statistischer {S}ignale},
  publisher = spr,
  address   = {Berlin},
  year      = 1983
}

@InProceedings{   hag:80,
  author    = {J. Hagenauer},
  title     = {Viterbi Decoding of Convolutional Codes for Fading and
          Burst--Channels},
  booktitle = {Proc. of the 1980 Zurich Seminar},
  year      = 1980
}

@Article{     hag:88,
  author    = {J. Hagenauer},
  title     = {Rate--Compatible Punctured Convolutional Codes ({RCPC}
          Codes) and their Applications},
  journal   = com,
  volume    = {COM-36},
  pages     = {389-400},
  month     = apr,
  year      = 1988
}

@Article{     hag:90,
  author    = {J. Hagenauer and N. Seshadri and C.-E. Sundberg},
  title     = {The Performance of Rate--Compatile Punctured Convolutional
          Codes for Digital Mobile Radio},
  journal   = com,
  volume    = {COM-38},
  pages     = {966-980},
  month     = jul,
  year      = 1990
}

@Article{     hag:90b,
  author    = {C.-E. Sundberg and J. Hagenauer},
  title     = {Hybrid Trellis--Coded 8/4--{PSK} Modulation Systems},
  journal   = com,
  volume    = {COM-38},
  pages     = {602-614},
  month     = may,
  year      = 1990
}

@Article{     hagenauer:88,
  author    = {J. Hagenauer and C.E. Sundberg},
  title     = {On the Performance Evaluation of Trellis-Coded 8PSK
          Systems with Carrier Phase Offset},
  journal   = { Electronics and Communications AEUE},
  volume    = {Bd.42},
  pages     = {274-284},
  year      = 1988
}

@Article{     Ham96,
  author    = {N.~Hamamoto},
  title     = {{D}ifferential {D}etection with {IIR} {F}ilter for {I}mproving {DPSK} {D}etection {P}erformance},
  journal   = com,
  volume    = {COM-44},
  pages     = {959-966},
  month     = aug,
  year      = 1996
}

@Article{     HS96,
  author    = {K.A.~Hamied and G.L.~St\"uber},
  title     = {{An Adaptive Truncated MLSE Receiver for Japanese Personal Digital Cellular}},
  journal   = veh,
  volume    = {45},
  pages     = {41-50},
  month     = feb,
  year      = 1996
}

@Book{        hanbueckers:89,
  author    = {L. Hanb"uckers},
  title     = {{N}achrichtentechnische {G}rundlagen zur {O}ptimierung
          eines {CPM}-{E}mpf"angers},
  publisher = {Diplomarbeit, Institut f"ur Nachrichtentechnik,
          Universit"at der Bundeswehr M"unchen},
  month     = dec,
  year      = 1989
}

@Article{     harashima:69,
  author    = {H.~Harashima and H.~Miyakawa},
  title     = {{M}atched-{T}ransmission {T}echnique for {C}hannels with
          {I}ntersymbol {I}nterference},
  journal   = com,
  volume    = {COM-20},
  pages     = {774-780},
  month     = aug,
  year      = 1972
}

@Article{     HH02,
  author    = {B.~Hassibi and B.M.~Hochwald},
  title     = {{Cayley Differential Unitary Space-Time Codes}},
  journal   = inf,
  volume    = {IT-48},
  pages     = {1485-1503},
  month     = jun,
  year      = 2002
}

@Article{     HH02a,
  author    = {B.~Hassibi and B.M.~Hochwald},
  title     = {{High-Rate Codes That Are Linear in Space and Time}},
  journal   = inf,
  volume    = {IT-48},
  pages     = {1804-1824},
  month     = jul,
  year      = 2002
}

@Article{     hatzinakos:91,
  author    = {D.~Hatzinakos and C.L.~Nikias},
  title     = {{B}lind {E}qualization {U}sing a {T}ricepstrum--{B}ased
          {A}lgorithm},
  journal   = com,
  volume    = {COM-39},
  pages     = {669-682},
  month     = may,
  year      = 1991
}

@Book{        hauser:95,
  author    = {T.~Hauser},
  title     = {{U}ntersuchung aufwandsg\"unstiger {E}ntzerrverfahren
          f\"ur den {M}obilfunk},
  publisher = {Studienarbeit (senior project), Lehrstuhl f\"ur
          Nachrichtentechnik, Universit\"at Erlangen-N\"urnberg},
  month     = sep,
  note      = {(in German)},
  year      = 1995
}

@Book{        haykin:86,
  author    = {S.~Haykin},
  title     = {Adaptive Filter Theory},
  publisher = {Prentice-Hall},
  address   = {Englewood Cliffs, New Jersey},
  year      = 1986
}

@Book{        Hay88,
  author    = {S. Haykin},
  title     = {Digital Communication},
  publisher = {J. Wiley \& Sons},
  address   = {New York},
  year      = 1988
}

@InCollection{    haykin:94,
  author    = {S.~Bellini},
  title     = {{B}ussgang {T}echniques for {B}lind {D}econvolution and
          {E}qualization},
  booktitle = {{B}lind {D}econvolution},
  publisher = {Prentice Hall},
  year      = {1994},
  editor    = {S.~Haykin},
  pages     = {8-59},
  address   = {Englewood Cliffs, NJ}
}

@Book{        Hay96,
  author    = {S.~Haykin},
  title     = {Adaptive Filter Theory},
  publisher = {Prentice-Hall},
  address   = {Upper Saddle River, New Jersey, Third Edition},
  year      = 1996
}

@Book{        heinhold:76,
  author    = {J. Heinhold},
  title     = {{E}inf"uhrung in die {H}"ohere {M}athematik, {T}eil 1-4},
  publisher = {Carl Hanser Verlag},
  address   = {M"unchen, Wien},
  year      = 1976
}

@InProceedings{   HSP03,
  author    = {R.W.~{Heath Jr.} and T.~Strohmer and A.J.~Paulraj},
  title     = {Grassmannian Signatures for CDMA Systems},
  booktitle = {Proceedings of the Global Telecommunications Conference (GLOBECOM)},
  volume    = {},
  pages     = {1553-1557},
  address   = {San Francisco},
  month     = dec,
  year      = 2003
}

@Article{     heller:71,
  author    = {Heller, J.A. and Jacobs, I.M.},
  title     = {Viterbi Decoding for Satellite and Space Communication},
  journal   = {IEEE Transactions on Communication Technology},
  volume    = {COM-19},
  pages     = {835-848},
  month     = oct,
  year      = 1971
}

@Book{        helstrom:75,
  author    = {Carl W. Helstrom},
  title     = {Statistical Theory of Signal Detection},
  publisher = {Pergamon Press},
  address   = {Oxford},
  year      = 1975
}

@Unpublished{     herz:96,
  author    = {H. Herzberg},
  title     = {{M}ultilevel {T}urbo {C}oding with {S}hort
          {I}nterleavers},
  note      = {Submitted to IEEE Journal on Selected Areas in
          Communications},
  year      = 1996
}

@Article{     hill:77,
  author    = {Lee, W.U. and Hill, F.S.},
  title     = {A Maximum--Likekihood Sequence Estimator with Decision
          Feedback Equalization},
  journal   = com,
  volume    = {COM-25},
  pages     = {971-979},
  year      = 1977
}

@Article{     ho:86,
  author    = {P.K.M. Ho and P.J. McLane},
  title     = {Power spectral density of digital continuous phase
          modulation with correlated data symbols -- {P}art {I} +
          {II}},
  journal   = {IEE Proc.--F. Commun., Radar {\rm\&} Signal Process},
  volume    = {},
  pages     = {95-114},
  month     = {},
  year      = {1986}
}

@Article{     Ho92,
  author    = {P.~Ho and D.~Fung},
  title     = {Error {P}erformance of {M}ultiple--{S}ymbol
          {D}ifferential {D}etection of {PSK} {S}ignals {T}ransmitted {O}ver {C}orrelated {R}ayleigh {F}ading {C}hannels},
  journal   = com,
  volume    = {COM-40},
  pages     = {25-29},
  month     = oct,
  year      = 1992
}

@Article{     HS00,
  author    = {B.M.~Hochwald and W.~Sweldens},
  title     = {{Differential Unitary Space--Time Modulation}},
  journal   = com,
  volume    = {COM-48},
  pages     = {2041-2052},
  month     = dec,
  year      = 2000
}

@Article{     HM00,
  author    = {B.M.~Hochwald and T.L.~Marzetta},
  title     = {{Unitary Space-Time Modulation for Mutilple-Antenna Communications in Rayleigh Flat Fading}},
  journal   = inf,
  volume    = {IT-46},
  pages     = {543-564},
  month     = mar,
  year      = 2000
}

@Article{     HMRSU00,
  author    = {B.M.~Hochwald and T.L.~Marzetta and T.J.~Richardson and W.~Sweldens and R.~Urbanke},
  title     = {{Systematic Design of Unitary Space-Time Constellations}},
  journal   = inf,
  volume    = {IT-46},
  pages     = {1962-1973},
  month     = sep,
  year      = 2000
}

@Article{     hoege:76,
  author    = {H. H"oge},
  title     = {{B}erechnung der {F}ehlerwahrscheinlichkeit in
          regenerativen {S}ystemen mit quantisierter
          {R}"uckkopplung},
  journal   = {AE"U},
  volume    = {Band 30},
  number    = {Heft 3},
  pages     = {S.130-133},
  year      = 1976
}

@InProceedings{   hoeher:89,
  author    = {Hagenauer, J. and H\"oher, P.},
  title     = {{A} {V}iterbi {A}lgorithm with {S}oft-{D}ecision {O}utputs
          and its {A}pplications},
  booktitle = {Proceedings of the IEEE Global Telecommunication
          Conference ({GLOBECOM}'89)},
  address   = {Dallas},
  pages     = {47.1.1-47.1.7},
  year      = 1989
}

@Book{        hoeher:90,
  author    = {H"oher, P.},
  title     = {{K}oh"arenter {E}mpfang trelliscodierter {PSK}--{S}ignale
          auf fre\-quenz\-se\-lek\-tiven {M}obilfunkkan"alen ---
          {E}ntzerrung, {D}ecodierung und {K}analparametersch"atzung},
  publisher = {Dissertation, Universit"at Kaiserslautern},
  month     = jul,
  year      = 1990
}

@InProceedings{   hoeher:90b,
  author    = {H\"oher, P.},
  title     = {{TCM} on {F}requency-{S}elective {F}ading {C}hannels: A
          {C}omparison of {S}oft-{O}utput {P}robabilistic
          {E}qualizers},
  booktitle = {Proceedings of the IEEE Global Telecommunication
          Conference ({GLOBECOM'90})},
  pages     = {401.4.1.-401.4.6.},
  address   = {San Diego},
  month     = dec,
  year      = 1990
}

@InProceedings{   hoeher:90c,
  author    = {P. H\"oher},
  title     = {A Channel Estimator with Application to
          Frequency--Selective Fading Channels},
  booktitle = {Proceedings of the {EUSIPCO}'90},
  volume    = {},
  pages     = {},
  address   = {Barcelona},
  month     = sep,
  year      = 1990
}

@Book{        hoelzler:75,
  author    = {E. {H"olzler, H. Holzwarth}},
  title     = {{P}ulstechnik},
  note      = {B"ande {I} und {II}},
  publisher = spr,
  address   = {Berlin},
  year      = {1975, 1976}
}

@Article{     hon:92,
  author    = {M.L. Honig and P. Crespo and K. Steiglitz},
  title     = {Suppression of Near- and Far-End Crosstalk by Linear Pre-
          and Post-Filtering},
  journal   = sel,
  volume    = {SAC-10},
  pages     = {614-629},
  month     = apr,
  year      = {1992}
}

@Book{        honig:84,
  author    = {M.L. Honig and D.G. Messerschmidt},
  title     = {Adaptive filters: structures algorithms and applications},
  publisher = {Kluwer Academic Publishers},
  address   = {Boston},
  year      = 1984
}

@Book{        HJ99,
  author    = {R.A.~Horn and C.R.~Johnson},
  title     = {Matrix Analysis},
  publisher = {Cambridge University Press},
  address   = {Cambridge},
  year      = 1999
}

@Book{        hub:82,
  author    = {J. Huber},
  title     = {{C}odierung f"ur ged"achtnisbehaftete {K}an"ale},
  publisher = {Dissertation, Universit"at der Bundeswehr M"unchen},
  month     = {Juli},
  year      = 1982
}

@Article{     hub:83,
  author    = {J. Huber},
  title     = {{Z}ur {A}nwendung von {K}analmodellen f"ur
          {C}odierverfahren},
  journal   = {{NTG}--Fachberichte 84, {\rm S.51--59}},
  month     = mar,
  year      = 1983
}

@InProceedings{   hub:84,
  author    = {J. Huber and M. Oenol},
  title     = {On the Performance of a Hybrid Coding Scheme},
  booktitle = {Proceedings of the 1984 International Z"urich Seminar on
          Digital Communications},
  pages     = {107-111},
  month     = mar,
  year      = 1984
}

@Article{     hub:84a,
  author    = {J. Huber},
  title     = {{U}ntersuchung von {B}lockcodierverfahren bei
          ged"achtnisbehafteten {K}an"alen},
  journal   = {ntz--Archiv},
  volume    = {Bd.6},
  pages     = {S.233-241},
  year      = {1984}
}

@TechReport{      hub:85,
  author    = {J. {Huber, K.P. Graf, K. Tr"ondle}},
  title     = {{R}ealisierung eines 2.048
          {M}bit/sec--{D}igital"ubertragungssystems mit
          ged"achtnisbehaftetem {E}ntscheider f"ur symmetrische
          {K}abel zum {Z}weck der {F}eldl"angenerh"ohung},
  institution   = {Universit"at der Bundeswehr M"unchen},
  type      = {{B}ericht f"ur das {FI} der {DBP} beim {FTZ} {D}armstadt},
  address   = {Neubiberg},
  month     = jun,
  year      = 1985
}

@InProceedings{   hub:87a,
  author    = {J. Huber and W.L. Liu},
  title     = {Convolutional Codes for {CPM} using the Memory of the
          Modulation Process},
  booktitle = {GLOBECOM'87},
  note      = {Conf. Record, vol.3},
  pages     = {43.1.-43.1.5},
  adrress   = {Tokyo},
  year      = 1987
}

@InProceedings{   hub:87b,
  author    = {J. Huber and W.L. Liu},
  title     = {Reduced--State--Viterbi--Detection of {CPM} combined with
          Convolutional Codes},
  booktitle = {SITA'87},
  note      = {Conf. Record},
  pages     = {ED~2-2-1 -- ED~2-2-6},
  adrress   = {Enoshima, Japan},
  year      = 1987
}

@Article{     hub:87c,
  author    = {J. Huber},
  title     = {{D}etektoren und {O}ptimalfilter f"ur {D}igitalsignale mit
          {I}mpulsinterferenzen, {T}eil {I}: {O}ptimaldetektion und
          {W}hitened--{M}atched--{F}ilter},
  journal   = {Frequenz},
  volume    = {Band 41},
  pages     = {S.161-167},
  month     = {},
  year      = 1987
}

@Article{     hub:87d,
  author    = {J. Huber},
  title     = {{D}etektoren und {O}ptimalfilter f"ur {D}igitalsignale mit
          {I}mpulsinterferenzen, {T}eil {II}: {S}uboptimale
          {E}mpf"anger},
  journal   = {Frequenz},
  volume    = {Band 41},
  pages     = {S.189-196},
  year      = 1987
}

@Article{     hub:87e,
  author    = {J. Huber},
  title     = {{S}t\"orabstandsverlust durch {H}ochpa\ss filterung bei
          digitalen {B}asisband\"ubertragungssystemen mit
          {Q}uantisierter {R}\"uckkopplung},
  journal   = {Frequenz},
  volume    = {Band 41},
  pages     = {S.112-114},
  month     = may,
  year      = 1987
}

@Misc{        hub:88v,
  author    = {J. Huber},
  title     = {{V}ortrag beim {K}olloquium der {D}eutschen
          {F}orschungsgemeinschaft in {K}arlsruhe ({B}egr"undung
          eines {F}orschungsantrags)},
  month     = "26.~"  # may,
  year      = 1988
}

@InProceedings{   hub:89a,
  author    = {J. Huber and W.L. Liu},
  title     = {Complexity Reduction for Coherent {CPM} Receivers},
  booktitle = {ITG--Fachberichte 107},
  note      = {Conf. Record},
  pages     = {219-224},
  adrress   = {N"urnberg, FRG},
  month     = sep,
  year      = 1989
}

@InProceedings{   hub:89b,
  author    = {J. Huber and W.L. Liu},
  title     = {Concatenation of {RS}--Codes and {CPM}},
  booktitle = {Proceedings of the 1989 {URSI} International Symposium on
          Signals, Systems, and Electronics {\rm (ISSSE'89)}},
  pages     = {272-275},
  address   = {Erlangen},
  month     = sep,
  year      = 1989
}

@Article{     hub:89c,
  author    = {J. Huber and W.L. Liu},
  title     = {An Alternative Approach to Reduced--Complexity
          {CPM}--Receivers},
  journal   = {IEEE J. Select. Areas Commun.},
  volume    = {SAC-7},
  pages     = {1437-1449},
  month     = dec,
  year      = 1989
}

@Article{     hub:89e,
  author    = {J. Huber},
  title     = {{D}igitale {M}odelle zeitvarianter
          {"U}bertragungskan"ale},
  journal   = {Kleinheubacher Berichte des Forschungsinstituts der
          Deutschen Bundespost},
  volume    = {Band 32},
  pages     = {S.537-544},
  year      = 1989
}

@Article{     hub:90a,
  author    = {J. {Huber, A. R\"uppel}},
  title     = {{Z}uverl\"assigkeitssch\"atzung f\"ur die
          {A}usgangssymbole von {T}rellis--{D}ecodern},
  journal   = {AE\"U (Electronics and Communication)},
  volume    = {Bd. 44},
  pages     = {S.8-21},
  month     = {},
  note      = {(in German)},
  year      = 1990
}

@Article{     hub:90b,
  author    = {J. {Huber, W. Liu}},
  title     = {{K}oher"ante {D}igitalsignalempf"anger mit
          {S}ignalrepr"asentation durch spektrale {A}btastung},
  journal   = {Kleinheubacher Berichte des Forschungsinstitutes der
          Deutschen Bundespost},
  volume    = {Band 34},
  pages     = {S.369-382},
  year      = 1991
}

@Article{     hub:90c,
  author    = {J. Huber and W. Liu},
  title     = {Data--Aided Synchronization of Coherent {CPM}--Receivers},
  journal   = {IEEE Trans. on Commun.},
  volume    = {COM-40},
  pages     = {178-189},
  month     = jan,
  year      = 1992
}

@Book{        hub:91,
  author    = {J. Huber},
  title     = {{D}igitale {\"U}bertragungssysteme --- {M}ethoden der
          {T}relliscodierung},
  publisher = {Habilitationsschrift, Institut f\"ur Nachrichtentechnik
          der Universit\"at der Bundeswehr M\"unchen},
  address   = {M\"unchen},
  year      = {1991}
}

@Book{        hub:92,
  author    = {J. Huber},
  title     = {Trelliscodierung in der digitalen \"Ubertragungstechnik
          --- Grundlagen und Anwendungen},
  publisher = spr,
  address   = {Berlin},
  year      = {1992}
}

@InProceedings{   hub:93a,
  author    = {J. Huber},
  title     = {{D}istance-{G}ains by {M}ultiple-{D}uplex {T}ransmission,
          {C}oding and {S}haping for {H}{D}{S}{L}},
  booktitle = {Proceedings of the International Conference on
          Communications ({ICC}'93)},
  pages     = {1820-1824},
  adrress   = {Geneva},
  month     = may,
  year      = 1993
}

@Book{        hubdigue:97,
  author    = {J.~Huber},
  title     = {Skriptum zur Vorlesung Digitale "Ubertragung},
  publisher = {Lehrstuhl f"ur Nachrichtentechnik II},
  address   = {Universit"at Erlangen--N"urnberg},
  year      = {1997}
}

@Misc{        hubenn:95,
  author    = {J.~Huber and J.~Benndorf and H.~Volkers and R.~Hempel},
  title     = {{V}erfahren zur digitalen {N}achrichten\"ubertragung
          \"uber ein elektrisches {K}abel},
  howpublished  = {German Patent Application no.~195 45 473.1},
  month     = dec,
  year      = 1995
}

@Unpublished{     huber:?,
  author    = {J. Huber},
  title     = {{M}ultilevel {C}odes: {D}istance {P}rofiles and {C}hannel
          {C}apacity},
  note      = {{I}n preparation}
}

@Book{        hubinf:97,
  author    = {J.~Huber},
  title     = {Skriptum zur Vorlesung Informationstheorie},
  publisher = {Lehrstuhl f"ur Nachrichtentechnik II},
  address   = {Universit"at Erlangen--N"urnberg},
  year      = {1997}
}

@TechReport{      hubke:92,
  author    = {J.~Huber},
  title     = {{R}eichweitenerh\"ohung durch {K}analcodierung bei der
          digitalen \"{U}bertragung \"uber symmetrische {L}eitungen},
  institution   = {Lehrstuhl f\"ur Nachrichtentechnik, Universit\"at
          Erlangen-N\"urnberg},
  type      = {Research Report},
  note      = {(in German)},
  year      = 1992
}

@Article{     hubsp:88,
  author    = {J. {Huber, H. Beckmann}},
  title     = {{M}ittleres {L}eistungsspektrum ged"achtnisbehafteter
          digitaler {S}ignalquellen},
  journal   = {ntz--Archiv},
  volume    = {Bd.10},
  pages     = {S.45-54},
  month     = {},
  year      = {1988}
}

@Unpublished{     huwa:94,
  author    = {J. Huber and U. Wachsmann},
  title     = {{C}apacities of the {E}quivalent {C}hannels in
          {M}ultilevel {C}oding {S}chemes},
  note      = {Submitted to Electr. Letters}
}

@Article{     imai:77,
  author    = {H. Imai and S. Hirakawa},
  title     = {A new multilevel coding method using error correcting
          codes},
  journal   = inf,
  volume    = {IT-23},
  pages     = {371-377},
  month     = may,
  year      = 1977
}

@Article{     jacobs:67,
  author    = {Jacobs, I.M. and Berlekamp, E.R.},
  title     = {A lower bound to the distribution computation for
          sequential decoding},
  journal   = inf,
  volume    = {IT-13},
  pages     = {167-174},
  month     = apr,
  year      = 1967
}

@Article{     jag:78,
  author    = {{F. de} Jager and C.B. Dekker},
  title     = {Tamed Frequency Modulation, A Novel Method to Achieve
          Spektrum Economy in Digital Transmission},
  journal   = com,
  volume    = {COM-26},
  pages     = {534-542},
  month     = may,
  year      = 1978
}

@Article{     JHHN04,
  author    = {M.~Janani and A.~Hedayat and T.E.~Hunter and A.~Nosratinia},
  title     = {{Coded Cooperation in Wireless Communications: Space-Time Transmission and Iterative Decoding}},
  journal   = sip,
  volume    = {SP-52},
  pages     = {362-371},
  month     = feb,
  year      = 2004
}

@Book{        Jak74,
  author    = {W.~C.~Jakes, Jr., Ed.},
  title     = {Microwave {M}obile {C}ommunications},
  publisher = {Prentice--Hall},
  address   = {New Jersey},
  year      = 1974
}

@Article{     janssen:88,
  author    = {A.J.E.M.~Janssen},
  title     = {{The Zak Transform: A Signal Transform For Sampled
          Time--Continuous Signals}},
  journal   = {Philips J. Res.},
  volume    = {43},
  pages     = {23-69},
  number    = {1},
  year      = 1988
}

@Article{     jayant:78,
  author    = {Jayant, N.S. and Christenson, S.A.},
  title     = {Tree encoding of speech using the {(M,L)}-algorithm and
          adaptive quantization},
  journal   = com,
  volume    = {COM-26},
  pages     = {1376-1379},
  year      = 1978
}

@Article{     jelinek:69,
  author    = {Jelinek, F.},
  title     = {Fast sequential decoding algorithm using a stack},
  journal   = {IBM Journal of Research and Development},
  volume    = {13},
  pages     = {675-685},
  year      = 1969
}

@Article{     jelinek:71,
  author    = {Jelinek, F. and Anderson, J.B.},
  title     = {Instrumentable tree encoding of information sources},
  journal   = inf,
  volume    = {IT-17},
  pages     = {118-119},
  year      = 1971
}

@Book{        johannesson:92,
  author    = {R. Johannesson},
  title     = {{I}nformationstheorie --- {G}rundlage der
          ({T}ele-){K}ommunikation},
  publisher = {Addison-Wesley},
  address   = {Lund, Schweden},
  year      = 1988
}

@Article{     johnson:91,
  author    = {C.R.~{Johnson, Jr.}},
  title     = {{A}dmissibility in {B}lind {A}daptive {C}hannel
          {E}qualization},
  journal   = {IEEE Control Systems Magazine},
  volume    = {11},
  pages     = {3-15},
  month     = jan,
  year      = 1991
}

@Book{        jones:66,
  author    = {Jones, D.S.},
  title     = {Generalized Functions},
  publisher = {McGraw--Hill},
  address   = {New York},
  year      = {1966}
}

@Article{     JSO02,
  author    = {G.~Jongren and M.~Skoglund and B.~Ottersten},
  title     = {{Combining Beamforming and Orthogonal Space-Time Block Coding}},
  journal   = inf,
  volume    = {48},
  pages     = {611-627},
  month     = mar,
  year      = 2002
}

@Article{     Jun94,
  author    = {P.~Jung},
  title     = {{Laurent's Representation of Binary Continuous Phase Modulated Signals with Modulation Index $1/2$ Revisited}},
  journal   = com,
  volume    = {COM-42},
  pages     = {221-224},
  month     = {Feb/Mar/Apr},
  year      = 1994
}

@Article{     kalet:90,
  author    = {I.~Kalet and S.~Shamai (Shitz)},
  title     = {{O}n the {C}apacity of a {T}wisted--{W}ire {P}air:
          {G}aussian {M}odel},
  journal   = com,
  volume    = {COM-38},
  pages     = {379-383},
  month     = mar,
  year      = 1990
}

@InProceedings{   kamel:93,
  author    = {R.E.~Kamel and Y.~{Bar--Ness}},
  title     = {{B}lind {D}ecision {F}eedback {E}qualization {U}sing the
          {D}ecorrelation {C}riterion},
  booktitle = {Proceedings of the IEEE Global Telecommunication
          Conference (GLOBECOM'93)},
  pages     = {87-91},
  address   = {Houston},
  month     = nov # "/"  # dec,
  year      = 1993
}

@Article{     kamel:94,
  author    = {R.E.~Kamel and Y.~{Bar--Ness}},
  title     = {{B}lind maximum likelihood sequence estimation of digital
          sequences in presence of intersymbol interference},
  journal   = {Electronics Letters},
  volume    = {30},
  pages     = {537-539},
  number    = {7},
  year      = 1994
}

@Article{     Kam94,
  author    = {K.D.~Kammeyer},
  title     = {{T}ime {T}runcation of {C}hannel {I}mpulse {R}esponses by
          {L}inear {F}iltering: {A} {M}ethod to {R}educe the
          {C}omplexity of {V}iterbi {E}qualization},
  journal   = {International Journal of Electronics and Communications
          (AE\"U)},
  volume    = {48},
  number    = {5},
  pages     = {237-243},
  year      = 1994
}

@Book{        Kam92,
  author    = {K.~D.~Kammeyer},
  title     = {{N}achrichten\"ubertragung},
  publisher = {B.~G.~Teubner},
  address   = {Stuttgart},
  year      = 1992
}

@Article{     kanal:79,
  author    = {L.N. Kanal and A.R.K. Sastry},
  title     = {Models for Channels with Memory and Their Applications to
          Error Control},
  journal   = {Proc. IEEE},
  volume    = {66},
  pages     = {724-744},
  year      = 1978
}

@Book{        Kay88,
  author    = {S.~M.~Kay},
  title     = {Modern {S}pectral {E}stimation: {T}heory and {A}pplication},
  publisher = {Prentice--Hall},
  address   = {New Jersey},
  year      = 1988
}

@Article{     kechriotis:94,
  author    = {G.~Kechriotis and E.~Zervas and E.S.~Manolakos},
  title     = {{U}sing {R}ecurrent {N}eural {N}etworks for {A}daptive
          {C}ommunication {C}hannel {E}qualization},
  journal   = neu,
  volume    = {5},
  pages     = {267-278},
  month     = mar,
  year      = 1994
}

@Article{     kechriotis:96,
  author    = {G.I.~Kechriotis and E.S.~Manolakos},
  title     = {{H}opfield {N}eural {N}etwork {I}mplementation of the
          {O}ptimal {CDMA} {M}ultiuser {D}etector},
  journal   = neu,
  volume    = {7},
  pages     = {131-141},
  month     = jan,
  year      = 1996
}

@Article{     kennedy:92,
  author    = {D.~Williamson and R.A.~Kennedy and G.W.~Pulford},
  title     = {{Block Decision Feedback Equalization}},
  journal   = com,
  volume    = {COM-40},
  number    = {2},
  pages     = {255-264},
  month     = feb,
  year      = 1992
}

@TechReport{      kerep:92a,
  author    = {J. Huber},
  title     = {{R}eichweitenerh"ohung durch {K}analcodierung bei der
          digitalen {"U}bertragung "uber symmetrische {L}eitungen},
  institution   = {Lehrstuhl f"ur Nachrichtentechnik der Universit"at
          Erlangen--N"urnberg},
  type      = {Techn. {B}ericht},
  year      = {1992}
}

@TechReport{      kerep:97,
  author    = {J.~Huber},
  title     = {{Leitungs- und Kanalcodierung f{\"u}r ein
          {\glqq}Single--Pair Digital Subscriber--Line{\grqq}
          (SDSL)--System}},
  institution   = {Lehrstuhl f"ur Nachrichtentechnik der Universit"at
          Erlangen--N"urnberg},
  type      = {Techn. {B}ericht},
  year      = {1997}
}

@Article{     kerpez:93,
  author    = {K.J.~Kerpez},
  title     = {{Near--End Crosstalk is Almost Gaussian}},
  journal   = com,
  volume    = {COM-41},
  pages     = {670-672},
  month     = jan,
  year      = 1993
}

@TechReport{      kittel:83,
  author    = {L. {Kittel, R. Wenzel}},
  title     = {{E}influ"sfaktoren auf die {D}igital"ubertragung beim
          {T}eilnehmeranschlu"s im {ISDN}},
  institution   = {{TEKADE} Techn. Mitteilungen},
  pages     = {S.77-83},
  year      = 1983
}

@Book{        knuth:69,
  author    = {Knuth, D.E.},
  title     = {The art of computer programming, Vol.1 Fundamental
          Algorithms},
  publisher = {Addison-Wesley},
  address   = {Reading, Massachusetts},
  year      = 1969
}

@Book{        knuth:73,
  author    = {Knuth, D.E.},
  title     = {The art of computer programming, Vol.3 Sorting and
          Searching},
  publisher = {Addison-Wesley},
  address   = {Reading, Massachusetts},
  year      = 1973
}

@Article{     kobayashi:71a,
  author    = {H. Kobayashi},
  title     = {Simultaneous Adaptive Estimation and Decision Algorithm
          for Carrier Modulated Data Transmission Systems},
  journal   = com,
  volume    = {COM-19},
  pages     = {268-280},
  month     = jun,
  year      = 1971
}

@Article{     kobayashi:71b,
  author    = {H. Kobayashi},
  title     = {A survey of Coding schemes for transmission or recording
          of digital data},
  journal   = com,
  volume    = {COM-19},
  pages     = {1087-1100},
  month     = {},
  year      = 1971
}

@InProceedings{   koch:89,
  author    = {W.~Koch and A.~Baier},
  title     = {{C}ombined {D}esign of {E}qualizer and {C}hannel {D}ecoder
          for {D}igital {M}obile {R}adio {R}eceivers},
  booktitle = {Proceedings of ITG Conference ,,Stochastische Modelle und
          Methoden in der Informationstechnik''},
  pages     = {263-270},
  address   = {N\"urnberg},
  month     = apr,
  year      = 1989
}

@InProceedings{   Koc90,
  author    = {W.~Koch and A.~Baier},
  title     = {{O}ptimum and {S}ub-{O}ptimum {D}etection of {C}oded
          {D}ata {D}isturbed by {T}ime-{V}arying {I}ntersymbol
          {I}nterference},
  booktitle = {Proceedings of the IEEE Global Telecommunication
          Conference ({GLOBECOM'90})},
  pages     = {807.5.1.-807.5.6.},
  address   = {San Diego},
  month     = dec,
  year      = 1990
}

@Book{        koehler:87,
  author    = {T. K"ohler},
  title     = {{B}andbreiten-- und leistungseffiziente
          {D}igitalsignal"ubertragung durch mehrstufig codierte
          {CPM}},
  publisher = {Diplomarbeit, Universit"at der Bundeswehr M"unchen},
  month     = dec,
  year      = 1987
}

@Book{        korn:85,
  author    = {I. Korn},
  title     = {Digital Communication},
  publisher = {North--Holland},
  address   = {Amsterdam},
  year      = 1985
}

@Book{        kressel:89,
  author    = {U. H.-G. Kre"sel},
  title     = {{I}nformationstheoretische {B}eurteilung digitaler
          {"U}bertragungsverfahren mit {H}ilfe des
          {F}ehlerexponenten},
  publisher = {Dissertation, Technische Hochschule Darmstadt},
  year      = 1989
}

@Book{        kroschel:86,
  author    = {K. Kroschel},
  title     = {Statistische Nachrichtentheorie},
  publisher = spr,
  address   = {Berlin},
  year      = 1986
}

@Article{     kruska:83,
  author    = {Kruskal, C.P.},
  title     = {Searching, merging and sorting in parallel computation},
  journal   = {IEEE Trans. on Comput.},
  volume    = {C-32},
  pages     = {942-946},
  year      = 1983
}

@Article{     kuehne:82,
  author    = {F. K"uhne},
  title     = {Peak Envelope Modulation {PAM}--{QAM}--Signals},
  journal   = {{AE"U} (Archiv f"ur Elektronik und "Ubertragungstechnik)},
  volume    = {Bd.36},
  pages     = {138-139},
  year      = 1982
}

@Article{     landau:62,
  author    = {H.J. Landau and H.O. Pollak},
  title     = {Prolate Spheroidal Wave Functions, Fourier Analysis and
          Uncertainty-{III}: The Dimension of the Space of
          Essentially Time- and Band- limited Signals},
  journal   = {Bell Syst. Tech. J.},
  volume    = {41},
  pages     = {1295-1336},
  month     = jul,
  year      = 1962
}

@Article{     lane:80,
  author    = {P.J. McLane},
  title     = {A Residual Intersymbol Interference Error Bound for
          Truncated--State Viterbi Detectors},
  journal   = inf,
  volume    = {IT-26},
  pages     = {548-553},
  year      = 1980
}

@ARTICLE{laneman2,
  author    = {J.N.~Laneman and G.W.~Wornell},
  title     = {{Distributed Space--Time Block Coded Protocols for Exploiting Cooperative Diversity in Wireless Networks}},
  journal   = inf,
  volume    = {IT-49},
  pages     = {2415-2425},
  month     = oct,
  year      = 2003
}

@ARTICLE{laneman1,
  author    = {J.~Laneman and D.~Tse and G.~Wornell},
  title     = {{Cooperative Diversity in Wireless Networks: Efficient Protocols and Outage Behavior}},
  journal   = inf,
  volume    = {50},
  pages     = {3062-3080},
  month     = dec,
  year      = 2004
}


@Article{     larsash:88,
  author    = {D.C.~Larson and J.~Ashley and T.D.~Howell},
  title     = {{O}n the {M}inimum {L}ength {E}rror {E}vent of {M}inimum
          {E}uclidean {W}eight},
  journal   = inf,
  volume    = {IT-34},
  pages     = {1074-1076},
  month     = sep,
  year      = 1988
}

@Article{     larsen:73,
  author    = {K.J. Larsen},
  title     = {Short convolutional codes with maximal free distance for
          rates 1/2, 1/3 and 1/4},
  journal   = inf,
  volume    = {IT-19},
  pages     = {371-372},
  year      = 1973
}

@InProceedings{   larsson:88,
  author    = {T. Aulin and T. Larsson},
  title     = {Two Classes of Algorithms for Asymptotical Optimal
          Simplified {MLSD} with Application to Digital Radio},
  booktitle = {EUROCON'88},
  note      = {Conf. Record},
  address   = {Stockholm, Sweden},
  pages     = {110-113},
  year      = 1988
}

@TechReport{      larsson:91,
  author    = {T.~Larsson},
  title     = {A state--space partitioning approach to trellis decoding},
  institution   = {Chalmers University of Technology},
  type      = {Technical Report 222},
  address   = {G\"oteborg},
  year      = 1991
}

@InProceedings{   leblanc:94,
  author    = {J.P.~LeBlanc and K.~Do\v{g}an\c{c}ay and R.A.~Kennedy and
          C.R.~{Johnson, Jr.}},
  title     = {{E}ffects of {I}nput {D}ata {C}orrelation on the
          {C}onvergence of {B}lind {A}daptive {E}qualizers},
  booktitle = {Proceedings of ICASSP'94},
  pages     = {III-313-III-316},
  address   = {Adelaide},
  month     = apr,
  year      = 1994
}

@Article{     lechleider:91,
  author    = {J.W.~Lechleider},
  title     = {{High Bit Rate Digital Subscriber Lines: A Review of HDSL
          Progress}},
  journal   = sel,
  volume    = {SAC-9},
  pages     = {769-784},
  month     = aug,
  year      = 1991
}

@Book{        lee:60,
  author    = {Y.W. Lee},
  title     = {Statistical Theory of Communication},
  publisher = {J. Wiley \& Sons},
  address   = {New York},
  year      = 1960
}

@Article{     lee:74,
  author    = {L.-N.~Lee},
  title     = {{R}eal-{T}ime {M}inimal-{B}it-{E}rror {P}robability
          {D}ecoding of {C}onvolutional {C}odes},
  journal   = com,
  volume    = {COM-22},
  pages     = {146-151},
  year      = 1974
}

@Article{     lee:85a,
  author    = {P.J. Lee},
  title     = {New short constraint length, rate 1/N convolutional codes
          which minimize the required SNR for given bit error rate},
  journal   = com,
  volume    = {COM-33},
  pages     = {171-177},
  year      = 1985
}

@InProceedings{   lee:85b,
  author    = {P.J. Lee},
  title     = {Further Results on Rate 1/N Convolutional Code
          Constructions with Minimum Required SNR Criterion},
  booktitle = {IEEE Global Communications Conference 1985},
  organization  = {GLOBECOM'85},
  pages     = {21.6.1-21.6.5},
  year      = 1985
}

@Book{        lee:88,
  author    = {E.A. Lee and D.G. Messerschmitt},
  title     = {{D}igital {C}ommunication},
  publisher = {Kluwer Academic Publishers},
  address   = {Boston},
  year      = 1988
}

@Article{     Lee98,
  author    = {I.~L.~Lee and J.~M~Cioffi},
  title     = {{Design of Equalized Maximum--Likelihood Receiver}},
  journal   = {IEEE Communications Letters},
  volume    = {2},
  pages     = {14-16},
  month     = jan,
  year      = 1998
}

@Article{     Lei88,
  author    = {H.~Leib and S.~Pasupathy},
  title     = {{T}he {P}hase of a {V}ector {P}erturbed by {G}aussian {N}oise
          and {{D}ifferentially} {C}oherent {R}eceivers},
  journal   = inf,
  volume    = {IT-34},
  pages     = {1491-1501},
  month     = nov,
  year      = 1988
}

@Article{     Lei95,
  author    = {H.~Leib},
  title     = {{D}ata--{A}ided {N}oncoherent {D}emodulation of {DPSK}},
  journal   = com,
  volume    = {COM-43},
  pages     = {722-725},
  month     = {feb-apr},
  year      = 1995
}

@Article{     Lei97,
  author    = {H.~Leib},
  title     = {{C}omments on ``{D}ifferential {D}etection with {IIR}
          {F}ilter for {I}mproving {DPSK} {D}etection {P}erformance''},
  journal   = com,
  volume    = {COM-45},
  pages     = {637},
  month     = jun,
  year      = 1997
}

@Article{     li:95,
  author    = {Y.~Li and B.~Vucetic and Y.~Sato},
  title     = {{O}ptimum {S}oft-{O}utput {D}etection for {C}hannels with
          {I}ntersymbol {I}nterference},
  journal   = inf,
  volume    = {IT-41},
  pages     = {704-713},
  month     = may,
  year      = 1995
}

@Article{     LCS99,
  author    = {Y.~Li and J.C.~Chung and N.R.~Sollenberger},
  title     = {{Transmit Diversity for OFDM Systems and its Impact on High--Rate Data Wireless Networks}},
  journal   = sel,
  volume    = {17},
  pages     = {1233-1243},
  month     = jul,
  year      = 1999
}

@Book{        lidl:83,
  author    = {R. Lidl and H. Niederreiter},
  title     = {Finite Fields, Encyclopedia of Math. and its Appl.},
  volume    = {20},
  publisher = {Addison Wesley},
  address   = {Reading, Mass.},
  year      = 1983
}

@Book{        lin:70,
  author    = {S. Lin},
  title     = {An Introduction to Error--Correction Codes},
  publisher = pre,
  address   = {Englewood Cliffs, N.J.},
  year      = 1970
}

@Book{        lin:83,
  author    = {S. Lin and D.J. {Costello Jr.}},
  title     = {Error Control Coding: Fundamentals and Applications},
  publisher = pre,
  address   = {Englewood Cliffs, N.J.},
  year      = 1983
}

@Article{     lin:93,
  author    = {T. Takata and S. Ujita and T. Kasami and S. Lin},
  title     = {{M}ultistage {D}ecoding of {M}ultilevel {B}lock {M-PSK}
          {M}odulation {C}odes and {I}ts {P}erformance {A}nalysis},
  journal   = inf,
  volume    = {IT-39},
  pages     = {1204-1218},
  month     = jul,
  year      = 1993
}

@InProceedings{   lindell:83,
  author    = {G. Lindell and C.-E. Sundberg},
  title     = {Multilevel Continuous Phase Modulation with High Rate
          Convolutional Codes},
  booktitle = {GLOBECOM'83},
  note      = {Conf. Record},
  pages     = {1021-1026},
  year      = 1983
}

@Article{     lindell:84a,
  author    = {G. Lindell and C.-E. Sundberg and T. Aulin},
  title     = {Multilevel Euclidean Distance for Combination of Short
          Rate 1/2 Convolutional Codes and {CPFSK} Modulation},
  journal   = inf,
  volume    = {IT-30},
  pages     = {509-519},
  month     = may,
  year      = 1984
}

@InProceedings{   lindell:84b,
  author    = {G. Lindell and C.-E. Sundberg and A. Svensson},
  title     = {Error Probability of Multilevel {CPM} with High Rate
          Convolutional Codes},
  booktitle = {Proceedings of the 1984 International Z"urich Seminar on
          Digital Communications 6.-8.3.1984},
  pages     = {93-100},
  year      = 1984
}

@PhDThesis{   lindell:85,
  author    = {G. Lindell},
  title     = {On Coded Continuous Phase Modulation},
  school    = {Lund University, Sweden},
  month     = may,
  year      = 1985
}

@Book{        lindsey:72,
  author    = {W. C. Lindsey},
  title     = {Synchronisation Systems in Communication and Control},
  publisher = {Prentice--Hall},
  address   = {Englewood Cliffs, NJ},
  year      = 1972
}

@Book{        lindsey:73,
  author    = {W. C. Lindsey and M. K. Simon},
  title     = {Telecommunication Systems Engeneering},
  publisher = {Prentice--Hall},
  address   = {Englewood Cliffs, NJ},
  year      = 1973
}

@InProceedings{   LP00,
  author    = {E.~Lindskog and A.~Paulraj},
  title     = {{A Transmit Diversity Scheme for Channels with Intersymbol Interference}},
  booktitle = {Proceedings of IEEE ICC},
  pages     = {307-311},
  address   = {New Orleans},
  year      = 2000
}

@Article{     Lin95,
  author    = {F.~Ling},
  title     = {{Matched Filter--Bound for Time--Discrete Multipath Rayleigh Fading Channels}},
  journal   = com,
  volume    = {COM-43},
  pages     = {710-713},
  month     = feb # "--"  # apr,
  year      = 1995
}


@InProceedings{   litzenburger:93,
  author    = {M. Litzenburger},
  title     = {{G}ezielte {B}eeinflussung der {H}\"ullkurve eines
          modulierten {S}ignals durch {C}odierung und ,,{S}haping''},
  booktitle = {8. DFG-Kolloquium im Schwerpunktprogramm ,,Grundlagen
          digitaler Kommunikationssysteme''},
  address   = {Saarbr\"ucken},
  month     = jun,
  year      = 1993
}

@Book{        liu:86,
  author    = {W.L. Liu},
  title     = {{F}altungscodierung f"ur {M}odulationsverfahren mit
          kontinuierlicher {P}hase},
  publisher = {Diplomarbeit, TU M"unchen},
  year      = 1986
}

@InProceedings{   liu:88a,
  author    = {W.L. Liu and J. Huber},
  title     = {Double Trellis--Coded {CPM}},
  booktitle = {Proceedings of the International Conference on
          Communications ({ICC}'88)},
  note      = {Conf. Record},
  pages     = {51.4.1-51.4.6},
  adrress   = {Philadelphia},
  year      = 1988
}

@InProceedings{   liu:88b,
  author    = {W.L. Liu and J. Huber},
  title     = {Special Quaternary {CPM} Schemes with Rate 2/3 Trellis
          Codes},
  booktitle = {International Workshop on Information Theory},
  note      = {Proceedings},
  pages     = {E5.1.-E5.4.},
  address   = {Beijing},
  year      = 1988
}

@Book{        liu:90,
  author    = {W. Liu},
  title     = {Complexity Reduction of coherent Receivers for Digital
          Continuous Phase Modulation},
  publisher = {Dissertation, Universit"at der Bundeswehr M"unchen},
  year      = 1990
}

@InProceedings{   liu:90b,
  author    = {W. Liu and J. Huber},
  title     = {Data--Aided Synchronization of {$M \geq 2$}--ary Coherent
          Receivers},
  booktitle = {GLOBECOM 1990},
  address   = {San Diego},
  pages     = {501.3.1-501.3.5},
  note      = {Conference Record},
  month     = dec,
  year      = 1990
}

@Article{     liu:95,
  author    = {Z.-S.~Liu},
  title     = {{QR methods of O(N) complexity in adaptive parameter
          estimation}},
  journal   = sip,
  volume    = {43},
  pages     = {720-729},
  year      = 1995
}

@Article{     liu:97,
  author    = {R.~Liu and G.~Dong},
  title     = {{A} {F}undamental {T}heorem for {M}ultiple--{C}hannel
          {B}lind {E}qualization},
  journal   = csi,
  volume    = {44},
  pages     = {472-473},
  month     = may,
  year      = 1997
}

@InProceedings{   LFT01,
  author    = {Y.~Liu and M.P.~Fitz and O.Y.~Takeshita},
  title     = {{Space--Time Codes Performance Criteria and Design for Frequency Selective Fading Channels}},
  booktitle = {Proceedings of IEEE International Conference on Communications (ICC)},
  address   = {Helsinki, Finland},
  month     = jun,
  pages     = {2800-2804},
  year      = 2001
}

@Article{     Lod90,
  author    = {J.~H.~Lodge and M.~L.~Moher},
  title     = {{M}aximum {L}ikelihood {S}equence {E}stimation of {CPM}
          {S}ignals {T}ransmitted {O}ver {R}ayleigh {F}lat--{F}ading
          {C}hannel},
  journal   = com,
  volume    = {COM-38},
  pages     = {787-794},
  month     = jun,
  year      = 1990
}

@Article{     lopes:94,
  author    = {S.~Safavi and L.B.~Lopes},
  title     = {Simple non-coherent equalizer for the {DECT} system},
  journal   = {Electronics Letters},
  volume    = {30},
  pages     = {756-757},
  number    = {10},
  year      = 1994
}

@Article{     lucky:65,
  author    = {R.W.~Lucky},
  title     = {{A}utomatic {E}qualization for {D}igital
          {C}ommunications},
  journal   = bel,
  volume    = {44},
  pages     = {547-588},
  month     = apr,
  year      = 1965
}

@Book{        Luc68,
  author    = {R.~W.~Lucky and J.~Salz and E.~J.~Weldon, Jr. },
  title     = {Principles of Data Communication},
  publisher = {McGraw--Hill},
  address   = {New York},
  year      = 1968
}

@Book{        luecke:90,
  author    = {H.D. L"uke},
  title     = {{S}ignal"ubertragung},
  publisher = spr,
  address:  = {Berlin},
  note      = {{V}ierte {A}uflage},
  year      = 1990
}

@Book{        luo:97,
  author    = {F.-L.~Luo and R.~Unbehauen},
  title     = {{A}pplied {N}eural {N}etworks for {S}ignal {P}rocessing},
  publisher = {Cambridge University Press},
  address   = {Cambridge},
  year      = 1997
}

@Article{     ma:86,
  author    = {Ma, H.H. and Wolf, J.K.},
  title     = {On Tail Biting Convolutional Codes},
  journal   = com,
  volume    = {COM-34},
  pages     = {104-111},
  year      = 1986
}

@Article{     macchi:84,
  author    = {O.~Macchi and E.~Eweda},
  title     = {{C}onvergence {A}nalysis of {S}elf--{A}daptive
          {E}qualizers},
  journal   = inf,
  volume    = {IT-30},
  pages     = {161-176},
  month     = mar,
  year      = 1984
}

@InProceedings{   macchi:96,
  author    = {J. Labat and O. Macchi and C. Laot and N.~{Le Squin}},
  title     = {{I}s {T}raining of {A}daptive {E}qualizers still
          {U}seful?},
  booktitle = {Proceedings of the IEEE Global Telecommunication
          Conference (GLOBECOM'96)},
  address   = {London},
  pages     = {968-972},
  month     = nov,
  year      = 1996
}

@Article{     Mac94,
  author    = {K.~M.~Mackethun, Jr.},
  title     = {{A} {F}ast {A}lgorithm for {M}ultiple-{S}ymbol {D}ifferential {D}etection of {MPSK}},
  journal   = com,
  volume    = {COM-42},
  pages     = {1471-1474},
  month     = {feb-apr},
  year      = 1994
}

@InProceedings{   Mag99,
  author    = {M.~Magarini and A.~Spalvieri and G.~Tartara},
  title     = {{Improving Error Performance of Equalized Receivers for Broadband Radio}},
  booktitle = {IEEE Vehicular Technology Conference (VTC)},
  address   = {Amsterdam, Netherlands},
  pages     = {2377-2381},
  month     = sep,
  year      = 1999
}

@Article{     Mak75,
  author    = {J.~Makhoul},
  title     = {Linear {P}rediction: {A} {T}utorial {R}eview},
  journal   = {Proceedings of the {IEEE}},
  volume    = {63},
  pages     = {561-580},
  month     = apr,
  year      = 1975
}

@Article{     Mak94,
  author    = {D.~Makrakis and P.~T.~Mathiopoulos and D.~P.~Bouras},
  title     = {{O}ptimal {D}ecoding of {C}oded {PSK} and {QAM} {S}ignals in
          {C}orrelated {F}ast {F}ading {C}hannels and {AWGN}: {A} {C}ombined
          {E}nvelope, {M}ultiple {D}ifferential and {C}oherent {D}etection {A}pproach},
  journal   = com,
  volume    = {COM-42},
  pages     = {63-74},
  month     = jan,
  year      = 1994
}

@Article{     mandelbaum:74,
  author    = {D.M. Mandelbaum},
  title     = {An Adaptive--Feedback Coding Scheme Using Incremental
          Redundancy},
  journal   = inf,
  volume    = {IT-20},
  pages     = {388-389},
  month     = may,
  year      = 1974
}

@Article{     marko:74,
  author    = {H. Marko},
  title     = {{O}ptimale und fast optimale bin"are und mehrstufige
          digitale {"U}bertragungssysteme},
  journal   = {AE"U 28},
  pages     = {S.402-414},
  year      = 1974
}

@Book{        marko:77,
  author    = {H. Marko},
  title     = {{M}ethoden der {S}ystemtheorie},
  publisher = {Springer-Verlag},
  address   = {Berlin, Heidelberg, New York},
  year      = 1977
}

@Article{     mason:53,
  author    = {S.L. Mason},
  title     = {Feedback Theory--Some Properties of Signal Flow Graphs},
  journal   = {Proceedings of the I.R.E},
  volume    = {Bd.41},
  pages     = {1144-1156},
  month     = sep,
  year      = 1953
}

@Book{        massey:63,
  author    = {J.L. Massey},
  title     = {Threshold decoding},
  publisher = {M.I.T.--Press},
  address   = {Cambridge, Massachusetts},
  year      = 1963
}

@InProceedings{   massey:74,
  author    = {J.L. Massey},
  title     = {Coding and Modulation in Digital Communications},
  booktitle = {1974 Intern. Z\"urich Seminar on Digital Communications},
  address   = {Z\"urich, Switzerland},
  month     = mar,
  year      = 1974
}

@InProceedings{   massey:78,
  author    = {J.L. Massey},
  title     = {Foundations and Methods of Channel Encoding},
  booktitle = {NTG--Fachbericht {65}},
  address   = {Berlin},
  pages     = {148-157},
  month     = sep,
  year      = 1978
}

@InProceedings{   massey:84,
  author    = {J.L. Massey},
  title     = {The how and why of channel coding},
  booktitle = {1984 International Z\"urich Seminar on Digital
          Communications},
  address   = {Z\"urich, Switzerland},
  pages     = {67-73},
  month     = mar,
  year      = 1984
}

@Misc{        massey:87,
  author    = {J.L. Massey},
  title     = {Structures of Convolutional Encoders},
  note      = {Lecture at Siemens {AG}, Munich, 24.4.1987}
}

@Misc{        massey:script,
  author    = {J.L. Massey},
  title     = {Applied Digital Information Theory},
  note      = {Vorlesungsskriptum an der ETH Z"urich 1987,1988}
}

@InProceedings{   MT01,
  author    = {P.~Maurer and V.~Tarokh},
  title     = {{Transmit Diversity When the Receiver Does not Know the Number of Transmit
Antennas}},
  booktitle = {Proceedings of the International Symposium on Wireless Multimedia Communications (WPMC)},
  address   = {Aalborg, Denmark},
  month     = sep,
  year      = 2001
}

@Article{     mazo:76,
  author    = {J.E.~Mazo and J.~Salz},
  title     = {{O}n the {T}ransmitted {P}ower in {G}eneralized {P}artial
          {R}esponse},
  journal   = com,
  volume    = {COM-24},
  pages     = {348-352},
  month     = mar,
  year      = 1976
}

@Article{     mazo:80,
  author    = {J.E.~Mazo},
  title     = {{A}nalysis of {D}ecision--{D}irected {E}qualizer
          {C}onvergence},
  journal   = {Bell Syst. Tech. J.},
  volume    = {59},
  pages     = {1857-1876},
  month     = dec,
  year      = 1980
}

@Article{     Maz91,
  author    = {J.E.~Mazo},
  title     = {{Exact Matched Filter Bound for Two--Beam Rayleigh Fading}},
  journal   = com,
  volume    = {COM-39},
  pages     = {1027-1030},
  month     = jul,
  year      = 1991
}

@Article{     mc:68,
  author    = {R.H. McCullough},
  title     = {The binary regenerative channel},
  journal   = {Bell Syst. Tech. J.},
  volume    = {47},
  pages     = {1713-1735},
  year      = {1968}
}

@Book{        mceliece:77,
  author    = {R.J. McEliece},
  title     = {The Theory of Information and Coding},
  publisher = {Addison--Wesley},
  address   = {Reading, Mass.},
  year      = 1977
}

@Book{        mcwill:78,
  author    = {mcwill:78},
  title     = {x},
  publisher = {x},
  address   = {x},
  year      = 1987
}

@Article{     mealy:55,
  author    = {G.H. Mealy},
  title     = {A method for synthesizing sequential circuits},
  journal   = {Bell Syst. Tech. J.},
  volume    = {34},
  pages     = {1054-1079},
  year      = 1955
}

@Misc{        mefige:96a,
  author    = {R.~Meyer and R.~Fischer and W.~Gerstacker and J.~Huber and
          P.~Schramm},
  title     = {{E}ntzerrer mit einem {S}equenzsch\"atzverfahren mit
          {Z}ustandsreduktion f\"ur einen {E}mpf\"anger in einem
          digitalen {\"U}bertragungssystem},
  howpublished  = {German Patent Application no.~196 14 544.9},
  month     = apr,
  year      = 1996
}

@Misc{        mefige:96b,
  author    = {R.~Meyer and R.~Fischer and W.~Gerstacker and J.~Huber and
          P.~Schramm},
  title     = {{E}ntzerrer mit erweiterter {K}analsch\"atzung f\"ur einen
          {E}mpf\"anger in einem digitalen {\"U}bertragungssystem},
  howpublished  = {German Patent Application no.~196 14 543.0},
  month     = apr,
  year      = 1996
}

@Article{     messerschmitt:73,
  author    = {D.G. Messerschmitt},
  title     = {{A} {G}eometric {T}heory of {I}ntersymbol {I}nterference,
          {P}art {I} and {II}},
  journal   = {Bell Syst. Tech. J.},
  volume    = {52},
  pages     = {1483-1539},
  month     = {},
  year      = 1973
}

@InProceedings{   messerschmitt:93,
  author    = {J.R.~Barry and E.A.~Lee and D.G.~Messerschmitt},
  title     = {{C}apacity {P}enalty due to {I}deal {Z}ero-{F}orcing
          {D}ecision-{F}eedback {E}qualization},
  booktitle = {Proceedings of the International Conference on
          Communications ({ICC}'93)},
  pages     = {422-427},
  address   = {Geneva},
  month     = may,
  year      = 1993
}

@InProceedings{   meyr:89,
  author    = {H. Meyr},
  title     = {Signal Processing in Digital Receivers: Modell Algorithm,
          Architecture},
  booktitle = {ITG--Fachbericht 107},
  note      = {Stochastische Modelle und Methoden in der
          Informationstechnik},
  publisher = {VDE--Verlag},
  pages     = {325-337},
  year      = 1989
}

@Book{        meyr:90,
  author    = {H. Meyr and G. Ascheid},
  title     = {Synchronisation in Digital Communication --- Vol {I}:
          Phase--, Frequency--Locked Loops and Amplitude Control},
  publisher = wil,
  address   = {New York},
  year      = 1990
}

@Book{        michelson:85,
  author    = {A.M. Michelson and A.H. Levesque},
  title     = {Error--Control Techniques for Digital Communication},
  publisher = wil,
  address   = {New York},
  year      = 1985
}

@Book{        Mil74,
  author    = {K.~Miller},
  title     = {{C}omplex {S}tochastic {P}rocesses},
  publisher = {Addison--Wesley},
  address   = {New York},
  year      = 1974
}

@Article{     millot:87,
  author    = {L.J. Millot},
  title     = {Cointensity spectra in nonlinear bandpass digital {QAM}
          systems},
  journal   = {{AE"U} (Arch. elektr. "Ubertragung)},
  volume    = {},
  pages     = {21-27},
  year      = {1987}
}

@TechReport{      mirsch:86,
  author    = {P.~Mirsch},
  title     = {{M}athematik f\"ur {I}ngenieure {III} + {IV}},
  institution   = {Universit\"at Erlangen-N\"urnberg},
  type      = {Vorlesungsskriptum},
  year      = 1986
}

@Article{     mohan:86,
  author    = {Mohan, S. and Sood, A.K.},
  title     = {A Multiprocessor Architecture for the {(M,L)}-Algorithm
          Suitable for {VLSI} Implementation},
  journal   = com,
  volume    = {COM-34},
  pages     = {1218-1224},
  year      = 1986
}

@PhDThesis{   moldi:89,
  author    = {B.E. Rimoldi},
  title     = {Continous Phase Modulation and Coding for Bandwidth and
          Energy Efficiency},
  school    = {Federal Institute of the Technology Z"urich, Switzerland},
  year      = 1988
}

@Article{     monsen:71,
  author    = {P.~Monsen},
  title     = {{F}eedback {E}qualization for {F}ading {D}ispersive
          {C}hannels},
  journal   = inf,
  volume    = {IT-17},
  pages     = {56-64},
  month     = jan,
  year      = 1971
}

@Article{     monsen:74,
  author    = {P.~Monsen},
  title     = {{A}daptive {E}qualization of the {S}low {F}ading
          {C}hannel},
  journal   = com,
  volume    = {COM-22},
  pages     = {1064-1075},
  month     = aug,
  year      = 1974
}

@InProceedings{   moon:93,
  author    = {J.~Moon and S.~She},
  title     = {{O}ptimal {F}ilter {D}esign for {F}ixed {D}elay {T}ree
          {S}earch with {D}ecision {F}eedback},
  booktitle = {Proceedings of the IEEE Global Telecommunication
          Conference (GLOBECOM'93)},
  pages     = {1965-1969},
  address   = {Houston},
  month     = nov # "/"  # dec,
  year      = 1993
}

@Book{        MS00,
  author    = {T.~Moon and W.~Stirling},
  title     = {{Mathematical Methods and Algorithms for Signal Processing}},
  publisher = {Prentice Hall},
  address   = {New York},
  year      = 2000
}

@Article{     mooser:83,
  author    = {M. Mooser},
  title     = {Some periodic convolutional codes better than any fixed
          code},
  journal   = inf,
  volume    = {vol:IT-29},
  pages     = {750-751},
  month     = sep,
  year      = 1983
}

@TechReport{      morgenstern:87,
  author    = {G. Morgenstern},
  title     = {{B}eseitigung von {F}ehlerb"undeln bei {A}nwendung der
          quantisierten {R}"uckkopplung zur
          {G}leichsignalwiedergewinnung},
  institution   = {Forschungsinstitut der Deutschen Bundespost},
  type      = {Techn. Bericht},
  number    = {44 TB 107},
  month     = sep,
  year      = 1987
}

@Article{     mori:91,
  author    = {I. Sasase and S. Mori},
  title     = {Multi--h Phase--Coded Modulation},
  journal   = cma,
  volume    = {29},
  pages     = {46-56},
  month     = dec,
  year      = 1991
}

@Article{     moulines:95,
  author    = {E.~Moulines and P.~Duhamel and J.-F.~Cardoso and
          S.~Mayrargue},
  title     = {{S}ubspace {M}ethods for the {B}lind {I}dentification of
          {M}ultichannel {FIR} {F}ilters},
  journal   = sip,
  volume    = {43},
  pages     = {516-525},
  month     = feb,
  year      = 1995
}

@InProceedings{   mour:92,
  author    = {Ch.~Mourot},
  title     = {{A} {H}igh {B}it {R}ate {T}ransmission {T}echnique in
          {M}obile {R}adio {C}ellular {E}nvironment},
  booktitle = {Proceedings of {UTC'92}},
  pages     = {740-743},
  year      = 1992
}

@InProceedings{  MP00,
  author    = {S.~Mudulodu and A.~Paulraj},
  title     = {{A Transmit Diversity Scheme for Frequency Selective Fading Channels}},
  booktitle = {Proceedings of the IEEE Global Telecommunications Conference (GLOBECOM)},
  address   = {San Francisco},
  pages     = {1089-1093},
  month     = nov,
  year      = 2000
}

@InProceedings{   muegehu:96,
  author    = {S.~M\"uller and W.~Gerstacker and J.~Huber},
  title     = {{R}educed--{S}tate {S}oft--{O}utput
          {T}rellis--{E}qualization {I}ncorporating {S}oft
          {F}eedback},
  booktitle = {Proceedings of the IEEE Global Telecommunication
          Conference (GLOBECOM'96)},
  address   = {London},
  pages     = {95-100},
  month     = nov,
  year      = 1996
}

@InProceedings{   muegehu:97,
  author    = {S.~M\"uller and W.~Gerstacker and J.~Huber},
  title     = {{S}oft {D}ecision--{F}eedback in {R}educed--{S}tate
          {T}rellis--{E}qualization with {S}oft--{O}utput},
  booktitle = {Proceedings of the IEEE Workshop Kommunikationstechnik
          '97},
  address   = {Schlo{\ss} Reisensburg bei Ulm},
  month     = jan,
  year      = 1997
}

@Book{        mueller:96,
  author    = {S.~M{\"u}ller},
  title     = {{S}ch"atzung der {Z}uverl"assigkeit der {A}usgangssymbole
          bei {S}equenzsch"atzung mit reduzierter {Z}ustandszahl},
  publisher = {Diplomarbeit, Lehrstuhl f\"ur Nachrichtentechnik der
          Universit\"at Erlangen-N\"urnberg},
  month     = feb,
  year      = 1996
}

@Article{     mulligan:84,
  author    = {M.G. Mulligan and S.G. Wilson},
  title     = {An Improved Algorithm for Evaluating Trellis Phase Codes},
  journal   = inf,
  volume    = {IT-30},
  pages     = {846-851},
  month     = nov,
  year      = 1984
}

@Article{     mur:81,
  author    = {K. Murota and K. Hirade},
  title     = {{GMSK} Modulation for Digital Mobile Telephony},
  journal   = com,
  volume    = {COM-29},
  pages     = {1044-1050},
  month     = jul,
  year      = 1981
}

@ARTICLE{eth,
  author    = {R.~Nabar and H.~B\"olcskei and F.~Kneub\"uhler},
  title     = {{Fading Relay Channels: Performance Limits and Space-Time Signal Design}},
  journal   = sel,
  volume    = {22},
  pages     = {1099-1109},
  month     = aug,
  year      = 2004
}

@InProceedings{   nagaosa:96,
  author    = {T.~Nagaosa and T.~Miyajima and T.~Hasegawa},
  title     = {{M}ultiuser {D}etection {U}sing a {H}opfield {N}etwork in
          {A}synchronous {M}--ary/{SSMA} {C}ommunications},
  booktitle = {Proceedings of the Fourth International Symposium on
          Spread Spectrum Techniques and Applications (ISSSTA'96)},
  address   = {Mainz},
  month     = sep,
  pages     = {837-841},
  year      = 1996
}

@Article{     NTSC98,
  author    = {A.F.~Naguib and V.~Tarokh and N.~Seshadri and A.R.~Calderbank},
  title     = {{A Space-Time Coding Modem for High-Data-Rate Wireless Communications}},
  journal   = sel,
  volume    = {SAC-16},
  pages     = {1459-1478},
  month     = oct,
  year      = 1998
}


@InProceedings{   Nag00,
  author    = {A.F.~Naguib},
  title     = {{Equalization of Transmit Diversity Space--Time Coded Signals}},
  booktitle = {IEEE Global Telecommunications Conference (GLOBECOM)},
  address   = {San Francisco},
  pages     = {1077-1082},
  month     = dec,
  year      = 2000
}

@Article{     NSL05,
  author    = {A.~Nasri and R.~Schober and L.~Lampe},
  title     = {{Performance of a BPSK NB Receiver in MB-OFDM UWB Interference}},
  journal   = {Submitted to IEEE International Conference on Communications (ICC)},
  volume    = {},
  pages     = {},
  month         = sep,
  year      = 2005
}

@Article{     Nee93,
  author    = {F.~D.~Neeser, J.~L.~Massey},
  title     = {{P}roper {C}omplex {R}andom {P}rocesses with {A}pplications to {I}nformation {T}heory},
  journal   = inf,
  volume    = {IT-39},
  pages     = {1293-1302},
  month     = jul,
  year      = 1993
}

@Article{     nikias:87,
  author    = {C.L.~Nikias and M.R.~Raghuveer},
  title     = {{B}ispectrum {E}stimation: {A} {D}igital {S}ignal
          {P}rocessing {F}ramework},
  journal   = {Proc. IEEE},
  volume    = {75},
  pages     = {869-891},
  month     = jul,
  year      = 1987
}

@Article{     nowlan:93,
  author    = {S.J.~Nowlan and G.E.~Hinton},
  title     = {{A} {S}oft {D}ecision--{D}irected {LMS} {A}lgorithm for
          {B}lind {E}qualization},
  journal   = com,
  volume    = {COM-41},
  pages     = {275-279},
  month     = feb,
  year      = 1993
}

@Article{     nyquist:28,
  author    = {H. Nyquist},
  title     = {Certain topics in telegraph transmission theory},
  journal   = {AIEE Transactions},
  volume    = {47},
  pages     = {617-644},
  year      = 1928
}

@Book{        odenwalder:76,
  author    = {J.P. Odenwalder},
  title     = {Error Control Handbook (Final Report)},
  publisher = {Linkabit Corp.},
  address   = {San Diego},
  year      = 1976
}

@Article{     oelcer:91,
  author    = {S.~{\"O}l{\c{c}}er},
  title     = {{Performance Analysis of Viterbi Detection of Class IV
          Partial Response for Data Transmission Over Multipair
          Cables}},
  journal   = com,
  volume    = {COM-39},
  number    = {10},
  pages     = {1423-1426},
  month     = oct,
  year      = 1991
}

@InProceedings{   oerder:85,
  author    = {M. "Order},
  title     = {Rotationally invariant trellis codes for {MPSK}
          modulation},
  booktitle = {IEEE Int. Conf. Commun. (ICC'85)},
  note      = {Conference Record},
  pages     = {552-556},
  year      = 1985
}

@Article{     oerder:87,
  author    = {M. "Order and H. Meyr},
  title     = {Rotationally invariant trellis codes for {MPSK}
          modulation},
  journal   = {Archiv f"ur Elektr. u. "Ubertragungstechnik ({AE"U})},
  volume    = {Bd.41},
  pages     = {28-32},
  month     = jan,
  year      = 1987
}

@Book{        oerder:89,
  author    = {M. "Order},
  title     = {{A}lgorithmen zur {D}igitalen {T}aktsynchronisation bei
          {D}aten"ubertragung},
  publisher = {Dissertation, RWTH Aachen},
  year      = 1989
}

@Book{        oppenheim:75,
  author    = {A.V. Oppenheim and R.W. Schafer},
  title     = {Digital Signal Processing},
  publisher = pre,
  address   = {Englewood Cliffs, New Jersey},
  year      = {1975}
}

@Book{        oppenheim:92,
  author    = {A.V.~Oppenheim and R.W.~Schafer},
  title     = {Zeitdiskrete Signalverarbeitung},
  publisher = old,
  address   = {M\"unchen Wien},
  year      = {1992}
}

@Book{        OW96,
  author    = {A.V.~Oppenheim and A.S.~Willsky},
  title     = {Signals and Systems},
  publisher = pre,
  address   = {Upper Saddle River, New Jersey},
  year      = {1996}
}

@Article{     paaske:74,
  author    = {E. Paaske},
  title     = {Short binary convolutional codes with maximal free
          distance for rates 2/3 and 3/4},
  journal   = inf,
  volume    = {IT-20},
  pages     = {683-689},
  year      = 1974
}

@Book{        papoulis:65,
  author    = {Athanasios Papoulis},
  title     = {Probability, Random Variables and Stochastic Processes},
  publisher = {McGraw--Hill},
  address   = {Tokyo},
  year      = {1965}
}

@Book{        Pap84,
  author    = {Athanasios Papoulis},
  title     = {{Probability, Random Variables and Stochastic Processes}},
  publisher = {McGraw--Hill},
  address   = {New York},
  year      = {1984}
}

@Article{     park:79,
  author    = {C.A.~Belfiore and J.H.~Park},
  title     = {Decision--feedback equalization},
  journal   = {Proc. IEEE},
  volume    = {67},
  pages     = {1143-1156},
  month     = aug,
  year      = 1979
}

@Book{        parsche:96,
  author    = {I.~Parsche},
  title     = {{Kombinierte Synchronisation und Entzerrung f\"ur digitale
          Kabel\"ubertragung mit Tomlinson--Harashima--Vorcodierung}},
  publisher = {Diplomarbeit, Lehrstuhl f\"ur Nachrichtentechnik der
          Universit\"at Erlangen-N\"urnberg},
  month     = dec,
  year      = 1996
}

@Article{     pas:79,
  author    = {S. Pasupathy},
  title     = {Minimum Shift Keying: A Spectrally Efficient Modulation},
  journal   = {IEEE Commun. Magazine},
  volume    = {17},
  pages     = {14-22},
  month     = jul,
  year      = 1979
}

@Article{     Mas96,
  author    = {A.~Masoomzadeh-Fard and S.~Pasupathy},
  title     = {{N}onlinear {E}qualization of {M}ultipath {F}ading
          {C}hannels with {N}oncoherent {D}emodulation},
  journal   = sel,
  volume    = {SAC-14},
  pages     = {512-520},
  month     = apr,
  year      = 1996
}

@Article{     Paw82,
  author    = {R.~F.~Pawula and S.~O.~Rice and J.~H.~Roberts},
  title     = {{Distribution of the Phase Angle Between Two
          Vectors Perturbed by Gaussian Noise}},
  journal   = com,
  volume    = {COM-30},
  number    = {8},
  pages     = {1828-1841},
  month     = aug,
  year      = 1982
}

@Article{     pe31,
  author    = {C. Beare},
  title     = {{The Choice of the Desired Impulse Response in Combined
          Linear--Viterbi Algorithm Equalizers}},
  journal   = com,
  volume    = {COM-26},
  number    = {8},
  pages     = {1301-1307},
  month     = aug,
  year      = 1978
}

@Article{     pe36,
  author    = {A. Desblanche},
  title     = {Optimal Short Desired Impulse Response for Maximum
          Likelihood Sequence Estimation},
  journal   = com,
  volume    = {COM-25},
  pages     = {735-738},
  month     = jul,
  year      = 1977
}

@Article{     pe38,
  author    = {D.~Falconer and F.~Magee},
  title     = {{A}daptive {C}hannel {M}emory {T}runcation for {M}aximum
          {L}ikelihood {S}equence {E}stimation},
  journal   = {The Bell System Technical Journal},
  volume    = {52},
  number    = {9},
  pages     = {1541-1562},
  month     = nov,
  year      = 1973
}

@Article{     pe43,
  author    = {G. Foschini},
  title     = {A Reduced State Variant of Maximum Likelihood Sequence
          Detection Attaining Optimum Performance for High
          Signal--to--Noise Ratios},
  journal   = inf,
  volume    = {IT-23},
  number    = {5},
  pages     = {605-609},
  month     = sep,
  year      = 1977
}

@Article{     pe53,
  author    = {F. Magee and J. Proakis},
  title     = {Adaptive Maximum--Likelihood--Sequence Esimation for
          Digital Signaling in the Presence of Intersymbol
          Interference},
  journal   = inf,
  volume    = {},
  pages     = {},
  month     = jan,
  year      = 1973
}

@Article{     pe59,
  author    = {P.J. McLane},
  title     = {Lower Bounds for Finite Intersymbol Interference Error
          Rates},
  journal   = com,
  volume    = {COM-22},
  pages     = {853-857},
  month     = jun,
  year      = 1974
}

@Article{     peters:80,
  author    = {U. {Peters, K. Tr"ondle, H.-W. Wellhausen}},
  title     = {{U}ntersuchung der {"U}bertragungseigenschaften und
          {S}t"orungen von {O}rtskabeln bei einer
          {D}igitalsignal"ubertragung oberhalb von 2.048 {MBit}/s},
  journal   = {{NTZ}--Archiv 2},
  volume    = {Heft 6},
  pages     = {S.111-116},
  year      = 1980
}

@Article{     peters:82,
  author    = {K. {Tr"ondle, U. Peters}},
  title     = {{P}r"adiktionsdetektion mit {Q}uantisierter
          {R}"uckkopplung},
  journal   = {{NTZ}--Archiv},
  volume    = {Bd. 5},
  pages     = {S.63-75},
  year      = 1983
}

@Book{        peters:83,
  author    = {Peters, U.},
  title     = {{E}mpfangsstrategien f"ur {D}igitalsignalempf"anger im
          {B}asisband},
  publisher = {Dissertation, Universit"at der Bundeswehr M"unchen},
  month     = jul,
  year      = 1983
}

@Book{        peterson:72,
  author    = {W.W. Peterson and E.J. {Weldon, Jr}},
  title     = {Error--Correcting Codes},
  edition   = {second},
  publisher = {{MIT} Press Cambridge, Mass.},
  year      = 1972
}

@Article{     picchi:87,
  author    = {G.~Picchi and G.~Prati},
  title     = {{B}lind {E}qualization and {C}arrier {R}ecovery {U}sing a
          ``{S}top--and--{G}o'' {D}ecision--{D}irected {A}lgorithm},
  journal   = com,
  volume    = {COM-35},
  pages     = {877-887},
  month     = sep,
  year      = 1987
}

@Book{        pierce:80,
  author    = {J.R. Pierce and E.C. Posner},
  title     = {Introduction to Communication Science and Systems},
  publisher = {Plenum Press},
  address   = {New York and London},
  year      = 1980
}

@Article{     pizzi:85,
  author    = {S.V. Pizzi and S.G. Wilson},
  title     = {Convolutional Coding Combined with Continuous Phase
          Modulation},
  journal   = com,
  volume    = {COM-33},
  pages     = {20-29},
  month     = jan,
  year      = 1985
}

@Book{        porombka:89,
  author    = {Porombka, M.},
  title     = {{Z}ur {A}nwendung von {S}elektionsalgorithmen bei
          trelliscodierten, digitalen {"U}bertragungssystemen},
  publisher = {Diplomarbeit, Universit"at der Bundeswehr M"unchen,
          Fakult"at f"ur Elektrotechnik},
  year      = 1989
}

@Book{        portugheis:92,
  author    = {J. Portugheis},
  title     = {{G}eneralized {C}oncatenated {C}odes for {M}-{PSK}
          {M}odulation},
  publisher = {Dissertation, Technische Hochschule Darmstadt},
  month     = jul,
  year      = 1992
}

@Article{     pottie:89,
  author    = {Pottie and Taylor},
  title     = {{M}ultilevel {C}odes based on {P}artitioning},
  journal   = inf,
  volume    = {IT-35},
  pages     = {87-98},
  month     = jan,
  year      = 1989
}

@Article{     pottie:91,
  author    = {G.J.~Pottie and M.V.~Eyubo\v{g}lu},
  title     = {{C}ombined {C}oding and {P}recoding for {PAM} and {QAM}
          {HDSL} {S}ystems},
  journal   = sel,
  volume    = {SAC-9},
  pages     = {861-870},
  month     = aug,
  year      = 1991
}

@Article{     prabhu:74,
  author    = {V.K. Prabhu and H.E. Rowe},
  title     = {Spektra of digital phase modulation by matrix methods},
  journal   = bel,
  volume    = {53},
  pages     = {899-935},
  year      = 1974
}

@TechReport{      pragcode,
  author    = {I.~Tamir},
  title     = {{E}uropean {T}rellis {C}ode {O}ption for {ADSL}},
  type      = {{ETSI} {TM}3, {T}emporary {D}ocument 36},
  address   = {Stockholm},
  month     = apr,
  year      = 1994
}

@Book{        press:88,
  author    = {W.H.~Press et al.},
  title     = {Numerical Recipes in C -- The Art of Scientific
          Computing},
  publisher = {Cambridge University Press},
  address   = {Cambridge},
  year      = 1988
}

@Book{        press:92,
  author    = {W.H.~Press and S.A.~Teukolsky and W.T.~Vetterling and
          B.P.~Flannery},
  title     = {Numerical Recipes in C -- The Art of Scientific
          Computing},
  edition   = {second},
  publisher = {Cambridge University Press},
  address   = {Cambridge},
  year      = 1992
}

@InProceedings{   price:72,
  author    = {R. Price},
  title     = {Nonlinearly feedback equalized {PAM} versus capacity for
          noisy filter channels},
  booktitle = {Proceedings of the International Conference on
          Communications {(ICC'72)}},
  pages     = {},
  month     = jun,
  year      = 1972
}

@Book{        Pri81,
  author    = {M.~B.~Priestley},
  title     = {{S}pectral {A}nalysis and {T}ime {S}eries, {V}olume
          2: {M}ultivariate {S}eries, {P}rediction and
          {C}ontrol},
  publisher = {{A}cademic {P}ress, Inc.},
  address   = {{O}rlando, {F}lorida},
  year      = 1981
}

@InProceedings{   proakis:86,
  author    = {J.G. Proakis and Khazen-Terezia, A.},
  title     = {A Decision-Feedback Tree-Search Algorithm for digital
          Communication through Channels with Intersymbol
          Interference},
  booktitle = {Proceedings of the International Conference on
          Communications (ICC'86)},
  pages     = {1218-1224},
  year      = 1986
}

@Book{        Pro89,
  author    = {J.G. Proakis},
  title     = {Digital Communications},
  publisher = {McGraw--Hill},
  address   = {New York, Second Edition},
  year      = 1989
}

@Book{        Pro95,
  author    = {J.G. Proakis},
  title     = {Digital Communications},
  publisher = {McGraw--Hill},
  address   = {New York},
  edition   = {third},
  year      = 1995
}

@Book{        Pro00,
  author    = {J.G. Proakis},
  title     = {Digital Communications},
  publisher = {McGraw--Hill},
  address   = {New York},
  edition   = {Forth},
  year      = 2000
}

@Book{        pujolle:88,
  author    = {G. Pujolle and D. Seret and D. Dromard and E. Horlait},
  title     = {Integrated Digital Communications Networks},
  note      = {vol.1 and vol.2},
  publisher = wil,
  address   = {New York},
  year      = 1988
}

@Book{        pusl:94,
  author    = {S.~Pusl},
  title     = {{A}daptive {E}ntzerrung mit {M}ehrfachabtastung f\"ur die
          digitale Kabel\"ubertragung mit
          {T}omlinson--{H}arashima--{V}orcodierung},
  publisher = {Diplomarbeit, Lehrstuhl f\"ur Nachrichtentechnik der
          Universit\"at Erlangen-N\"urnberg},
  month     = oct,
  year      = 1994
}

@Article{     Qur73,
  author    = {S.U.H.~Qureshi and E.E.~Newhall},
  title     = {{A}n {A}daptive {R}eceiver for {D}ata {T}ransmission over
          {T}ime-{D}ispersive {C}hannels},
  journal   = inf,
  volume    = {IT-19},
  pages     = {448-457},
  month     = jul,
  year      = 1973
}

@Article{     qureshi:85,
  author    = {S.U.H.~Qureshi},
  title     = {{A}daptive {E}qualization},
  journal   = {Proceedings of the {IEEE}},
  volume    = {73},
  pages     = {1349-1387},
  month     = sep,
  year      = 1985
}

@Article{     Rah95,
  author    = {R.~Raheli and A.~Polydoros and C.-K.~Tzou},
  title     = {{P}er-{S}urvivor {P}rocessing: {A} {G}eneral {A}pproach to
          {MLSE} in {U}ncertain {E}nvironments},
  journal   = com,
  volume    = {COM-43},
  pages     = {354-364},
  month     = feb # "/"  # mar # "/"  # apr,
  year      = 1995
}

@InProceedings{   Rah97,
  author    = {G.~Colavolpe and R.~Raheli},
  title     = {{N}on-{C}oherent {S}equence {D}etection of ${M}$--ary
          {PSK}},
  booktitle = {Proceedings of the International Conference on
          Communications ({ICC}'97)},
  address   = {Montreal},
  pages     = {21-25},
  month     = jun,
  year      = 1997
}

@Article{     Raph96,
  author    = {D.~Raphaeli},
  title     = {{N}oncoherent {C}oded {M}odulation},
  journal   = com,
  volume    = {COM-44},
  pages     = {172-183},
  month     = feb,
  year      = 1996
}

@InProceedings{   rapp:90,
  author    = {Ch. Rapp},
  title     = {Efficient Calculation of the Power Spectral Density of
          Filtered and Nonlinearly Distorted Digital Signals},
  booktitle = {Conf. Record of the {IEEE} Intern. Telecommunications
          Symposium},
  address   = {Rio de Janeiro},
  month     = sep,
  year      = 1990
}

@InProceedings{   rapp:90b,
  author    = {Ch. Rapp},
  title     = {Coded and Uncoded {M--PSK} and {CPM} Signals on Nonlinear
          Bandpa\ss Channels: An Approach to a Fair Comperison},
  booktitle = {Proceedings of the IEEE Global Telecommunication
          Conference ({GLOBECOM}'90)},
  address   = {San Diego},
  pages     = {501.5.1-501.5.5},
  month     = dec,
  year      = 1990
}

@TechReport{      rapp:91,
  author    = {Ch. Rapp},
  title     = {{A}nalyse der nichtlinearen {V}erzerrungen modulierter
          {D}igitalsignale -- {V}ergleich codierter und uncodierter
          {M}odulationsverfahren und {M}ethoden der {K}ompensation
          durch {V}orverzerrung},
  institution   = {VDI Fortschr.--Ber. Reihe 10},
  number    = {Nr. 195},
  address   = {D"usseldorf},
  year      = 1992
}

@Book{        Rap96,
  author    = {T.S.~Rappaport},
  title     = {{W}ireless {C}ommunications},
  publisher = {Prentice Hall},
  address   = {Upper Saddle River, NJ},
  year      = 1996
}

@Book{        rebhan:93,
  author    = {K. Rebhan},
  title     = {{S}chrittweise {D}ecodierung von {M}ehrstufencodes},
  publisher = {Diplomarbeit, Lehrstuhl f\"ur Nachrichtentechnik der
          Universit\"at Erlangen-N\"urnberg},
  month     = oct,
  year      = 1993
}

@Article{     reed:72,
  author    = {L.W.~Brooks and I.S.~Reed},
  title     = {{E}quivalence of the {L}ikelihood {R}atio {P}rocessor, the
          {M}aximum {S}ignal-to-{N}oise {R}atio {F}ilter, and the
          {W}iener {F}ilter},
  journal   = {IEEE Trans.~on Aerospace and Electronic Systems},
  volume    = {AES-8},
  pages     = {690-692},
  month     = sep,
  year      = 1972
}

@Article{     Roh,
  author    = {J.~Roh and B.~Rao},
  title     = {{Transmit Beamforming in Multiple Antenna Systems with Finite Rate Feedback: A VQ-based Approach}},
  journal   = inf,
  volume    = {52},
  pages     = {1101-1112},
  month     = mar,
  year      = 2006
}

@Article{     rimoldi:88,
  author    = {B.E. Rimoldi},
  title     = {A Decomposition Approach to {CPM}},
  journal   = inf,
  volume    = {IT-34},
  pages     = {260-270},
  month     = mar,
  year      = 1988
}

@InProceedings{   rmueller:97,
  author    = {R.~M\"uller and J. Huber},
  title     = {{I}terated {S}oft--{D}ecision {I}nterference
          {C}ancellation for {CDMA}},
  booktitle = {Tyrrhenian International Workshop on Digital
          Communications},
  note      = {Proceedings},
  address   = {Lerici, Italia},
  year      = 1997
}

@Unpublished{     robertson:93,
  author    = {P. Robertson},
  title     = {{I}lluminating the {S}tructure of {D}ecoders for
          {P}arallel {C}oncatenated {R}ecursive {S}ystematic
          ({T}urbo) {C}odes},
  note      = {Submitted for International Conference on Communications
          ({ICC}'94)}
}

@Book{        roden:88,
  author    = {M.S. Roden},
  title     = {Digital Communication Systems Design},
  publisher = pre,
  address   = {Englewood Cliffs, N.J.},
  year      = 1988
}

@InProceedings{   rohrs:95,
  author    = {C.E.~Rohrs},
  title     = {{D}ecision {F}eedback {E}qualization and {C}apacity on the
          {L}inear {S}tationary {G}aussian {C}hannel},
  booktitle = {Proceedings of the IEEE Global Telecommunication
          Conference ({GLOBECOM'95})},
  pages     = {871-873},
  address   = {Singapore},
  month     = nov,
  year      = 1995
}

@Book{        rothlauf:97,
  author    = {F.~Rothlauf},
  title     = {{Impulsverk\"urzung durch Vorfilterung f\"ur die
          Maximum--Likelihood Sequenzsch\"atzung und
          Mehrtr\"ager\"ubertragungsverfahren}},
  publisher = {Diplomarbeit, Lehrstuhl f\"ur Nachrichtentechnik der
          Universit\"at Erlangen-N\"urnberg},
  month     = jan,
  year      = 1997
}

@Article{     rounne:89,
  author    = {M. Rounne and D.J. Costello},
  title     = {An Algorithm for Computing the Distance Spectrum of
          Trelliscodes},
  journal   = sel,
  volume    = {SAC-7},
  pages     = {929-940},
  month     = sep,
  year      = 1989
}

@Book{        rueppel:89,
  author    = {K. A. R\"uppel},
  title     = {{M}ehrstufige {T}relliscodierung},
  publisher = {Diplomarbeit, Institut f\"ur Nachrichtentechnik der
          Universit\"at der Bundeswehr M\"unchen},
  month     = mar,
  year      = 1989
}

@InProceedings{   SST01,
  author    = {A.~Swami and B.~Sadler and J.~Turner},
  title     = {{On the Coexistence of Ultra-Wideband and Narrowband Radio Systems}},
  booktitle = {Proceedings of IEEE Military Communications Conference},
  address   = {Washington},
  pages     = {16-19},
  month     = oct,
  year      = 2001
}

@Article{     sain:68,
  author    = {M.K. Sain and J.L. Massey},
  title     = {Inverses of Linear Sequential Circuits},
  journal   = {IEEE Trans. Computers},
  volume    = {C-17},
  pages     = {330-337},
  year      = 1968
}

@Article{     saleh:81,
  author    = {A.A.M. Saleh},
  title     = {Frequency--Independent and Frequency--Dependent Nonlinear
          Models of {TWT} Amplifiers},
  journal   = com,
  volume    = {COM-29},
  pages     = {},
  month     = nov,
  year      = 1981
}

@Article{     salz:73,
  author    = {J.~Salz},
  title     = {{O}ptimum {M}ean-{S}quared {D}ecision {F}eedback
          {E}qualization},
  journal   = {Bell System Technical Journal},
  volume    = {52},
  pages     = {1341-1373},
  month     = oct,
  year      = 1973
}

@Book{        sam:79,
  author    = {K.S. Shanmugam},
  title     = {Digital and Analog Communication Systems},
  publisher = wil,
  address   = {New York},
  year      = 1979
}


@InProceedings{   samueli:88,
  author    = {H. Samueli},
  title     = {Linear programming design of digital data transmission
          filters with arbitrary magnitude specifications},
  booktitle = {Intern. Commun. Conference (ICC'88)},
  pages     = {30.6.1-30.6.5},
  address   = {Philadelphia},
  month     = jun,
  year      = 1988
}

@Article{     sato:75,
  author    = {Y.~Sato},
  title     = {A {M}ethod of {S}elf-{R}ecovering {E}qualization for
          {M}ultilevel {A}mplitude-{M}odulation},
  journal   = com,
  volume    = {COM-23},
  pages     = {679-682},
  month     = jun,
  year      = 1975
}

@Article{     sauer:87,
  author    = {W. {Sauer, W. Rupprecht}},
  title     = {{E}in aufwandsg"unstiges {D}etektionsverfahren f"ur stark
          verzerrte und gest"orte {D}atensignale},
  journal   = {ntz--Archiv},
  volume    = {Band 9},
  pages     = {155-169},
  year      = 1987
}

@Book{        sauer:89,
  author    = {W.~{Sauer--Greff}},
  title     = {{O}ptimale und suboptimale {E}mpf"anger f"ur verzerrte und
          gest"orte {D}igitalsysteme unter besonderer
          {B}er"ucksichtigung der aufwandsreduzierten {D}etektion
          mittels {M}--{A}lgorithmus},
  publisher = {Dissertation, Universit"at Kaiserslautern},
  month     = jul,
  year      = 1989
}

@Article{     savage:66,
  author    = {Savage, J.E.},
  title     = {Sequential decoding. The computational problem},
  journal   = {Bell System Technical Journal},
  volume    = {45},
  pages     = {149-176},
  year      = 1966
}

@Article{     sayegh:86,
  author    = {S.I. Sayegh},
  title     = {A class of optimum block codes in signal space},
  journal   = com,
  volume    = {COM-34},
  pages     = {1043-1045},
  month     = oct,
  year      = 1986
}

@Book{        schaback:93,
  author    = {R.~Schaback and H.~Werner},
  title     = {Numerische Mathematik},
  publisher = spr,
  address   = {Berlin},
  year      = {1993}
}

@TechReport{      schlegel:90,
  author    = {Ch. Schlegel and A. Frost},
  title     = {A general approach to maximum--likelihood and
          reduced--state decoding},
  institution   = {Asea Brown Boveri Corporate Research},
  type      = {Research Report},
  month     = jul,
  year      = 1990
}

@InProceedings{   Schm98,
  author    = {M.~Schmidt and G.~P.~Fettweis},
  title     = {{FIR prefiltering for near minimum phase target channels}},
  booktitle = {6th Canadian Workshop on Information Theory},
  address   = {},
  month     = jun,
  year      = 1999
}

@Book{        Sch97,
  author    = {R.~Schober},
  title     = {{E}mpfangsverfahren f\"ur den digitalen {M}obilfunk
          nach dem {IS}--54 {S}tandard},
  publisher = {Diplomarbeit, Lehrstuhl f\"ur Nachrichtentechnik der
          Universit\"at Erlangen-N\"urnberg},
  month     = sep,
  year      = 1997
}

@InProceedings{   Sch98,
  author    = {R.~Schober and W.~Gerstacker and J.~Huber},
  title     = {{I}mproving {D}ifferential {D}etection of {MDPSK} by {N}oise {P}rediction},
  booktitle = {Proceedings of Globecom'98},
  address   = {Sydney},
  month     = nov,
  year      = 1998
}
@Article{     Sch98c,
  author    = {R.~Schober and W.~H.~Gerstacker and J.~B.~Huber},
  title     = {{D}ecision--{F}eedback {D}ifferential {D}etection of {MDPSK}
          for {F}lat {R}ayleigh {F}ading {C}hannels},
  journal   = {to be published in {IEEE} {T}rans. on {C}ommun.},
  volume    = {},
  pages     = {},
  month     = jul,
  year      = 1998
}

@Article{     Sch98d,
  author    = {R.~Schober and W.~H.~Gerstacker and J.~B.~Huber},
  title     = {{D}ecision--feedback differential detection
          scheme for 16--{DAPSK}},
  journal   = {{E}lectronics {L}etters},
  volume    = {34},
  pages     = {1812-1813},
  number    = {19},
  month     = sep,
  year      = 1998

}

@Article{     SG01,
  author    = {R.~Schober and W.H.~Gerstacker},
  title     = {{On the Distribution of Zeros of Mobile Channels with Application to GSM/EDGE}},
  journal   = com,
  volume    = {19},
  pages     = {1289-1299},
  month     = jul,
  year      = 2001
}

@Article{     SL02,
  author    = {R.~Schober and L.~Lampe},
  title     = {{Noncoherent Receivers for Differential Space--Time Modulation}},
  journal   = com,
  volume    = {50},
  pages     = {768-777},
  month     = may,
  year      = 2002
}

@InProceedings{   SGL02,
  author    = {R.~Schober and W.H.~Gerstacker and L.H.-J.~Lampe},
  title     = {{Performance Analysis and Design of STBCs for Fading ISI Channels}},
  booktitle = {Proceedings of the International Conference on Communications (ICC)},
  pages     = {1451-1455},
  month     = may,
  year      = 2002
}

@Article{     SHG04,
  author    = {R.~Schober and T.~Hehn and W.~H.~Gerstacker},
  title     = {{Optimized Delay Diversity for Frequency-Selective Fading Channels}},
  journal   = {Accepted for publication in IEEE Transactions on Wireless Communications},
  pages     = {},
  month     = {},
  year      = 2004,
  note      = {The conference version of this paper was presented at the IEEE International
Conference on Communications (ICC), Paris, France, June 2004}
}

@InProceedings{   schreitmueller:86,
  author    = {S. Rasmussen and W. Schreitm"uller},
  title     = {{SMSK} Performance in Nonlinear Satellite Channels},
  booktitle = {Proceedings of the {ICDSC}'86},
  address   = {Munich},
  pages     = {619-626},
  year      = 1986
}

@Book{        schussler:88,
  author    = {H.W.~Sch\"u{\ss}ler},
  title     = {Digitale Signalverarbeitung},
  publisher = spr,
  address   = {Berlin Heidelberg},
  year      = {1988}
}

@Book{        schussler:94,
  author    = {H.W.~Sch\"u{\ss}ler},
  title     = {Digitale Signalverarbeitung 1},
  publisher = spr,
  note      = {4.~Auflage},
  address   = {Berlin Heidelberg New York},
  year      = {1994}
}

@Book{        schwarz:66,
  author    = {Joachim Schwarz},
  title     = {x},
  publisher = {Oldenburg Verlag},
  address   = {{M\"unchen}},
  year      = 1966
}

@Book{        schwarz:88,
  author    = {Joachim Schwarz},
  title     = {{D}igitale {V}erarbeitung stochastischer {S}ignale},
  publisher = {Oldenburg Verlag},
  address   = {{M\"unchen}},
  year      = 1988
}

@Book{        SBS66,
  author    = {M.~Schwartz and W.~Bennett and S.~Stein},
  title     = {{Communication Systems and Techniques}},
  publisher = {McGraw--Hill},
  address   = {{New York}},
  year      = 1966
}

@Article{     sehier:90,
  author    = {P.~Sehier and G.~Kawas Kaleh},
  title     = {{A}daptive equaliser for differentially coherent
          receiver},
  journal   = {IEE Proceedings-I},
  volume    = {137},
  pages     = {9-12},
  month     = feb,
  year      = 1990
}

@ARTICLE{erkip1,
  author    = {A.~Sendonaris and E.~Erkip and B.~Aazhang},
  title     = {{User Cooperation Diversity --- Part I. System Description}},
  journal   = com,
  volume    = {51},
  pages     = {1927-1938},
  month     = nov,
  year      = 2003
}

@ARTICLE{erkip2,
  author    = {A.~Sendonaris and E.~Erkip and B.~Aazhang},
  title     = {{User Cooperation Diversity --- Part II. Implementation Aspects and Performance Analysis}},
  journal   = com,
  volume    = {51},
  pages     = {1939-1948},
  month     = nov,
  year      = 2003
}

@Article{     seshadri:89,
  author    = {N. Seshadri and J.B. Anderson},
  title     = {Decoding of Severly Filtered Modulation Codes Using the
          {(M,L)} Algorithm},
  journal   = sel,
  volume    = {SAC-7},
  pages     = {1006-1016},
  month     = {},
  year      = 1989
}

@Article{     shalvi:90,
  author    = {O.~Shalvi and E.~Weinstein},
  title     = {{N}ew {C}riteria for {B}lind {D}econvolution of
          {N}onminimum {P}hase {S}ystems ({C}hannels)},
  journal   = inf,
  volume    = {IT-36},
  pages     = {312-321},
  month     = mar,
  year      = 1990
}

@Article{     Sha96,
  author    = {S.~Shamai (Shitz) and R.~Laroia},
  title     = {{{T}he {I}ntersymbol {I}nterference {C}hannel: {L}ower {B}ounds on
          {C}apacity and {C}hannel {P}recoding {L}oss}},
  journal   = inf,
  volume    = {IT-42},
  pages     = {1388-1404},
  month     = sep,
  year      = 1996
}

@Article{     shannon:48,
  author    = {C.E. Shannon},
  title     = {A Mathematical Theory of Communication},
  journal   = {Bell System Technical Journal},
  volume    = {27},
  pages     = {part I, pp. 379-427; part II, pp. 623-656},
  year      = 1948
}

@Article{     shannon:49,
  author    = {C.E. Shannon},
  title     = {Communication in the Presence of Noise},
  journal   = {Proceedings of the {IRE}},
  volume    = {37},
  pages     = {10-21},
  month     = jan,
  year      = 1949
}

@Article{     SFGK00,
  author    = {D.-S.~Shiu and G.J.~Foschini and M.J.~Gans and J.M.~Kahn},
  title     = {{Fading Correlation and Its Effect on the Capacity of Multielement Antenna Systems}},
  journal   = com,
  volume    = {COM-48},
  pages     = {502-513},
  month     = mar,
  year      = 2000
}

@Article{     SHHS01,
  author    = {A.~Shokrollahi and B.~Hassibi and B.M.~Hochwald and W.~Sweldens},
  title     = {{Representation Theory for High-Rate Multiple-Antenna Code Design}},
  journal   = inf,
  volume    = {IT-47},
  pages     = {2335-2367},
  month     = sep,
  year      = 2001
}

@InProceedings{   simon:87,
  author    = {M.K. Simon and D. Divsalar},
  title     = {The performance of trellis--coded multilevel {DPSK} on a
          fading mobile satellite channel},
  booktitle = {Proceedings of the Int. Conf. on Communications
          ({ICC}'87)},
  pages     = {21.2.1-21.2.7},
  year      = 1987
}

@Article{     SA98,
  author    = {M.K.~Simon and M.-S.~Alouini},
  title     = {{A Unified Analysis to the Performance Analysis of Digital Communication over Generalized Fading Channels}},
  journal   = {Proceedings of the IEEE},
  volume    = {86},
  pages     = {1860-1877},
  month     = sep,
  year      = 1998
}

@Book{        sklar:88,
  author    = {Bernard Sklar},
  title     = {Digital Communications, Fundamentals and Applications},
  publisher = pre,
  address   = {Englewood Cliffs, New Jersey},
  year      = {1988}
}

@Article{     sloane:84,
  author    = {N.J.A. Sloane},
  title     = {The packing of spheres},
  journal   = {Scientific American},
  volume    = {250},
  pages     = {116-125},
  month     = jan,
  year      = 1984
}

@InProceedings{   slock:94,
  author    = {D.T.M.~Slock},
  title     = {{B}lind {F}ractionally--{S}paced {E}qualization,
          {P}erfect--{R}econstruction {F}ilter {B}anks and
          {M}ultichannel {L}inear {P}rediction},
  booktitle = {Proceedings of ICASSP'94},
  pages     = {IV-585-IV-588},
  month     = apr,
  address   = {Adelaide},
  year      = 1994
}

@InProceedings{   slock:95,
  author    = {D.T.M.~Slock and C.B.~Papadias},
  title     = {{F}urther {R}esults on {B}lind {I}dentification and
          {E}qualization of {M}ultiple {FIR} {C}hannels},
  booktitle = {Proceedings of ICASSP'95},
  pages     = {1964-1967},
  month     = may,
  address   = {Detroit},
  year      = 1995
}

@Manual{      SMG2,
  title     = {{GSM} {R}ecommendation 05.04: ``{I}ntroduction of {8PSK}'', {V}ers.~5.01, {R}elease 1999, {S}ource {E}ricsson}
}

@Article{     soeder:77,
  author    = {H. {Marko, K. Tr"ondle, G. S"oder}},
  title     = {{V}ergleich optimaler, bin"arer und mehrstufiger
          {R}egenerativverst"arkersysteme f"ur koaxiale {K}abel bei
          symmetrischer {I}mpulsform unter {B}er"ucksichtigung der
          {T}oleranzen},
  journal   = {NTZ},
  volume    = {29 und 30},
  pages     = {S.601-608 und S.316-323},
  year      = {1976,1977}
}

@Book{        soeder:85,
  author    = {G. {S"oder, K. Tr"ondle}},
  title     = {{D}igitale {"U}bertragungsysteme},
  publisher = {Springer Verlag},
  address   = {Berlin, Heidelberg},
  year      = 1985
}

@Article{     Sol90,
  author    = {N.~R.~Sollenberger and J.~C.--I.~Chuang},
  title     = { {L}ow--{O}verhead {S}ymbol {T}iming and {C}arrier {R}ecovery
          for {TDMA} {P}ortable {R}adio {S}ystems},
  journal   = com,
  volume    = {COM-38},
  pages     = {1886-1892},
  month     = oct,
  year      = 1990
}

@InProceedings{   spihu:95,
  author    = {B.~Spinnler and J.~Huber},
  title     = {{D}esign of {H}yper {S}tates for {R}educed-{S}tate
          {S}equence {E}stimation},
  booktitle = {Proceedings of the International Conference on
          Communications ({ICC}'95)},
  pages     = {1-6},
  address   = {Seattle},
  month     = jun,
  year      = 1995
}

@Book{        spilker:77,
  author    = {J.J. Spilker Jr.},
  title     = {Digital Communications by Satellite},
  publisher = pre,
  address   = {Englewood Cliffs, N.J.},
  year      = 1977
}

@Book{        spinnler:94,
  author    = {B.~Spinnler},
  title     = {{Z}ustandsreduktion bei {E}mpf"angern f"ur die digitale
          {PAM}--"Ubertragung mit {I}mpulsinterferenzen},
  publisher = {Diplomarbeit, Lehrstuhl f\"ur Nachrichtentechnik der
          Universit\"at Erlangen-N\"urnberg},
  month     = feb,
  year      = 1994
}

@Article{     steele:94,
  author    = {J.C.S.~Cheung and R.~Steele},
  title     = {{S}oft-{D}ecision {F}eedback {E}qualizer for {C}ontinuous
          {P}hase {M}odulated {S}ignals in {W}ideband {M}obile
          {R}adio {C}hannels},
  journal   = com,
  volume    = {COM-42},
  pages     = {1628-1638},
  month     = feb # "/"  # mar # "/"  # apr,
  year      = 1994
}

@Article{     Ste82,
  author    = {K.~Steiglitz and B.~Dickinson},
  title     = {{Phase Unwrapping by Factorization}},
  journal   = assp,
  volume    = {ASSP-30},
  pages     = {984-991},
  month     = dec,
  year      = 1982
}

@Book{        stoeger:97,
  author    = {M.~St{\"o}ger},
  title     = {{S}ynchronisation f\"ur digitale
          Basisband\"ubertragungssysteme mit \"uberabgetasteter
          entscheidungsr\"uckgekoppelter Entzerrung},
  publisher = {Diplomarbeit, Lehrstuhl f\"ur Nachrichtentechnik der
          Universit\"at Erlangen-N\"urnberg},
  month     = mar,
  year      = 1997
}

@Article{     SH03,
  author    = {T.~Strohmer and R.W.~{Heath Jr.}},
  title     = {{Grassmannian Frames with Applications to Coding and Communications}},
  journal   = {Applied and Computational Harmonic Analysis},
  volume    = {14},
  pages     = {257-275},
  month     = {},
  year      = 2003
}

@Article{     sund:86,
  author    = {C-E. Sundberg},
  title     = {Continuous Phase Modulation},
  journal   = {IEEE Commun. Magazine},
  volume    = {24},
  pages     = {25-38},
  month     = apr,
  year      = 1986
}

@InCollection{    sund:89,
  author    = {C.-E. Sundberg},
  title     = {Combined Channel Coding and Constant Amplitude Continuous
          Phase Modulation},
  booktitle = {Topics in Coding Theory},
  editor    = {G. Einarsson e.a.},
  publisher = {Springer--Verlag},
  address   = {Berlin},
  year      = 1989
}

@Article{     sund:91,
  author    = {J.B. Anderson and C.-E. Sundberg},
  title     = {Advances in Constant Envelope Coded Modulation},
  journal   = cma,
  volume    = {29},
  pages     = {36-45},
  month     = dec,
  year      = 1991
}

@InProceedings{   Suz94,
  author    = {T.~Suzuki and T.~Mizuno},
  title     = {{M}ultiple--{S}ymbol {D}ifferential {D}etection {S}cheme for
          {D}ifferential {A}mplitude {M}odulation},
  booktitle = {Proceedings of {IZS}'94 ({I}nternational {Z}urich {S}eminar
          on {D}igital {C}ommunications},
  pages     = {326-337},
  month     = mar,
  address   = {Zurich},
  year      = 1994
}

@Article{     svensson:84,
  author    = {A. Svensson and T. Aulin and C.-E. Sundberg},
  title     = {A Class of Reduced Complexity Viterbi Detectors for
          Partial Response Continuous Phase Modulation},
  journal   = com,
  volume    = {COM-32},
  pages     = {1079-1087},
  month     = {},
  year      = 1984
}

@Article{     Sve94,
  author    = {A.~Svensson},
  title     = {{C}oherent detection based on linear prediction and decision feedback for {QDPSK}},
  journal   = {Electronics {L}etters},
  volume    = {30},
  pages     = {1642-1643},
  number    = {20},
  year      = 1994
}

@Article{     Sve95,
  author    = {N.~A.~Svensson},
  title     = {On {D}ifferentially {E}ncoded {S}tar 16{QAM} with {D}ifferential {D}etection and {D}iversity},
  journal   = veh,
  volume    = {44},
  pages     = {586-593},
  month     = aug,
  year      = 1995
}

@InProceedings{   TMB04,
  author    = {P.~Tarasak and H.~Minn and V.K.~Bhargava},
  title     = {{Differential Modulation for Two-User Cooperative Diversity Systems}},
  booktitle = {Proceedings of the Global Telecommunications Conference (GLOBECOM)},
  pages     = {},
  address   = {Dallas},
  month     = dec,
  year      = 2004
}

@InProceedings{   tarkoey:95,
  author    = {F.~Tark\"oy},
  title     = {{MMSE}-{O}ptimal {F}eedback and its {A}pplications},
  booktitle = {Proceedings of ISIT'95},
  pages     = {334},
  address   = {Whistler, B.C.},
  month     = sep,
  year      = 1995
}

@Article{     TSC98,
  author    = {V.~Tarokh and N.~Seshadri and A.R.~Calderbank},
  title     = {{Space--Time Codes for High Data Rate Wireless Communication: Performance Criterion and Code Construction}},
  journal   = inf,
  volume    = {IT-44},
  pages     = {744-765},
  month     = mar,
  year      = 1998
}

@Article{     TJC99,
  author    = {V.~Tarokh and H.~Jafarkhani and A.R.~Calderbank},
  title     = {{Space--Time Block Codes from Orthogonal Designs}},
  journal   = inf,
  volume    = {IT-45},
  pages     = {1456-1467},
  month     = jul,
  year      = 1999
}

@Article{     TNSC99,
  author    = {V.~Tarokh and A.~Naguib and N.~Seshadri and A.R.~Calderbank},
  title     = {{Space--Time Codes for High Data Rate Wireless Communication: Performance Criteria in the Presence of Channel Estimation Errors, Mobility, and Multiple Paths}},
  journal   = com,
  volume    = {47},
  pages     = {199-207},
  month     = feb,
  year      = 1999
}

@Article{     TJ00,
  author    = {V.~Tarokh and H.~Jafarkhani},
  title     = {{A Differential Detection Scheme for Transmit Diversity}},
  journal   = sel,
  volume    = {SAC-18},
  pages     = {1169-1174},
  month     = jul,
  year      = 2000
}

@Book{        taub:71,
  author    = {Herbert Taub and Donald L. Schilling},
  title     = {Principles of Communication Systems},
  publisher = {McGraw--Hill},
  address   = {Tokyo},
  year      = 1971
}

@Article{     taylor:73,
  author    = {D.P.~Taylor},
  title     = {{T}he {E}stimate {F}eedback {E}qualizer: {A} {S}uboptimum
          {N}onlinear {R}eceiver},
  journal   = com,
  volume    = {COM-21},
  pages     = {979-990},
  month     = sep,
  year      = 1973
}

@InProceedings{   teich:96,
  author    = {W.G.~Teich and M.~Seidl},
  title     = {{C}ode {D}ivision {M}ultiple {A}ccess {C}ommunications:
          {M}ultiuser {D}etection based on a {R}ecurrent {N}eural
          {N}etwork {S}tructure},
  booktitle = {Proceedings of the Fourth International Symposium on
          Spread Spectrum Techniques and Applications (ISSSTA'96)},
  address   = {Mainz},
  month     = sep,
  pages     = {979-984},
  year      = 1996
}

@Article{     TH02,
  author    = {O.~Tirkkonen and A.~Hottinen},
  title     = {{Square-Matrix Embeddable Space-Time Block Codes for Complex Signal Constellations}},
  journal   = inf,
  volume    = {IT-48},
  pages     = {384-395},
  month     = feb,
  year      = {2002}
}

@TechReport{      titsworth:61,
  author    = {R.C. Titsworth and L.R. Welch},
  title     = {Power spectra of signals modulated by random and
          pseudorandom sequences},
  institution   = {Jet Propulsion Lab.},
  address   = {Pasadena/CA},
  type      = {{T}ech. {R}ep.},
  month     = oct,
  year      = {1961}
}

@Article{     tomlinson:72,
  author    = {M.~Tomlinson},
  title     = {{New Automatic Equaliser Employing Modulo Arithmetic}},
  journal   = {Electron. Lett.},
  volume    = {7},
  pages     = {138-139},
  month     = mar,
  year      = 1971
}

@Article{     tong:94,
  author    = {L.~Tong and G.~Xu and T.~Kailath},
  title     = {{B}lind {I}dentification and {E}qualization {B}ased on
          {S}econd--{O}rder {S}tatistics: {A} {T}ime {D}omain
          {A}pproach},
  journal   = inf,
  volume    = {IT-40},
  pages     = {340-349},
  month     = mar,
  year      = 1994
}

@Article{     tong:95,
  author    = {L.~Tong and G.~Xu and B.~Hassibi and T.~Kailath},
  title     = {{B}lind {C}hannel {I}dentification {B}ased on
          {S}econd--{O}rder {S}tatistics: {A} {F}requency {D}omain
          {A}pproach},
  journal   = inf,
  volume    = {IT-41},
  pages     = {329-334},
  month     = jan,
  year      = 1995
}

@Article{     tong:95b,
  author    = {L.~Tong},
  title     = {{B}lind {S}equence {E}stimation},
  journal   = com,
  volume    = {COM-43},
  pages     = {2986-2994},
  month     = dec,
  year      = 1995
}

@Book{        trees:68,
  author    = {{H.L. van} Trees},
  title     = {Detection, Estimation, and Modulation Theory, {\rm Part
          {I} -- Part {III}}},
  publisher = wil,
  address   = {New York},
  year      = {1968,1971,1971}
}

@Article{     treichler:83,
  author    = {J.R.~Treichler and B.G.~Agee},
  title     = {{A} {N}ew {A}pproach to {M}ultipath {C}orrection of
          {C}onstant {M}odulus {S}ignals},
  journal   = assp,
  volume    = {ASSP-31},
  pages     = {459-472},
  month     = apr,
  year      = 1983
}

@Book{        tretter:76,
  author    = {S. Tretter},
  title     = {Introduction to Discrete--Time Signal Processing},
  publisher = {Wiley},
  address   = {New York},
  year      = 1976
}

@Article{     TDHS04,
  author    = {J.A.~Tropp and I.S.~Dhillon and R.W.~{Heath Jr.} and T.~Strohmer},
  title     = {{Designing Structured Thight Frames via an Alternating Projection Method}},
  journal   = {Accepted for Publication in the IEEE Transactions on Information Theory,
available at: http://www.ece.utexas.edu/\~rheath/papers/2003/struct\_tight\_frame/paper.pdf},
  volume    = {},
  pages     = {},
  month     = {},
  year      = 2004
}

@InProceedings{   trumpis:77,
  author    = {B.D. Trumpis and P.L. McAdam},
  title     = {Performance of Convolutional Codes on Burst Noise
          Channels},
  booktitle = {Proc. of the {NTC}-77},
  pages     = {36:3-1 -- 36:3-14},
  address   = {Los Angeles},
  year      = 1977
}

@Article{     tugnait:92,
  author    = {J.K.~Tugnait},
  title     = {{C}omments on ``{N}ew {C}riteria for {B}lind
          {D}econvolution of {N}onminimum {P}hase {S}ystems
          ({C}hannels)''},
  journal   = inf,
  volume    = {IT-38},
  pages     = {210-213},
  month     = jan,
  year      = 1992
}

@InProceedings{   tugnait:93,
  author    = {J.K.~Tugnait},
  title     = {{O}n {B}lind {I}dentifiability {O}f {M}ultipath {C}hannels
          {U}sing {F}ractional {S}ampling {A}nd {S}econd--{O}rder
          {S}tatistics},
  booktitle = {Proceedings of the IEEE Global Telecommunication
          Conference (GLOBECOM'93)},
  address   = {Houston},
  pages     = {2001-2005},
  month     = nov # "/"  # dec,
  year      = 1993
}

@InProceedings{   tugnait:94,
  author    = {J.K.~Tugnait},
  title     = {{A} {P}arallel {M}ultimodel {CMA}/{G}odard {A}daptive
          {F}ilter {B}ank {A}pproach {T}o {F}ractionally--{S}paced
          {B}lind {A}daptive {E}qualization},
  booktitle = {Proceedings of the International Conference on
          Communications (ICC'94)},
  pages     = {549-553},
  address   = {New Orleans},
  month     = may,
  year      = 1994
}

@Article{     tugnait:96,
  author    = {J.K.~Tugnait},
  title     = {{O}n {F}ractionally {S}paced {B}lind {A}dapitve
          {E}qualization {U}nder {S}ymbol {T}iming {O}ffsets {U}sing
          {G}odard and {R}elated {E}qualizers},
  journal   = sip,
  volume    = {44},
  pages     = {1817-1821},
  month     = jul,
  year      = 1996
}

@Book{        unbehauen:93,
  author    = {A.~Cichocki and R.~Unbehauen},
  title     = {{N}eural {N}etworks for {O}ptimization and {S}ignal
          {P}rocessing},
  publisher = teu,
  address   = {Stuttgart},
  year      = 1993
}

@Article{     unbehauen:95,
  author    = {M.-Y.~Zou and R.~Unbehauen},
  title     = {{G}reatest {C}ommon {D}ivisor {A}lgorithms and {B}lind
          {D}econvolution},
  journal   = {International Journal of Electronics and Communications
          (AE\"U)},
  volume    = {49},
  pages     = {160-169},
  number    = {3},
  year      = {1995}
}

@Article{     ungerboeck:72,
  author    = {Ungerb{\"o}ck, G.},
  title     = {{T}heory on the {S}peed of {C}onvergence in {A}daptive
          {E}qualizers for {D}igital {C}ommunication},
  journal   = {IBM Journal on Research and Development},
  volume    = {16},
  pages     = {546-555},
  month     = nov,
  year      = 1972
}

@Article{     Ung74,
  author    = {G. Ungerb{\"o}ck},
  title     = {Adaptive maximum--likelihood receiver for
          carrier--modulated data--transmission systems},
  journal   = com,
  volume    = {COM-22},
  pages     = {624-636},
  year      = 1974
}

@InProceedings{   ungerboeck:76,
  author    = {G. Ungerb\"ock and I. Csajka},
  title     = {On improving data--link performance by increasing channel
          alphabet and introducing sequence coding},
  booktitle = {Int. Sym. Inform. Theory},
  address   = {Ronneby, Sweden},
  month     = jun,
  year      = 1976
}

@Article{     ungerboeck:76b,
  author    = {G.~Ungerb{\"o}ck},
  title     = {{F}ractional {T}ap--{S}pacing {E}qualizer and
          {C}onsequences for {C}lock {R}ecovery in {D}ata {M}odems},
  journal   = com,
  volume    = {24},
  pages     = {856-864},
  month     = aug,
  year      = 1976
}

@Article{     ungerboeck:82,
  author    = {G. Ungerb\"ock},
  title     = {Channel coding with multilevel/phase signals},
  journal   = inf,
  volume    = {IT-28},
  pages     = {55-67},
  month     = jan,
  year      = 1982
}

@Article{     ungerboeck:87a,
  author    = {G. Ungerb{\"o}ck},
  title     = {{T}rellis--{C}oded {M}odulation with {R}edundant {S}ignal
          {S}ets, {P}art {I}},
  journal   = {IEEE Commun. Mag.},
  volume    = {25},
  pages     = {5-11},
  month     = feb,
  year      = 1987
}

@Article{     ungerboeck:87b,
  author    = {G. Ungerb{\"o}ck},
  title     = {{T}rellis--{C}oded {M}odulation with {R}edundant {S}ignal
          {S}ets, {P}art {II}},
  journal   = {IEEE Commun. Mag.},
  volume    = {25},
  pages     = {12-21},
  month     = feb,
  year      = 1987
}

@Article{     ungerboeck:90,
  author    = {Pietrobon, S.S. and Deng, R.H. and Lafanech\'ere and
          Ungerboeck, G. and Costello, D.J.},
  title     = {Trellis--Coded Multidimensional Phase Modulation},
  journal   = inf,
  volume    = {IT-36},
  pages     = {63-89},
  month     = {},
  year      = 1990
}

@Article{     ungerboeck:97,
  author    = {G.~Cherubini and S.~{\"O}l\c{c}er and G.~Ungerb{\"o}ck and
          J.~Creigh and S.K.~Rao},
  title     = {{100Base-T2: A New Standard for 100 Mb/s Ethernet
          Transmission over Voice-Grade Cables}},
  journal   = cma,
  volume    = {35},
  number    = {11},
  pages     = {115-122},
  month     = nov,
  year      = 1997
}

@Article{     ungerboeck_ges:87,
  author    = {G. Ungerb{\"o}ck},
  title     = {{T}rellis--{C}oded {M}odulation with {R}edundant {S}ignal
          {S}ets, {P}arts {I} and {II}},
  journal   = {IEEE Commun. Mag.},
  volume    = {25},
  pages     = {5-21},
  month     = feb,
  year      = 1987
}

@Book{        VT02,
  author    = {H.L.~{Van Trees}},
  title     = {Optimum Array Processing},
  publisher = {Wiley},
  address   = {New York},
  year      = {2002}
}

@Article{     VE76,
  author    = {W.~{Van Etten}},
  title     = {{Maximum--Likelihood Receiver for Multiple Channel Transmission Systems}},
  journal   = com,
  volume    = {COM-76},
  pages     = {276-283},
  month     = feb,
  year      = 1976
}

@Article{     vannfo:91,
  author    = {G.~Vannucci and G.J.~Foschini},
  title     = {{T}he {M}inimum {D}istance for {D}igital {M}agnetic
          {R}ecording {P}artial {R}esponses},
  journal   = inf,
  volume    = {IT-37},
  pages     = {955-960},
  month     = may,
  year      = 1991
}

@InProceedings{   vermeulen:74,
  author    = {Vermeulen, F.L. and Hellmann, M.E.},
  title     = {Reduced state Viterbi decoders for channels with
          intersymbol interference},
  booktitle = {IEEE International Conference on Communications
          ({ICC}'74)},
  address   = {Minneapolis},
  pages     = {37B1-4},
  month     = jun,
  year      = 1974
}

@Article{     Vis97,
  author    = {M.~Visintin},
  title     = {{Differential PSK Block Demodulation over a Flat
          Correlated Rayleigh--Fading Channel}},
  journal   = com,
  volume    = {COM-45},
  pages     = {9-11},
  month     = jan,
  year      = 1997
}

@Article{     VB00,
  author    = {R.~Visoz and E.~Bejjani},
  title     = {{Matched Filter Bound for Multichannel Diversity Over Frequency--Selective Rayleigh Fading Mobile Channels}},
  journal   = veh,
  volume    = {49},
  pages     = {1832-1845},
  month     = sep,
  year      = 2000
}

@Book{        viterbi:66,
  author    = {Andrew J. Viterbi},
  title     = {Principles of Coherent Communication},
  publisher = {McGraw--Hill},
  address   = {New York},
  year      = 1966
}

@Article{     viterbi:67,
  author    = {Viterbi, A.J.},
  title     = {Error bounds for convolutional codes and an asymptotically
          optimum decoding algorithm},
  journal   = inf,
  volume    = {IT-13},
  pages     = {260-269},
  year      = 1967
}

@Article{     viterbi:71,
  author    = {Viterbi, A.J.},
  title     = {Convolutional Codes and Their Performance in Communication
          Systems},
  journal   = com,
  volume    = {COM-19},
  pages     = {751-772},
  month     = oct,
  year      = 1971
}

@Book{        viterbi:79,
  author    = {A.J. Viterbi and J.K. Omura},
  title     = {Principles of Digital Communication and Coding},
  publisher = {McGraw--Hill},
  address   = {New York},
  year      = {1979}
}

@Article{     Vit95,
  author    = {G.~M.~Vitetta and D.~P.~Taylor},
  title     = {{V}iterbi {D}ecoding of {D}ifferentially {E}ncoded {PSK}
          {S}ignals {T}ransmitted over {R}ayleigh {F}requency--{F}lat {F}ading {C}hannels},
  journal   = com,
  volume    = {COM-43},
  pages     = {1256-1259},
  month     = {Feb-Apr},
  year      = 1995
}

@Book{        Vla64,
  author    = {V.~S.~Vladimirov},
  title     = {{Methods of the Theory of Functions of Many Complex Variables}},
  publisher = {M.I.T.~Press},
  address   = {Cambridge, Massachusetts},
  year      = {1964}
}

@Article{     voois:96,
  author    = {P.A.~Voois and I.~Lee and J.M.~Cioffi},
  title     = {{T}he {E}ffect of {D}ecision {D}elay in {F}inite-{L}ength
          {D}ecision {F}eedback {E}qualization},
  journal   = inf,
  volume    = {IT-42},
  pages     = {618-621},
  month     = mar,
  year      = 1996
}

@Unpublished{     wachsmann:94,
  author    = {U. Wachsmann},
  title     = {{M}ehrstufencodierung mit {T}urbocodes},
  note      = {Diplomarbeit, Lehrstuhl f\"ur Nachrichtentechnik der
          Universit\"at Erlangen-N\"urnberg, Abschlu\ss\
          voraussichtlich Feb. 1994}
}

@Article{     wafihu:98,
  author    = {U.~Wachsmann and R.~Fischer and J.~Huber},
  title     = {{Multilevel--Codes: Theoretical Concepts and Practical
          Design Rules}},
  journal   = inf,
  note      = {Accepted for publication},
  year      = 1998
}

@Book{        walke:87,
  author    = {B. Walke},
  title     = {{D}atenkommunikation, {\rm Teil 1 und Teil 2}},
  publisher = {H"uthig},
  address   = {Heidelberg},
  year      = 1987
}

@Article{     Web91,
  author    = {W.~T.~Webb and L.~Hanzo and R.~Steele},
  title     = {Bandwidth efficient {QAM} schemes for {R}ayleigh fading channels},
  journal   = {Proceedings of the {IEEE}},
  volume    = {138},
  pages     = {169-175},
  month     = jun,
  year      = 1991
}

@Book{        Web94,
  author    = {W.~T.~Webb and L.~Hanzo},
  title     = {{M}odern {Q}uadrature {A}mplitude {M}odulation},
  publisher = {Pentech Press},
  address   = {London},
  year      = 1994
}

@Book{        weber:97,
  author    = {R. Weber},
  title     = {{E}insatz von fehlerkorrigierenden {B}lock--{C}odes in der
          codierten {M}odulation},
  publisher = {Diplomarbeit, Lehrstuhl f\"ur Nachrichtentechnik der
          Universit\"at Erlangen-N\"urnberg},
  month     = mar,
  year      = 1997
}

@Book{        Web98,
  author    = {M.~Weber},
  title     = {Entscheidungsr\"uckgekoppelte differentielle
          Detection von MDPSK bei Rice--Fading},
  publisher = {Studienarbeit, Lehrstuhl f\"ur Nachrichtentechnik der
          Universit\"at Erlangen-N\"urnberg},
  address   = {Erlangen},
  year      = 1998
}

@Article{     wei:84a,
  author    = {L.-F. Wei},
  title     = {{Rotationally invariant convolutional channel coding with
          expanded signal space --- Part {I}: 180 degrees}},
  journal   = sel,
  volume    = {SAC-2},
  pages     = {659-671},
  month     = sep,
  year      = 1984
}

@Article{     wei:84b,
  author    = {L.-F. Wei},
  title     = {{Rotationally invariant convolutional channel coding with
          expanded signal space --- Part {II}: Nonlinear codes}},
  journal   = sel,
  volume    = {SAC-2},
  pages     = {672-686},
  month     = sep,
  year      = 1984
}

@Article{     wei:87,
  author    = {L.-F. Wei},
  title     = {{Trellis-Coded Modulation with Multidimensional
          Constellations}},
  journal   = inf,
  volume    = {IT-33},
  pages     = {483-501},
  month     = jul,
  year      = 1987
}

@Article{     Wei97,
  author    = {R.~Y.~Wei and M.~C.~Lin},
  title     = {{D}ifferential {P}hase {D}etection {U}sing {R}ecursively {G}enerated {P}hase {R}eferences},
  journal   = com,
  volume    = {COM-97},
  pages     = {1504-1507},
  month     = dec,
  year      = 1997
}

@Article{     Wei98,
  author    = {R.--Y.~Wei and M.--C.~Lin},
  title     = {Modified decision feedback differential detection
          for differentially encoded 16 {APSK} signals},
  journal   = {Electronics Letters},
  volume    = {34},
  pages     = {336-337},
  number    = {4},
  year      = 1998
}

@Book{        weidinger:93,
  author    = {J.~Weidinger},
  title     = {{E}ntzerrung f\"ur digitale {\"U}bertragungsverfahren mit
          {T}omlinson--{H}arashima--{V}orcodierung},
  publisher = {Diplomarbeit, Lehrstuhl f\"ur Nachrichtentechnik der
          Universit\"at Erlangen-N\"urnberg},
  month     = may,
  year      = 1993
}

@InProceedings{   weinrichter:98,
  author    = {W.~Pusch and H.~Weinrichter},
  title     = {{Improvements of Data Transmission on ISI Channels by
          Means of Channel Matched $m$--ary PAM--Trellis Codes}},
  booktitle = {Proceedings of the International Z{\"u}rich Seminar},
  pages     = {253-257},
  address   = {Z{\"u}rich},
  month     = feb,
  year      = 1998
}

@Article{     well:89,
  author    = {H.-W. Wellhausen},
  title     = {{E}igenschaften symmetrischer {K}abel der {O}rtsnetze und
          generelle \"{U}ber\-tra\-gungs\-m\"og\-lich\-keiten},
  journal   = {Der Fernmelde-Ingenieur},
  volume    = {43.Jahrgang/Heft 10/11},
  pages     = {1-51},
  month     = oct # ","  # nov,
  year      = {1989}
}

@Article{     wellang:89,
  author    = {H.-W. Wellhausen},
  title     = {{E}igenschaften symmetrischer {K}abel der {O}rtsnetze und
          generelle \"{U}ber\-tra\-gungs\-m\"og\-lich\-keiten},
  journal   = {Der Fernmelde-Ingenieur},
  volume    = {43.Jahrgang/Heft 10/11},
  pages     = {1-51},
  month     = oct # ","  # nov,
  note      = {(in German)},
  year      = {1989}
}

@Article{     wellhausen:95,
  author    = {H.-W.~Wellhausen},
  title     = {{Neue Nutzungsm{\"o}glichkeiten vorhandener
          Kupferanschlu{\ss}netze}},
  journal   = ntz,
  number    = {4},
  pages     = {18-27},
  year      = 1995
}

@Article{     wen:90,
  author    = {Wen, K.A. and Wen, T.S. and Wang, J.F.},
  title     = {A New Transform Algorithm for Viterbi Decoding},
  journal   = com,
  volume    = {COM-38},
  pages     = {764-772},
  month     = {},
  year      = 1990
}

@Book{        whalen:71,
  author    = {A.D. Whalen},
  title     = {Detection of Signals in Noise},
  publisher = {Academic Press},
  address   = {New York},
  year      = 1971
}

@Book{        wicker:94,
  author    = {S.B. Wicker and V.K. Bhargava (Editors)},
  title     = {{R}eed--{S}olomon {C}odes and {T}heir {A}pplications},
  publisher = {IEEE Press},
  address   = {New York},
  year      = 1994
}

@InProceedings{   widrow:60,
  author    = {B.~Widrow and M.E.~{Hoff, Jr.}},
  title     = {{Adaptive Switching Circuits}},
  booktitle = {Proceedings of IRE WESCON},
  pages     = {96-104},
  year      = 1960
}

@Book{        williams:78,
  author    = {F.J. MacWilliams and N.J.A. Sloane},
  title     = {The Theory of Error--Correcting Codes},
  publisher = {North--Holland},
  address   = {Amsterdam},
  year      = 1978
}

@InProceedings{   wilson:84b,
  author    = {S.G. Wilson and H.A. Sleeper and N.K. Srinath},
  title     = {Four--Dimensional Modulation and Coding: An Alternative to
          Frequency Reuse},
  booktitle = {ICC Conference Record},
  address   = {Amsterdam},
  year      = 1984
}

@Article{     wilson:86,
  author    = {S.G. Wilson},
  title     = {Rate 5/6 Trelliscoded 8{PSK}},
  journal   = com,
  volume    = {COM-34},
  pages     = {1045-1049},
  month     = oct,
  year      = 1986
}

@InProceedings{   Wit93,
  author    = {A.~Wittneben},
  title     = {{A New Bandwidth Efficient Transmit Antenna Modulation Diversity Scheme for Linear Digital Modulation}},
  booktitle = {Proceedings of the IEEE International Communications Conference},
  pages     = {1630-1634},
  address   = {Geneva},
  month     = may,
  year      = 1993
}

@InProceedings{   woerz:90,
  author    = {T. W\"orz and J. Hagenauer},
  title     = {Multistage Coding and Decoding},
  booktitle = {Proceedings of the IEEE Global Telecommunication
          Conference (GLOBECOM'90)},
  address   = {San Diego},
  pages     = {501.1.1-501.1.6},
  month     = dec,
  year      = 1990
}

@InProceedings{   woerz:92,
  author    = {T. Woerz and J. Hagenauer},
  title     = {{I}terative {D}ecoding for {M}ultilevel {C}odes using
          {R}eliability {I}nformation},
  booktitle = {Proceedings of the IEEE Global Telecommunication
          Conference (GLOBECOM'92)},
  address   = {Orlando},
  month     = dec,
  year      = 1992
}

@Article{     woerz:93,
  author    = {T. Woerz and J. Hagenauer},
  title     = {{D}ecoding of {M}-{PSK}-multilevel codes},
  journal   = {European Transactions on Telecommunications},
  volume    = {4},
  pages     = {65-74},
  month     = may # "-"  # jun,
  year      = 1993
}

@Article{     wolf:76,
  author    = {J.L. Wolf},
  title     = {Efficient Maximum Likelihood Decoding of Linear Block
          Codes Using a Trellis},
  journal   = inf,
  volume    = {IT-24},
  pages     = {76-80},
  year      = 1978
}

@Article{     wolf:87,
  author    = {E. Zehavi and J.K. Wolf},
  title     = {On the performance evaluation of trellis codes},
  journal   = inf,
  volume    = {IT--33},
  pages     = {196-202},
  month     = mar,
  year      = {1987}
}

@Article{     wolf:93,
  author    = {S.A.~Raghavan and J.K.~Wolf and L.B.~Milstein},
  title     = {{O}n the {P}erformance {E}valuation of {ISI} {C}hannels},
  journal   = inf,
  volume    = {IT-39},
  pages     = {957-965},
  month     = may,
  year      = 1993
}

@Article{     wolfo:67,
  author    = {J. Wolfowitz},
  title     = {Memory Increases Capacity},
  journal   = {Inform. Control},
  volume    = {11},
  pages     = {423-428},
  year      = 1967
}

@Book{        wozencraft:65,
  author    = {J.M. Wozencraft and I.M. Jacobs},
  title     = {Principles of Communication Engineering},
  publisher = wil,
  address   = {New York},
  year      = 1965
}

@InProceedings{   xu:94,
  author    = {G.~Xu and L.~Tong and H.~Liu},
  title     = {{A} {N}ew {A}lgorithm for {F}ast {B}lind {E}qualization of
          {W}ireless {C}ommunication {C}hannels},
  booktitle = {Proceedings of the International Conference on
          Communications {(ICC'94)}},
  pages     = {544-548},
  address   = {New Orleans},
  month     = may,
  year      = 1994
}

@InProceedings{   yao:74,
  author    = {E.~Shamash and K.~Yao},
  title     = {{O}n the {S}tructure and {P}erformance of a {L}inear
          {D}ecision {F}eedback {E}qualizer {B}ased on the {M}inimum
          {E}rror {P}robability {C}riterion},
  booktitle = {Proceedings of the International Conference on
          Communications {(ICC'74)}},
  pages     = {25F-1-25F-5},
  year      = 1974
}

@Article{     yasuda:84,
  author    = {Y. Yasuda and K. Kashiki and Y. Hirata},
  title     = {High rate punctured convolutional codes for soft decision
          Viterbi decoding},
  journal   = com,
  volume    = {COM-32},
  pages     = {315-319},
  month     = mar,
  year      = 1984
}

@InProceedings{   YMC04,
  author    = {Z.~Ye and A.S.~Madhukumar and F.~Chin},
  title     = {{Power Spectral Density and In-Band Interference Power of UWB Signals at Narrowband Systems}},
  booktitle = {Proceedings of the International Conference on
          Communications {(ICC)}},
  pages     = {3561-3565},
  address   = {Paris},
  month     = jun,
  year      = 2004
}

@Article{     Yu95,
  author    = {X.~Yu and S.~Pasupathy},
  title     = {{I}nnovations--{B}ased {MLSE} for {R}ayleigh {F}ading {C}hannels},
  journal   = com,
  volume    = {COM-43},
  pages     = {1534-1544},
  month     = {Feb-Apr},
  year      = 1995
}

@Book{        zeh:92,
  author    = {T. Zeh},
  title     = {{V}ergleich von digitalen {B}asisband- und
          {B}andpa\ss\"ubertragungsverfahren bei {K}an\"alen mit
          {T}iefpa\ss verhalten},
  publisher = {Diplomarbeit, Lehrstuhl f\"ur Nachrichtentechnik der
          Universit\"at Erlangen-N\"urnberg},
  month     = oct,
  year      = 1992
}

@Book{        zell:93,
  author    = {A. Zell},
  title     = {{A}daptive {E}ntzerrverfahren f\"ur digitale
          {K}abel\"ubertragung mit
          {T}omlinson--{H}arashima--{V}orcodierung},
  publisher = {Diplomarbeit, Lehrstuhl f\"ur Nachrichtentechnik der
          Universit\"at Erlangen-N\"urnberg},
  month     = nov,
  year      = 1993
}

@Article{     zheng:93,
  author    = {F.-C.~Zheng and S.~McLaughlin and B.~Mulgrew},
  title     = {{B}lind {E}qualization of {N}onminimum {P}hase {C}hannels:
          {H}igher {O}rder {C}umulant {B}ased {A}lgorithm},
  journal   = sip,
  volume    = {41},
  pages     = {681-691},
  month     = feb,
  year      = 1993
}

@InProceedings{   ZG01,
  author    = {S.~Zhou and G.B.~Giannakis},
  title = {{Space--Time Coded Transmissions with Maximum Diversity Gains over Frequency--Selective Multipath Fading Channels}},
  booktitle = {Proceedings of the IEEE Global Telecommunications Conference (GLOBECOM)},
  pages = {440-444},
  address   = {San Antonio},
  month = nov,
  year  = 2001
}

@Article{     ZG03,
  author    = {S.~Zhou and G.B.~Giannakis},
  title     = {{Single--Carrier Space--Time Block--Coded Transmission Over Frequency--Selective Fading Channels}},
  journal   = inf,
  volume    = {49},
  pages     = {164-179},
  month     = jan,
  year      = 2003
}

@Book{        ziemer:85,
  author    = {R. Ziemer and R.L. Peterson},
  title     = {Digital Communications and Spread Spektrum Systems},
  publisher = {McMillon},
  address   = {New York},
  year      = 1985
}

@Article{     zig:66,
  author    = {Zigangirov, K.S.},
  title     = {Some sequential decoding procedures},
  journal   = {Problemy Predachi Informacii},
  volume    = {2},
  pages     = {13-25},
  year      = 1966
}

@InProceedings{   zuerbes:94,
  author    = {S.~Z\"urbes and W.~Papen and W.~Schmidt},
  title     = {{A} {N}ew {A}rchitecture for {M}obile {R}adio with
          {M}acroscopic {D}iversity and {O}verlapping {C}ells},
  booktitle = {Proceedings of PIMRC'94},
  address   = {The Hague, The Netherlands},
  month     = sep,
  year      = 1994
}

@Book{        zurmuehl:84,
  author    = {R. {Zurm\"uhl, S. Falk}},
  title     = {{M}atrizen},
  publisher = {Springer Verlag},
  address   = {Berlin},
  year      = {1984}
}


@Book{ lucky,
    author ={R.~W.~Lucky and J.~Salz~Jr. and E.~J.~Weldon},
    title ={{Principles of Data Communication}},
    publisher = {McGraw-Hill},
    address ={New York},
    year ={1968}
}

@Article{     QB04,
  author    = {M.~Qin and R.~S.~Blum},
  title     = {{Properties of Space-Time Codes for Frequency--Selective Channels}},
  journal   = sip,
  volume    = {52},
  pages     = {694-702},
  month     = mar,
  year      = 2004
}

@Article {crozier,
    author = {S. N. Crozier and D. D. Falconer and S. A. Mahmoud},
  title = {{Least Sum of Squared Errors ({LSSE}) Channel Estimation}},
  journal = {IEE Proceedings-F},
  pages = {371-378, issue: 4},
  month = {August},
  volume = {138},
  year = {1991},
}

@Article {mazur,
    author = {A. Furuskar and S. Mazur and F. Muller and H. Olofsson},
    title = {EDGE: Enhanced data rates for {GSM} and {TDMA/136} evolution},
    journal = {IEEE Personal Communications Magazine},
    volume = {6},
    pages = {56-66},
    month = {June},
    year = {1999}
}

@Article{     802.15,
  author    = {{IEEE P802.15}},
  title     = {{Multiband OFDM Physical Layer Proposal for IEEE 802.15 Task Group 3a (Doc.~Number P802.15-03/268r3}},
  month     = mar,
  year      = 2004
}

@Article{     MBOA04,
  author    = {{MultiBand OFDM Alliance SIG}},
  title     = {{In-band Interference Properties of MB--OFDM}},
  journal       = {[Online] http://www.multi\-band\-ofdm.org/papers/MBOA-SIG-2004-in-band-interference-properties-mb-ofdm.ppt},

  month     = sep,
  year      = 2004
}

@Article{     wlan04,
  author    = {{IEEE P802.15}},
  title     = {{Coexistence of Multi-band OFDM and IEEE 802.11a: Interference Measurements (Doc.~Number P802.15-04/017r0}},
  month     = jan,
  year      = 2004
}

@Article{     dtv05_1,
  author    = {{IEEE P802.15}},
  title     = {{Impact of MB--OFDM and DS--UWB Interference -- Part 2 (Doc.~Number P802.15-05/0039r0}},
  month     = jan,
  year      = 2005
}

@Article{     dtv05_2,
  author    = {{National Telecommunications and Information Administration (NTIA)}},
  title     = {{Interference Potential of Ultrawideband Signals (NTIA Report TR-05-419)}},
  journal       = {[Online] http://www.its.bldr\-doc.gov/pub/ntia-rpt/05-419/05-419.pdf},
  month     = feb,
  year      = 2005
}

@InProceedings{   Yiu,
  author    = {S.~Yiu and R.~Schober and W.~Gerstacker},
  title     = {{Optimization of Delay Diversity for Decision-Feedback Equalization}},
  booktitle = {Proceedings of IEEE Symposium on Personal, Indoor and Mobile Radio Communications},
  pages         = {68-72},
  address   = {Barcelona, Spain},
  month     = sep,
  year      = 2004
}

@Article{     Dighe,
  author    = {P.~Dighe and R.~Mallik and S.~Jamuar},
  title     = {{Analysis of Transmit-Receive Diversity in Rayleigh Fading}},
  journal   = com,
  volume    = {51},
  pages     = {694-703},
  month     = apr,
  year      = 2003
}

@Article{     Love,
  author    = {D.~Love and R.~Heath and T.~Strohmer},
  title     = {{Grassmannian Beamforming for Multiple-Input Multiple-Output Wirelss Systems}},
  journal   = inf,
  volume    = {49},
  pages     = {2735-2747},
  month     = oct,
  year      = 2003
}

@Article{     Mukkavilli,
  author    = {K.~Mukkavilli and A.~Sabharwal and E.~Erkip and B.~Aazhang},
  title     = {{Beamforming with Finite Rate Feedback in Multiple Antenna Systems}},
  journal   = inf,
  volume    = {49},
  pages     = {2562-2579},
  month     = oct,
  year      = 2003
}

@Article{     Choi,
  author    = {J.~Choi and R.~Heath},
  title     = {{Interpolation Based Transmit Beamforming for MIMO-OFDM with Limited Feedback}},
  journal   = sip,
  volume    = {53},
  pages     = {4125-4135},
  month     = nov,
  year      = 2005
}

@Article{     Xia,
  author    = {P.~Xia and S.~Zhou and G.~Giannakis},
  title     = {{Adaptive MIMO-OFDM Based on Partial Channel State Information}},
  journal   = sip,
  volume    = {52},
  pages     = {202-213},
  month     = jan,
  year      = 2004
}

@InProceedings{   Xia-2,
  author    = {P.~Xia and G.~Giannakis},
  title = {{Design and Analysis of Transmit-Beamforming based on Limited-Rate Feedback}},
  booktitle = {Proceedings of the IEEE Vehicular Technology Conference},
  address   = {},
  month = sep,
  year  = 2004
}

@Article{     Cioffi,
  author    = {J.~Cioffi and G.~Dudevoir and M.~Eyuboglu and {G.~Forney Jr.}},
  title     = {{MMSE Decision-Feedback Equalizers and Coding - Part I: Equalization Results}},
  journal   = com,
  volume    = {43},
  pages     = {2582-2594},
  month     = oct,
  year      = 1995
}

@Article{     Cameron,
  author    = {R.~Cameron},
  title     = {{Minimizing the Product of Two Raleigh Quotients}},
  journal   = {Linear and Multilinear Algebra},
  volume    = {13},
  pages     = {177-178},
  month     = {},
  year      = 1983
}

@Article{     Martin,
  author    = {R.~Martin and K.~Vanbleu and M.~Ding and G.~Ysebaert and M.~Milosevic and B.~Evans and M.~Moonen and R.~Johnson},
  title     = {{Unification and Evaluation of Equalization Structures and Design Algorithms for Discrete Multitone Modulation Systems}},
  journal   = sip,
  volume    = {53},
  pages     = {3880-3894},
  month     = oct,
  year      = 2005
}

@Book{        Weinstock,
  author    = {R.~Weinstock},
  title     = {{Calculus of Variations, with Applications to Physics and Engineering}},
  publisher = {Dover},
  address   = {New York},
  year      = 1974
}

@Article{     Gersho,
  author    = {A.~Gersho},
  title     = {{Asymptotically Optimal Block Quantization}},
  journal   = inf,
  volume    = {25},
  pages     = {373-380},
  month     = jul,
  year      = 1979
}

@Article{     LBG80,
  author    = {Y.~Linde and A.~Buzo and R.~Gray},
  title     = {{An Algorithm for Vector Quantizer Design}},
  journal   = com,
  volume    = {28},
  pages     = {84-95},
  month     = jan,
  year      = 1980
}

@Article{     Likas,
  author    = {A.~Likas and N.~Vlassis and J.~Verbeek},
  title     = {{The Global K-means Clustering Algorithm}},
  journal   = {Pattern Recognition},
  volume    = {36},
  pages     = {451-561},
  month     = {},
  year      = 2003
}

@Article{     XW05,
  author    = {R.~Xu and D.~{Wunsch II}},
  title     = {{Survey of Clustering Algorithms}},
  journal   = {IEEE Trans.~Neural Networks},
  volume    = {16},
  pages     = {645-678},
  month     = may,
  year      = 2005
}

@Article{     SH05,
  author    = {F.~Shen and O.~Hasegawa},
  title     = {{An Adaptive Incremental LBG for Vector Quantization}},
  journal   = {To appear in Neural Networks},
  volume    = {},
  pages     = {},
  month     = {},
  year      = 2006
}

@Article{     PR01,
  author    = {G.~Patan\`{e} and M.~Russo},
  title     = {{The Enhanced LBG Algorithm}},
  journal   = {Neural Networks},
  volume    = {14},
  pages     = {1219-1237},
  month     = sep,
  year      = 2001
}

@Article{     YSG06,
  author    = {Y.~Liang and R.~Schober and W.~Gerstacker},
  title     = {{Transmit Beamforming with Perfect CSI for Frequency-Selective Channels}},
  journal   = {Submitted to the IEEE Vehicular Technology Conference},
  volume    = {},
  pages     = {},
  month     = mar,
  year      = 2006
}

@Manual{ieee11n,
  author    = {{V. Erceg et al.}},
  title     = {{IEEE} 802.11-0/940r4, {TG}n {I}ndoor {MIMO} {WLAN} {C}hannel {M}odels},
  month     = may,
  year      = 2004
}

@Article{     BOLCSKEI03,
  author    = {H.~B\"olcskei and M.~Borgmann and A.~J. Paulraj},
  title     = {Impact of the propagation environment on the performance of space-frequency coded {MIMO-OFDM}},
  journal   = sel,
  volume    = 21,
  pages     = {427-439},
  month     = apr,
  year      = 2003
}

@Manual{wimax,
  author    = {IEEE Std 802.16e-2005},
  title     = {IEEE Standard for Local and Metropolitan Area Networks -- Part 16},
  year      = 2006
}

@Article{zhou06,
  author    = {S.~Zhou and B.~Li and P.~Willett},
  title     = {{Recursive and Trellis-Based Feedback Reduction for {MIMO-OFDM} with Rate-Limited Feedback}},
  journal   = {IEEE Trans. Wireless Commun.},
  volume    = 5,
  pages     = {3400-3405},
  month     = dec,
  year      = 2006
}

@Article{ zhou02adaptive,
  author    = {S. Zhou and G. Giannakis},
  title     = {{Adaptive Modulation for Multiantenna Transmissions with Channel Mean Feedback}},
  journal   = {IEEE Trans. Wireless Commun.},
  volume    = 3,
  pages     = {1626-1636},
  month     = sep,
  year      = 2004
}

@article{ chung01degrees,
  author    = {S. Chung and A. Goldsmith},
  title     = {{Degrees of Freedom in Adaptive Modulation: A Unified View}},
  journal   = {IEEE Trans. Commun.},
  volume    = 49,
  number    = 9,
  pages     = {1561-1571},
  month     = sep,
  year      = 2001
}

@ARTICLE{Shemesh,
  AUTHOR =       {D. Shemesh},
  TITLE =        {Common eigenvectors of two matrices},
  JOURNAL =      {Linear Algebra and its Applications},
  YEAR =         {1984},
  volume =       {62}
}


@Article{LiangGCM,
  author    = {Y.~Liang and R.~Schober and W.~Gerstacker},
  title     = {{Transmit Beamforming for Frequency--Selective Channels with Decision-Feedback Equalization}},
  journal   = {IEEE Trans. Wireless Commun.},
  volume    = 6,
  pages     = {4401-4411},
  month     = dec,
  year      = 2007
}

@article{LiangGCM2,
  author    = {Y.~Liang and R.~Schober and W.~Gerstacker},
  title     = {{Time--Domain Transmit Beamforming for MIMO--OFDM Systems}},
  journal   = {To be presented at the IEEE Global Telecommun. Conf.},
  month     = nov,
  year      = 2007
}

@InProceedings{ASA05,
  author    = {E.~Akay and E.~Sengul and E.~Ayanoglu},
  title     = {{Performance Analysis of Beamforming for MIMO OFDM with BICM}},
  booktitle = {Proceedings of the IEEE Intern. Conf. Commun.},
  address   = {},
  month     = jun,
  year      = 2005
}

@BOOK{NW06,
  AUTHOR =       {J.~Nocedal and S.~Wright},
  TITLE =        {Numerical Optimization},
  PUBLISHER =    {Springer},
  address   = {New York},
  YEAR =         {2006},
}

@BOOK{Gol05,
  AUTHOR =       {A.~Goldsmith},
  TITLE =        {Wireless Communications},
  PUBLISHER =    {Cambridge University Press},
  YEAR =         {2005},
}

@Article{   Sidiropoulos,
  author    = {N.~Sidiropoulos and T.~Davidson and Z.~Luo},
  title     = {{Transmit Beamforming for Physical--Layer Multicasting}},
  journal   = sip,
  volume    = 54,
  pages     = {2239-2251},
  month     = jun,
  year      = 2006
}

@Article{   Love2,
  author    = {D.~J.~Love and R.~W.~Heath Jr. and W.~Santipach and M.~L.~Honig},
  title     = {{What is the Value of Limited Feedback for MIMO Channels?}},
  journal   = cma,
  volume    = 42,
  number    = 10,
  pages     = {54-59},
  month     = Oct,
  year      = 2004
}

@Manual{      IEEE802.16,
title = {{IEEE802.16-2004, IEEE Standard for Local and Metropolitan Area Networks-Part16: Air Interface for Fixed Broadband Wireless Access System, October, 2004.}}
}

@Manual{   IEEE802.11n,
title = {{IEEE 802.11 working group, IEEEP802.11n/D0.02, Feb 2006.}}
}

@ARTICLE{LiShaoHua,
  AUTHOR =       {S.~Li and D.~Huang and K.~Letaief and Z.~Zhou},
  TITLE =        {{Multi-Stage Beamforming for Coded OFDM with Multiple Transmit and Multiple Receive Antennas}},
  JOURNAL =      wc,
  YEAR =         2007,
  volume =       6,
  number =       3,
  pages =        {959-969},
  month =        mar,
}

@article{Foschini98,
 author = {G. J. Foschini and M. J. Gans},
 title = {{On Limits of Wireless Communications in a Fading Environment when Using Multiple Antennas}},
 journal = {Wirel. Pers. Commun.},
 volume = {6},
 number = {3},
 year = {1998},
 issn = {0929-6212},
 pages = {311--335},
 doi = {http://dx.doi.org/10.1023/A:1008889222784},
 publisher = {Kluwer Academic Publishers},
 address = {Hingham, MA, USA},
 }

@ARTICLE{Bhashyam02,
  AUTHOR =       {S.~Bhashyam and A.~Sabharwal and B.~Aazhang},
  TITLE =        {{Feedback Gain in Multiple Antenna Systems}},
  JOURNAL =      com,
  YEAR =         2002,
  volume =       50,
  number =       5,
  pages =        {785--798},
  month =        may,
}

@ARTICLE{JSO04,
  AUTHOR =       {G.~Jongren and M.~Skoglund},
  TITLE =        {{Quantized Feedback Information in Orthogonal Space-Time Block Coding}},
  JOURNAL =      {inf},
  YEAR =         {2004},
  volume =       {50},
  number =       {10},
  pages =        {2473--2486},
  month =        oct,
}

@ARTICLE{Zheng07,
  AUTHOR =       {J.~Zheng and E.~Duni and B.~Rao},
  TITLE =        {{Analysis of Multiple-Antenna Systems With Finite--Rate Feedback Using High--Resolution Quantization Theory}},
  JOURNAL =      sip,
  YEAR =         {2007},
  volume =       {55},
  pages =        {1461--1476},
  month =        apr,
}

@ARTICLE{Pande06,
  AUTHOR =       {T.~Pande and D.~Love and J.~Krogmeier},
  TITLE =        {{A Weighted Least Squares Approach to Precoding With Pilots for MIMO--OFDM}},
  JOURNAL =      sip,
  YEAR =         2006,
  volume =       54,
  pages =        {4067--4073},
  month =        oct,
}

@ARTICLE{Pande07,
  AUTHOR =       {T.~Pande and D.~Love and J.~Krogmeier},
  TITLE =        {{Reduced Feedback MIMO--OFDM Precoding and Antenna Selection}},
  JOURNAL =      sip,
  YEAR =         2007,
  volume =       55,
  pages =        {2284--2293},
  month =        may,
}


@InProceedings{ DK01,
  author    = {A. Dammann and S. Kaiser},
  title     = {{Standard Conformable Antenna Diversity Techniques for OFDM Systems and Its Application to The DVB-T System}},
  booktitle = {Proceedings of the IEEE Global Telecommun. Conf.},
  address   = {},
  month     = dec,
  year      = 2001
}

@Article{     BM06,
  author    = {G. Bauch and J. Malik},
  title     = {{Cyclic Delay Diversity with Bit-Interleaved Coded Modulation in Orthogonal Frequency Division Multiple Access}},
  journal   = wc,
  volume    = {5},
  pages     = {2092-2100},
  month     = aug,
  year      = 2006
}

@ARTICLE{ PCL03,
  AUTHOR =       {D.~Palomar and J.~Cioffi and M.~Lagunas},
  TITLE =        {{Joint Tx-Rx Beamforming Design for Multicarrier MIMO Channels: A Unified Framework for Convex Optimization}},
  JOURNAL =      sip,
  YEAR =         2003,
  volume =       51,
  pages =        {2381--2401},
  month =        sep,
}

@ARTICLE{ ASA07,
  AUTHOR =       {E.~Akay and E.~Sengul and E.~Ayanoglu},
  TITLE =        {{Bit Interleaved Coded Multiple Beamforming}},
  JOURNAL =      com,
  YEAR =         2007,
  volume =       55,
  pages =        {1802--1811},
  month =        sep,
}

@ARTICLE{ JF07,
  AUTHOR =       {S.~Johnson and M.~Frigo},
  TITLE =        {{A Modified Split--Radix FFT With Fewer Arithmetic Operations}},
  JOURNAL =      sip,
  YEAR =         2007,
  volume =       55,
  pages =        {111-119},
  month =        jan,
}

@UNPUBLISHED{Love04,
  AUTHOR =       {D.~Love},
  TITLE =        {{Tables of Complex Grassmannian Packings. [Online]}},
  NOTE =         {Available: http://www.ece.purdue.edu/~djlove/grass.html},
}

@INPROCEEDINGS{LiangICC08,
  AUTHOR =       {Y.~Liang and R.~Schober and W.~Gerstacker},
  TITLE =        {{Minimum BER Transmit Beamforming for MIMO--OFDM Systems with Finite Rate Feedback}},
  BOOKTITLE =    {Proceedings of the IEEE International Conference on Communications},
  YEAR =         {2008},
  month =        may,
}

@INPROCEEDINGS{LiangGCM07,
  AUTHOR =       {Y.~Liang and R.~Schober and W.~Gerstacker},
  TITLE =        {{Time--Domain Transmit Beamforming for MIMO-OFDM Systems}},
  BOOKTITLE =    {Proceedings of the IEEE Global Telecommunication Conference},
  YEAR =         {2007},
  month =        dec,
}

@Article{   love08,
  author    = {D.~Love and R.~Heath and V.~Lau and D.~Gesbert and B.~Rao and M.~Andrews},
  title     = {{An Overview of Limited Feedback in Wireless Communications Systems (Tutorial Paper)}},
  journal   = sel,
  year      = {to appear 2008}
}

@Article{   Jing08,
  author    = {Y.~Jing and H.~Jafarkhani},
  title     = {{Network Beamforming Using Relays With Perfect Channel Information}},
  journal   = inf,
  volume    = 55,
  number    = 6,
  pages     = {2499-2517},
  month     = jun,
  year      = 2009
}

@ARTICLE{Hammerstrom07,
  AUTHOR =       {I.~Hammerstrom and A.~Wittneben},
  TITLE =        {{Power Allocation Schemes for Amplify--and--Forward MIMO--OFDM Relay Links}},
  JOURNAL =      {IEEE Trans. Wireless Commun.},
  YEAR =         2007,
  volume =       6,
  number =       8,
  pages =        {2798-2802},
  month =        aug,
}

@ARTICLE{Munoz07,
  AUTHOR =       {O.~Munoz-Medina and J.~Vidal and A.~Agustin},
  TITLE =        {{Linear Transceiver Design in Nonregenerative Relays With Channel State Information}},
  JOURNAL =      sip,
  YEAR =         2007,
  volume =       55,
  number =       6,
  pages =        {2593-2604},
  month =        jun,
}


@ARTICLE{Ng07,
  AUTHOR =       {T.~Ng and W.~Yu},
  TITLE =        {{Joint Optimization of Relay Strategies and Resource Allocations in Cooperative Cellular Networks}},
  JOURNAL =      sel,
  YEAR =         2007,
  volume =       25,
  number =       2,
  pages =        {328-339},
  month =        feb,
}


@ARTICLE{ma08,
  AUTHOR =       {Y.~Ma and N.~Yi and R.~Tafazolli},
  TITLE =        {{Bit and Power Loading for OFDM-Based Three-Node Relaying Communications}},
  JOURNAL =      sip,
  YEAR =         2008,
  volume =       56,
  number =       7,
  pages =        {3236-3247},
  month =        jul,
}


@BOOK{nocedal06,
  AUTHOR =       {J.~Nocedal and S.~J.~Wright},
  TITLE =        {Numerical Optimization},
  PUBLISHER =    {Springer},
  YEAR =         {2006},
}

@Article{   yu06,
  author    = {W.~Yu and R.~Lui},
  title     = {{Dual Methods for Nonconvex Spectrum Optimization of Multicarrier Systems}},
  journal   = com,
  volume    = 54,
  number    = 7,
  pages     = {1310-1322},
  month     = july,
  year      = 2006
}

@Article{   love08,
  author    = {D.~Love and R.~Heath and V.~Lau and D.~Gesbert and B.~Rao and M.~Andrews},
  title     = {{An Overview of Limited Feedback in Wireless Communications Systems (Tutorial Paper)}},
  journal   = sel,
  year      = {to appear 2008}
}

@Article{   Nabar04,
  author    = {R.~U.~Nabar and H.~B\"{o}lcskei and F.~W.~Kneub\"{u}hler},
  title     = {{Fading Relay Channels: Performance Limits and Space--Time Signal Design}},
  journal   = sel,
  volume    = 22,
  pages     = {1099-1109},
  month     = aug,
  year      = 2004
}

@BOOK{Wilkinson65,
  AUTHOR =       {J.~H.~Wilkinson},
  TITLE =        {{The Algebraic Eigenvalue Problem}},
  PUBLISHER =    {Clarendon Press},
  YEAR =         {1965},
}



@ARTICLE{Peters09,
  AUTHOR =       {S.~W.~Peters and  R.~W.~Heath~Jr.},
  TITLE =        {{The Future of WiMAX: Multihop Relaying with IEEE 802.16j}},
  JOURNAL =      {IEEE Communications Magazine},
  YEAR =         2009,
  volume =       47,
  number =       1,
  pages =        {104-111},
  month =        Jan,
}

@ARTICLE{Zhao08,
  AUTHOR =       {Y.~Zhao and R.~Adve and T.~J.~Lim},
  TITLE =        {{Beamforming with Limited Feedback in Amplify--and--Forward Cooperative Networks}},
  JOURNAL =      wc,
  YEAR =         2008,
  volume =       7,
  number =       12,
  pages =        {5145-5149},
  month =        Dec,
}

@ARTICLE{Fan07,
  AUTHOR =       {Y.~Fan and J.~Thompson},
  TITLE =        {{MIMO Configurations for Relay Channels: Theory and Practice}},
  JOURNAL =      wc,
  YEAR =         2007,
  volume =       6,
  number =       5,
  pages =        {1774-1786},
}


%%%%

@ARTICLE{WangBo2005,
  AUTHOR =       {B.~Wang and J.~Zhang and A.~Host-Madsen},
  TITLE =        {{On the Capacity of MIMO Relay Channels}},
  JOURNAL =      inf,
  YEAR =         2005,
  volume =       51,
  number =       1,
  pages =        {29-43},
  month =        jan,
}

@ARTICLE{Shi2007,
  AUTHOR =       {H.~Shi and T.~Abe and T.~Asai and H.~Yoshino},
  TITLE =        {{Relaying Schemes Using Matrix Triangularization for MIMO Wireless Networks}},
  JOURNAL =      com,
  YEAR =         2007,
  volume =       55,
  number =       9,
  pages =        {1683-1688},
  month =        sep,
}


@ARTICLE{Chae2008,
  AUTHOR =       {C.~Chae and T.~Tang and R.~W.~Heath and S.~Cho},
  TITLE =        {{MIMO Relaying With Linear Processing for Multiuser Transmission in Fixed Relay Networks}},
  JOURNAL =      sip,
  YEAR =         2008,
  volume =       56,
  number =       2,
  pages =        {727-738},
  month =        feb,
}


@ARTICLE{Kang2007,
  AUTHOR =       {T.~Kang and V.~Rodoplu},
  TITLE =        {{Algorithms for the MIMO Single Relay Channel}},
  JOURNAL =      wc,
  YEAR =         2007,
  volume =       6,
  number =       5,
  pages =        {1596-1600},
  month =        may,
}


@ARTICLE{Peters2008,
  AUTHOR =       {S.~Peters and R.~W.~Heath},
  TITLE =        {{Nonregenerative MIMO Relaying With Optimal Transmit Antenna Selection}},
  JOURNAL =      siplett,
  YEAR =         2008,
  volume =       15,
  pages =        {421-424},
}

@ARTICLE{Tang2007,
  AUTHOR =       {X.~Tang and Y.~Hua},
  TITLE =        {{Optimal Design of Non-Regenerative MIMO Wireless Relays}},
  JOURNAL =      wc,
  YEAR =         2007,
  volume =       6,
  number =       4,
  pages =        {1398-1407},
  month =        apr,
}

@ARTICLE{CA09,
  AUTHOR =       {D.~Costa and S.~Aissa},
  TITLE =        {{Cooperative Dual-Hop Relaying Systems with Beamforming over Nakagami-m Fading Channels}},
  JOURNAL =      wc,
  YEAR =         2009,
  volume =       8,
  pages =        {3950-3954},
  month =        aug,
}

@ARTICLE{LLSV09,
  AUTHOR =       {R. Louie and Y. Li and H. Suraweera and B. Vucetic},
  TITLE =        {{Performance Analysis of Beamforming in Two Hop Amplify and Forward Relay Networks with Antenna Correlation}},
  JOURNAL =      wc,
  YEAR =         2009,
  volume =       8,
  pages =        {3132-3141},
  month =        jun,
}

@ARTICLE{Khoshnevis2008,
  AUTHOR =       {B.~Khoshnevis and W.~Yu and R.~Adve},
  TITLE =        {{Grassmannian Beamforming for MIMO Amplify-and-Forward Relaying}},
  JOURNAL =      sel,
  YEAR =         2008,
  volume =       26,
  number =       8,
  pages =        {1397-1407},
  month =        oct,
}

@ARTICLE{Borade2007,
  AUTHOR =       {S.~Borade and L.~Zheng and R.~Gallager},
  TITLE =        {{Amplify-and-Forward in Wireless Relay Networks: Rate, Diversity, and Network Size}},
  JOURNAL =      inf,
  YEAR =         2007,
  volume =       53,
  number =       10,
  pages =        {3302-3318},
  month =        oct,
}

@ARTICLE{Behbahani2008,
  AUTHOR =       {A.~S.~Behbahani and R.~Merched and A.~M.~Eltawil},
  TITLE =        {{Optimizations of a MIMO Relay Network}},
  JOURNAL =      sip,
  YEAR =         2008,
  volume =       56,
  pages =        {5062-5073},
  month =        oct,
}

@ARTICLE{AP08,
  AUTHOR =       {M.~Abdallah and H.~Papadopoulos},
  TITLE =        {{Beamforming Algorithms for Information Relaying in Wireless Sensor Networks}},
  JOURNAL =      sip,
  YEAR =         2008,
  volume =       56,
  pages =        {4772-4784},
  month =        oct,
}

@ARTICLE{ZWPO09,
  AUTHOR =       {G.~Zheng and K.-K.~Wong and A.~Paulraj and B.~Ottersten},
  TITLE =        {{Robust Collaborative-Relay Beamforming}},
  JOURNAL =      sip,
  YEAR =         2009,
  volume =       57,
  pages =        {3130-3143},
  month =        aug,
}

@ARTICLE{ZWPO09a,
  AUTHOR =       {G.~Zheng and K.-K.~Wong and A.~Paulraj and B.~Ottersten},
  TITLE =        {{Collaborative-Relay Beamforming with Perfect CSI: Optimum and Distributed Implementation}},
  JOURNAL =      siplett,
  YEAR =         2009,
  volume =       16,
  pages =        {257-260},
  month =        apr,
}


@ARTICLE{Zhang2009,
  AUTHOR =       {R.~Zhang and C.~C.~Chai and Y.~C.~Liang},
  TITLE =        {{Joint Beamforming and Power Control for Multiantenna Relay Broadcast Channel With QoS Constraints}},
  JOURNAL =      sip,
  YEAR =         2009,
  volume =       57,
  pages =        {726-737},
  month =        feb,
}

@INPROCEEDINGS{LiangICC09,
  AUTHOR =       {Y.~Liang and R.~Schober},
  TITLE =        {{Cooperative Amplify-and-Forward Beamforming for OFDM Systems with Multiple Relays}},
  BOOKTITLE =    {accepted for presentation at the IEEE International Conference on Communications},
  YEAR =         {2009},
  month =        jun,
}

@INPROCEEDINGS{Gastpar2002,
  AUTHOR =       {M.~Gastpar and M.~Vetterli},
  TITLE =        {{On the Capacity of Wireless Networks: the Relay Case}},
  BOOKTITLE =    {Proceedings of INFOCOM 2002},
  YEAR =         {2002},
  volume =       {3},
  pages =        {1577-1586},
}


@ARTICLE{Brewer1978,
  AUTHOR =       {J.~Brewer},
  TITLE =        {{Kronecker Products and Matrix Calculus in System Theory}},
  JOURNAL =      {IEEE Tran. on Circuits and Systems},
  YEAR =         {1978},
  volume =       {25},
  number =       {9},
  pages =        {772-781},
  month =        sep,
}

@Article{Larsson03,
  AUTHOR =       {P.~Larsson},
  TITLE =        {{Large--Scale Cooperative Relaying Network with Optimal Coherent Combining Under Aggregate Relay Power Constraint}},
  Journal =      {Future Telecommunications Conf.},
  YEAR =         {2003},
  month =        dec,
}

@Article{TK08,
  AUTHOR =       {A.~Talebi and W. Krzymien},
  TITLE =        {{Multiple-Antenna Multiple-Relay Cooperative Communication System with Beamforming}},
  Journal =      {IEEE Veh. Techn. Conf. (VTC)},
  YEAR =         {2008},
  month =        may,
}


@ARTICLE{Henrion02,
    author = {D.~Henrion and J.~B.~Lasserre},
    title = {{GloptiPoly: Global Optimization over Polynomials with Matlab and SeDuMi}},
    journal = {ACM Trans. Math. Soft},
    year = {2002},
    volume = {29},
    pages = {165--194}
}

@ARTICLE{Parrilo02,
  AUTHOR =       {S.~Prajna and A.~Papachristodoulou and P.~A.~Parrilo},
  TITLE =        {{SOSTOOLS: Sum of Squares Optimization Toolbox for Matlab}},
  JOURNAL =      {available from http://www.cds.caltech.edu/sostools},
  YEAR =         {2002--04},
}

@BOOK{Boyd_CO,
  AUTHOR =       {S.~Boyd and L.~Vandenberghe},
  TITLE =        {Convex Optimization},
  PUBLISHER =    {Cambridge University Press},
  YEAR =         {2004},
}

@BOOK{Ber08,
  AUTHOR =       {D.~Bertsekas},
  TITLE =        {Nonlinear Programming},
  PUBLISHER =    {Athena Scientific},
  YEAR =         {2008},
}

@ARTICLE{chen09,
  author    = {H.~Chen and A.~Gershman and S.~Shahbazpanahi},
  title     = {{Filter--And--Forward Distributed Beamforming in Relay Networks with Frequency Selective Fading}},
  JOURNAL =      sip,
  YEAR =         2010,
  volume =       58,
  pages =        {1251-1262},
  month =        mar
}

@ARTICLE{Mheidat07,
  AUTHOR =       {H.~Mheidat and M.~Uysal and N.~Al-Dhahir},
  TITLE =        {{Equalization Techniques for Distributed Space--Time Block Codes With Amplify--and--Forward Relaying}},
  JOURNAL =      sip,
  YEAR =         2007,
  volume =       55,
  number =       5,
  pages =        {1839-1852},
  month =        may
}

@ARTICLE{LiangTWC07,
title={Transmit beamforming for frequency-selective channels with decision-feedback equalization},
author={Y.~Liang and R.~Schober and W.~Gerstacker},
journal=wc,
year={2007},
month={December},
volume={6},
number={12},
pages={4401-4411},
}

@UNPUBLISHED{LiangTWC10,
  AUTHOR =       {Y.~Liang and A.~Ikhlef and W.~Gerstacker and R.~Schober},
  TITLE =        {{Cooperative Filter--and--Forward Beamforming for Frequency--Selective Channels with Equalization}},
  month={February},
  year={2010},
  NOTE =         {Submitted to IEEE Trans. Wireless Commun., Available: http://www.ece.ubc.ca/$\sim$yangl/mimo\_cap/TWC-10.pdf},
}

@ARTICLE{Aissa11,
title={{Buffers Improve the Performance of Relay Selection}},
author={A. Ikhlef and D. Michalopoulos and R. Schober},
journal={Accepted for presentation at IEEE Global Telecommun. Conf. (Globecom). [Online] http://ece.ubc.ca/$\sim$dio/Globecom11.pdf},
year={2011},
}

@ARTICLE{meulen,
title={{Three-Terminal Communication Channels}},
author={E. C.  Van Der Meulen},
journal={Advances in Applied Probability},
year={1971},
volume={3},
pages={120-154},
}


@ARTICLE{nostrina,
author={A. Nosratinia and T.E. Hunter and A. Hedayat},
journal=cma,
title={{Cooperative Communication in Wireless Networks}},
year=2004,
month=oct,
volume={42},
pages={ 74 - 80},
keywords={ cooperative communication; multiple-antenna transmitter; multiuser environment; single-antenna mobiles; transmit diversity; wireless networks; MIMO systems; antenna arrays; diversity reception; mobile radio; radio transmitters; transmitting antennas;},
doi={10.1109/MCOM.2004.1341264},
ISSN={0163-6804},}


@ARTICLE{6130553,
author={A. Ikhlef and D. S. Michalopoulos and R. Schober},
journal={IEEE Transactions on Wireless Communications},
title={Max-Max Relay Selection for Relays with Buffers},
year={2012},
volume={11},
number={3},
pages={1124-1135},
keywords={Rayleigh channels;decode and forward communication;diversity reception;error statistics;HRS;MMRS;Rayleigh fading;SNR gain;buffer state;channel state;decode-and-forward protocol;diversity gain;half-duplex relay;hybrid relay selection;max-max relay selection;relay-destination channel;signal-to-noise ratio;source-relay channel;symbol error probability;Buffer storage;Fading;Gain;Markov processes;Protocols;Relays;Signal to noise ratio;Cooperative relaying;error rate analysis;outage analysis;relay selection;relays with buffers},
doi={10.1109/TWC.2012.011012.110682},
ISSN={1536-1276},
month={March},}

@ARTICLE{XFTP08,
title={{Buffering in a Three-Node Relay Network}},
author={B. Xia and Y. Fan and J. Thompson and H. V. Poor},
journal=wc,
year=2008,
month=nov,
volume={7},
pages={4492-4496},
}


@ARTICLE{Bletsas06,
title={{A Simple Cooperative Diversity Method Based on Network Path selection}},
author={A. Bletsas and A. Khisti and D. Reed and A. Lippman},
journal=sel,
year=2006,
month=mar,
volume={24},
pages={659-672},
}

@BOOK{gallager,
  author    = {R. Gallager},
  title     = {{Information Theory and Reliable Communication}},
  publisher = { New York: Wiley},
  year      = 1968
}

@ARTICLE{little,
title={{A Proof of the Queueing Formula: $L = \lambda w$}},
author={J. D. C. Little},
journal={Operations Research},
year={1961},
month={May - Jun.},
volume={9},
number={3},
pages={383-388},
}


@BOOK{2,
  author    = {Leonidas Georgiadis and Michael J.
Neely and Leandros Tassiulas},
  title     = {{Resource Allocation and Cross Layer Control in Wireless Networks}},
  publisher = {Now Publishers Inc},
  year      = 2006
}

@BOOK{neely-2,
  author    = {M. J. Neely},
  title     = {{Stochastic Network Optimization with Application to
Communication and Queueing Systems}},
  publisher = {Morgan \& Claypool},
  year      = 2010
}

@BOOK{gross-harris,
  author    = {D. Gross and J. F. Shortle  and J. M. Thompson  and C. M. Harris},
  title     = {{Fundamentals of Queueing Theory}},
  edition   = {4th},
  publisher = {John Wiley \& Sons, Inc},
  year      = 2008
}


@BOOK{newton,
  author    = {C. Kelley},
  title     = {{Solving Nonlinear Equations With Newton's Method}},
  publisher = {{Society Ind. Appl. Math.}},
  year      =  2003
}



@ARTICLE{kingman,
title={{Some Inequalities for the Queue GI/G/1}},
author={J.F.C. Kingman},
journal={Biometrika},
year={1962},
volume={49},
pages={315-324},
}

@ARTICLE{daley,
title={{Inequalities for Moments of Tails of Random Variables With a Queueing
Application}},
author={J. Daley},
journal={Zeitschrift fur Wahrscheinlichkeitstheorie und verwandte Gebiete},
year={1977},
volume={41},
pages={139-143},
}


@ARTICLE{1435648,
author={A. Host-Madsen and J. Zhang},
journal=inf,
title={{Capacity Bounds and Power Allocation for Wireless Relay Channels}},
year=2005,
month=jun,
volume={51},
pages={2020 -2040},
}


@ARTICLE{1542409,
author={K. Azarian and H. El Gamal and P. Schniter},
journal=inf,
title={{On the Achievable Diversity-Multiplexing Tradeoff in Half-Duplex Cooperative Channels}},
year=2005,
month=dec,
volume={51},
pages={4152-4172}
}


@ARTICLE{1611050,
author={T.E. Hunter and  A. Nosratinia},
journal=wc,
title={{Diversity Through Coded Cooperation}},
year=2006,
month=feb,
volume={5},
pages={283 - 289},
keywords={ BER; FER; channel coding; coded cooperation; codeword; cooperative diversity; relay channel; channel coding; diversity reception; error statistics; transmitting antennas;},
doi={10.1109/TWC.2006.1611050},
ISSN={1536-1276},}


@ARTICLE{1499041,
author={G. Kramer and M. Gastpar P. and Gupta},
journal=inf,
title={{Cooperative Strategies and Capacity Theorems for Relay Networks}},
year=2005,
month=sep,
volume={51},
pages={3037 - 3063}
}


@ARTICLE{corless1996lambertw,
  title={{On the LambertW function}},
  author={Corless, R.M. and Gonnet, G.H. and Hare, D.E.G. and Jeffrey, D.J. and Knuth, D.E.},
  journal={Advances in Computational mathematics},
  volume={5},
  number={1},
  pages={329--359},
  year={1996},
  publisher={Springer}
}




@ARTICLE{hunter2006diversity,
  title={{Diversity Through Coded Cooperation}},
  author={Hunter, T.E. and Nosratinia, A.},
  journal=wc,
  volume={5},
  number={2},
  pages={283--289},
  year={2006},
  publisher={IEEE}
}


@ARTICLE{anghel2004exact,
  title={Exact symbol error probability of a cooperative network in a Rayleigh-fading environment},
  author={Anghel, P.A. and Kaveh, M.},
  journal={Wireless Communications, IEEE Transactions on},
  volume={3},
  number={5},
  pages={1416--1421},
  year={2004},
  publisher={IEEE}
}

@ARTICLE{telatar1999capacity,
  title={{Capacity of Multi-antenna Gaussian Channels}},
  author={Emre Telatar},
  journal={European transactions on telecommunications},
  volume={10},
  number={6},
  pages={585--595},
  year={1999},
  publisher={Wiley Online Library}
}

@book{abramowitz1964handbook,
  title={Handbook of mathematical functions with formulas, graphs, and mathematical tables},
  author={Abramowitz, M. and Stegun, I.A.},
  volume={55},
  number={1972},
  year={1964},
  publisher={Dover publications}
}


@ARTICLE{1327795,
author={Hochwald, B.M. and Marzetta, T.L. and Tarokh, V.},
journal=inf,
title={{Multiple-Antenna Channel Hardening and its Implications for Rate Feedback and Scheduling}},
year=2004,
month=sep,
volume={50},
number={9},
pages={ 1893 - 1909},
}

@ARTICLE{1306612,
author={Smith, P. and Shafi, M.},
journal=com,
title={{An Approximate Capacity Distribution for MIMO Systems}},
year=2004,
month=jun,
volume={52},
number={6},
pages={ 887 - 890},
}

@inproceedings{Jain_2011,
  title={{Practical, Real-Time, Full Duplex Wireless}},
  author={Jain, M. and Choi, J.I. and Kim, T. and Bharadia, D. and Seth, S. and Srinivasan, K. and Levis, P. and Katti, S. and Sinha, P.},
  booktitle={17th annual international conference on Mobile computing and networking},
  pages={301--312},
  year={2011},
  organization={ACM}
}

@INPROCEEDINGS{6133900,
author={Zlatanov, N. and Schober, R. and Popovski, P.},
booktitle={IEEE Global Telecommunications Conference (GLOBECOM 2011)}, title={{Throughput and Diversity Gain of Buffer-Aided Relaying}},
year=2011,
month=dec,
}

@article {ETT:ETT4460100604,
author = {Telatar, Emre},
title = {{Capacity of Multi-antenna Gaussian Channels}},
journal = {European Transactions on Telecommunications},
volume = {10},
number = {6},
publisher = {Wiley Subscription Services, Inc., A Wiley Company},
pages = {585--595},
year = {1999},
}


@INPROCEEDINGS{4917634,
author={Riihonen, T. and Werner, S. and Wichman, R.},
booktitle={Wireless Communications and Networking Conference, 2009. IEEE}, title={{Comparison of Full-Duplex and Half-Duplex Modes with a Fixed Amplify-and-Forward Relay}},
year={2009},
month={april},
volume={},
number={},
pages={1 -5},}



@techreport{TD:100922,
	author={Vaneet Aggarwal and N Shankaranarayanan and Melissa Duarte and Ashutosh Sabharwal},
	institution={{IEEE ITW 2012}},
	month={September},
	title={{Full- or Half-Duplex? A Capacity Analysis with Bounded Radio Resources}},
	year=2012,
}

@INPROCEEDINGS{4533732,
author={Nikjah, R. and Beaulieu, N.C.},
booktitle={ IEEE International Conference on Communications, 2008. ICC '08.}, title={{Achievable Rates and Fairness in Rateless Coded Decode-and-Forward Half-Duplex and Full-Duplex Opportunistic Relaying}},
year={2008},
month={may},
pages={3701 -3707},
}

@INPROCEEDINGS{Duarte,
author={Duarte, M. and Sabharwal, A.},
booktitle={2010 Conference Record of the Forty Fourth Asilomar Conference on Signals, Systems and Computers (ASILOMAR)}, title={{Full-Duplex Wireless Communications Using off-the-shelf Radios: Feasibility and First Results}},
year={2010},
month={nov.},
pages={1558 -1562},
}


@INPROCEEDINGS{5507905,
author={Radunovic, Bozidar and Gunawardena, Dinan and Key, Peter and Proutiere, Alexandre and Singh, Nikhil and Balan, Vlad and Dejean, Gerald},
booktitle={2010 Fifth IEEE Workshop on Wireless Mesh Networks (WIMESH 2010)}, title={{Rethinking Indoor Wireless Mesh Design: Low Power, Low Frequency, Full-Duplex}},
year={2010},
month={june},
pages={1-6},
}

@ARTICLE{6086737,
author={Snow, T. and Fulton, C. and Chappell, W.J.},
journal={IEEE Transactions on Microwave Theory and Techniques}, title={{Transmit-Receive Duplexing Using Digital Beamforming System to Cancel Self-Interference}},
year={2011},
month={dec.},
volume={59},
number={12},
pages={3494-3503},
}


@inproceedings{1859997,
 author = {Choi, Jung Il and Jain, Mayank and Srinivasan, Kannan and Levis, Phil and Katti, Sachin},
 title = {{Achieving Single Channel, Full-Duplex Wireless Communication}},
 booktitle = {Proceedings of the sixteenth annual international conference on Mobile computing and networking},
 series = {MobiCom '10},
 year = {2010},
 pages = {1--12},
 publisher = {ACM},
}


@inproceedings{radunovic2010rethinking,
  title={{Rethinking Indoor Wireless Mesh Design: Low Power, Low Frequency, Full-Duplex}},
  author={Radunovic, B. and Gunawardena, D. and Key, P. and Proutiere, A. and Singh, N. and Balan, V. and Dejean, G.},
  booktitle={2010 Fifth IEEE Workshop on Wireless Mesh Networks (WIMESH 2010)},
  pages={1--6},
  year={2010},
}


@phdthesis{khojastepour2004distributed,
  title={{Distributed Cooperative Communications in Wireless Networks}},
  author={Khojastepour, M.A.},
  year={2004},
  school={Rice University}
}

@book{el2011network,
  title={{Network Information Theory}},
  author={El Gamal, A. and Kim, Y.H.},
  year={2011},
  publisher={Cambridge University Press}
}

@book{cover2012elements,
  title={{Elements of Information Theory}},
  author={Cover, Thomas M and Thomas, Joy A},
  year={2012},
  publisher={John Wiley \& Sons}
}

@ARTICLE{petar_two_way,
author={Huaping Liu and Popovski, P. and de Carvalho, E. and Yuping Zhao},
journal={IEEE Commun. Letters},
title={Sum-Rate Optimization in a Two-Way Relay Network with Buffering},
year={2013},
volume={17},
number={1},
pages={95-98}}


@ARTICLE{6189806,
author={Chen Dong and Lie-Liang Yang and Hanzo, L.},
journal=veh,
title={{Performance Analysis of Multihop-Diversity-Aided Multihop Links}},
year={2012},
volume={61},
month=jul,
pages={2504-2516}}


@ARTICLE{6783948,
author={Zafar, A and Shaqfeh, M. and Alouini, M.-S. and Alnuweiri, H.},
journal=com,
title={{Resource Allocation for Two Source-Destination Pairs Sharing a Single Relay with a Buffer}},
year={2014},
month=may,
volume={62},
pages={1444-1457}}


@ARTICLE{6847181,
author={Huang, J. and Swindlehurst, AL.},
journal=wc,
title={{Buffer-Aided Relaying for Two-Hop Secure Communication}},
year={2014}, }


@ARTICLE{6746659,
author={Gaojie Chen and Zhao Tian and Yu Gong and Zhi Chen and Chambers, J.A},
journal={IEEE Transactions on Information Forensics and Security},
title={{Max-Ratio Relay Selection in Secure Buffer-Aided Cooperative Wireless Networks}},
year={2014},
month=apr,
volume={9},
pages={719-729}}

@inproceedings{kramer2004models,
  title={{Models and Theory for Relay Channels with Receive Constraints}},
  author={Kramer, Gerhard},
  booktitle={Proc. 42nd Annual Allerton Conf. on Commun., Control, and Computing},
  pages={1312--1321},
  year={2004}
}

@book{deuflhard2011newton,
  title={{Newton Methods for Nonlinear Problems: Affine Invariance and Adaptive Algorithms}},
  author={Deuflhard, Peter},
  volume={35},
  year={2011},
  publisher={Springer}
}

@INPROCEEDINGS{cheap_paper,
 author={Khojastepour, Mohammad and Sabharwal, Ashutosh and Aazhang, Behnaam},
  title = {On the {C}apacity of '{C}heap' {R}elay {N}etworks},
  booktitle = {Proc. Conf. on Inform. Sciences and Systems},
  year = {2003},
}


@ARTICLE{6193208,
author={Fahs, J.J. and Abou-Faycal, IC.},
journal=inf,
title={{Using Hermite Bases in Studying Capacity-Achieving Distributions Over AWGN Channels}},
year={2012},
month=aug,
volume={58},
pages={5302-5322}}

@ARTICLE{6763001,
author={Cardone, M. and Tuninetti, D. and Knopp, R. and Salim, U.},
journal=inf,
title={{On the Gaussian Half-Duplex Relay Channel}},
year={2014},
month=may,
volume={60},
pages={2542-2562}}


@BOOK{kramer_book_1,
  title={{Cooperative Communications}},
  author={Kramer, Gerhard and Mari{\'c}, Ivana and Yates, Roy D},
  journal={Foundations and Trends{\textregistered} in Networking},
  volume={1},
  number={3},
  pages={271--425},
  year={2006},
  publisher={Now Publishers Inc.}
}

@INPROCEEDINGS{full-duplex-Khandani,
 author={A. K. Khandani},
  title = {{Two-Way (True Full-Duplex) Wireless}},
  booktitle = {Proc. 13th Canadian Workshop on Inform. Theory (CWIT)},
  year = {2014},
}




@INPROCEEDINGS{full-duplex-stanford,
 author={M. Jain and J. I. Choi and T. Kim and D.  Bharadia and S. Seth and D. Srinivasan  and P. Sinha},
  title = {{Practical, Real-Time, Full-Duplex Wireless}},
  booktitle = {Proc. 17th ACM   Annual Intern. Conf. on Mobile Computing and Networking},
  year = {2011},
}

@ARTICLE{6121995,
author={Lutz, T. and Hausl, C. and Kotter, R.},
journal=inf,
title={{Bits Through Deterministic Relay Cascades With Half-Duplex Constraint}},
year={2012},
month={Jan},
volume={58},
pages={369-381},
}


@INPROCEEDINGS{6034180,
author={Lei Zhang and Dongning Guo},
booktitle={IEEE Intern. Symp. on Inform. Theory Proc. (ISIT)},
title={{Capacity of Gaussian channels with duty cycle and power constraints}},
year={2011},
month=jul,
pages={513-517}}


@ARTICLE{6690191,
author={Lei Zhang and Hui Li and Dongning Guo},
journal=inf,
title={{Capacity of Gaussian Channels With Duty Cycle and Power Constraints}},
year={2014},
volume={60},
pages={1615-1629},
month=mar}

@ARTICLE{5730555,
author={Avestimehr, A.S. and Diggavi, S.N. and Tse, D.N.C.},
journal=inf,
title={{Wireless Network Information Flow: A Deterministic Approach}},
year={2011},
volume={57},
pages={1872-1905} ,
month=apr}

@ARTICLE{4107956,
author={Rankov, B. and Wittneben, A.},
journal=sel,
title={{Spectral Efficient Protocols for Half-Duplex Fading Relay Channels}},
year={2007},
volume={25},
pages={379-389},
month=feb}


@ARTICLE{1397921,
author={Gastpar, M. and Vetterli, M.},
journal=inf,
title={{On the Capacity of Large Gaussian Relay Networks}},
year={2005},
volume={51},
pages={765-779},
month=mar}


@ARTICLE{1214069,
author={Gupta, P. and Kumar, P.R.},
journal=inf,
title={{Towards an Information Theory of Large Networks: An Achievable Rate Region}},
year={2003},
volume={49},
pages={1877-1894},
month=aug}


@ARTICLE{4294174,
author={Sheng Yang and Belfiore, J.-C.},
journal=inf,
title={{Towards the Optimal Amplify-and-Forward Cooperative Diversity Scheme}},
year={2007},
volume={53},
pages={3114-3126},
month=sep}


@ARTICLE{4373409,
author={Yindi Jing and Jafarkhani, Hamid},
journal=inf,
title={{Using Orthogonal and Quasi-Orthogonal Designs in Wireless Relay Networks}},
year={2007},
volume={53},
pages={4106-4118},
month=nov}


@ARTICLE{1321222,
author={Nabar, R.U. and Bolcskei, H. and Kneubuhler, F.W.},
journal=sel,
title={{Fading Relay Channels: Performance Limits and Space-Time Signal Design}},
year={2004},
volume={22},
pages={1099-1109},
month=aug}


@ARTICLE{1614082,
author={El Gamal, A. and Mohseni, M. and Zahedi, S.},
journal=inf,
title={{Bounds on Capacity and Minimum Energy-Per-Bit for AWGN Relay Channels}},
year={2006},
volume={52},
pages={1545-1561},
month=apr}


@INPROCEEDINGS{zlatanov2014capacity-globecom,
  title={{On the Capacity of the Two-Hop Half-Duplex Relay Channel}},
  author={Zlatanov, Nikola and Jamali, Vahid and Schober, Robert},
  booktitle = {Proc. of the IEEE Global Telecomm. Conf. (Globecom)},
  address   = {San Diego},
  month     = dec,
  year      = 2015
}

@ARTICLE{6832464,
author={Sabharwal, A. and Schniter, P. and Dongning Guo and Bliss, D.W. and Rangarajan, S. and Wichman, R.},
journal=sel,
title={{In-Band Full-Duplex Wireless: Challenges and Opportunities}},
year={2014},
volume={32},
pages={1637-1652},
month=sep}


@ARTICLE{7024120,
author={Gang Liu and Yu, F.R. and Hong Ji and Leung, V.C.M. and Xi Li},
journal={IEEE Commun. Surveys Tutorials},
title={{In-Band Full-Duplex Relaying: A Survey, Research Issues and Challenges}},
year={2015},
volume={17},
number={2},
pages={500-524},
month={Secondquarter}}


@ARTICLE{5961159,
author={Riihonen, T. and Werner, S. and Wichman, R.},
journal=wc,
title={{Hybrid Full-Duplex/Half-Duplex Relaying with Transmit Power Adaptation}},
year={2011},
volume={10},
number={9},
pages={3074-3085},
month=sep}

@ARTICLE{Day,
author={Day, B.P. and Margetts, A.R. and Bliss, D.W. and Schniter, P.},
journal=sel,
title={{Full-Duplex MIMO Relaying: Achievable Rates Under Limited Dynamic Range}},
year={2012},
volume={30},
number={8},
pages={1541-1553},
month=sep}


@ARTICLE{Riihonen2,
author={Riihonen, T. and Werner, S. and Wichman, R.},
journal=wc,
title={{Hybrid Full-Duplex/Half-Duplex Relaying with Transmit Power Adaptation}},
year={2011},
volume={10},
number={9},
pages={3074-3085},
month=sep}

@book{hayes2009statistical,
  title={{Statistical Digital Signal Processing and Modeling}},
  author={Hayes, Monson H},
  year={2009},
  publisher={John Wiley \& Sons}
}


@ARTICLE{641562,
author={Goldsmith, A.J. and Varaiya, P.P.},
journal=inf,
title={{Capacity of Fading Channels with Channel Side Information}},
year={1997},
month=nov,
volume={43},
pages={1986-1992}
}



@ARTICLE{782125,
author={Caire, G. and Shamai, S.},
journal=inf,
title={{On the Capacity of Some Channels with Channel State Information}},
year={1999},
volume={45},
number={6},
pages={2007-2019},
month=sep}



@ARTICLE{ext_paper,
author={Nikola Zlatanov and Vahid Jamali and Robert Schober},
journal={Extended Version, Submitted to IEEE Trans. Inform. Theory},
title={{Capacity of the Two-Hop Half-Duplex Relay Channel}},
url={http://arxiv.org/abs/1411.5299},
}

@ARTICLE{720551,
author={Biglieri, Ezio and Proakis, J. and Shamai, S.},
journal=inf,
title={{Fading Channels: Information-Theoretic and Communications Aspects}},
year={1998},
volume={44},
number={6},
pages={2619-2692},
month={Oct}
}


@inproceedings{Choi:2010,
 author = {Choi, Jung Il and Jain, Mayank and Srinivasan, Kannan and Levis, Phil and Katti, Sachin},
 title = {{Achieving Single Channel, Full Duplex Wireless Communication}},
 booktitle = {MobiCom '10},
 year = {2010},
 location = {Chicago, Illinois, USA},
 pages = {1--12},
 publisher = {ACM},
 address = {New York, NY, USA},
 keywords = {wireless full-duplex},
}

@ARTICLE{6702851,
author={Everett, E. and Sahai, A. and Sabharwal, A.},
journal=wc,
title={{Passive Self-Interference Suppression for Full-Duplex Infrastructure Nodes}},
year={2014},
volume={13},
number={2},
pages={680-694},
month=feb}


@ARTICLE{5985554,
author={Riihonen, T. and Werner, S. and Wichman, R.},
journal=sip,
title={{Mitigation of Loopback Self-Interference in Full-Duplex MIMO Relays}},
year={2011},
volume={59},
number={12},
pages={5983-5993},
month=dec}

@ARTICLE{6353396,
author={Duarte, M. and Dick, C. and Sabharwal, A.},
journal=wc,
title={{Experiment-Driven Characterization of Full-Duplex Wireless Systems}},
year={2012},
volume={11},
number={12},
pages={4296-4307},
month=dec}


@ARTICLE{6177689,
author={Day, B.P. and Margetts, A.R. and Bliss, D.W. and Schniter, P.},
journal=sip,
title={{Full-Duplex Bidirectional MIMO: Achievable Rates Under Limited Dynamic Range}},
year={2012},
volume={60},
number={7},
pages={3702-3713},
month=jul}

@ARTICLE{6656015,
author={Duarte, M. and Sabharwal, A. and Aggarwal, V. and Jana, R. and Ramakrishnan, K.K. and Rice, C.W. and Shankaranarayanan, N.K.},
journal=veh,
title={{Design and Characterization of a Full-Duplex Multiantenna System for WiFi Networks}},
year={2014},
volume={63},
number={3},
pages={1160-1177},
month=mar}


@ARTICLE{6523998,
author={Sahai, A. and Patel, G. and Dick, C. and Sabharwal, A.},
journal=veh,
title={{On the Impact of Phase Noise on Active Cancelation in Wireless Full-Duplex}},
year={2013},
volume={62},
number={9},
pages={4494-4510},
month=nov}

@ARTICLE{6542771,
author={Ahmed, E. and Eltawil, A.M. and Sabharwal, A.},
journal=wc,
title={{Rate Gain Region and Design Tradeoffs for Full-Duplex Wireless Communications}},
year={2013},
volume={12},
number={7},
pages={3556-3565},
month=jul}


@ARTICLE{6736751,
author={Hong, S. and Brand, J. and Jung Choi and Jain, M. and Mehlman, J. and Katti, S. and Levis, P.},
journal=cma,
title={{Applications of Self-Interference Cancellation in 5G and Beyond}},
year={2014},
volume={52},
number={2},
pages={114-121},
month=feb}

@INPROCEEDINGS{5757799,
author={Duarte, M. and Sabharwal, A.},
booktitle={Conference Record of the Forty Fourth Asilomar Conference on Signals, Systems and Computers},
title={{Full-Duplex Wireless Communications Using Off-the-Shelf Radios: Feasibility and First Results}},
year={2010},
pages={1558-1562},
month=nov}

@ARTICLE{7105647,
author={Heino, M. and Korpi, D. and Huusari, T. and Antonio-Rodriguez, E. and Venkatasubramanian, S. and Riihonen, T. and Anttila, L. and Icheln, C. and Haneda, K. and Wichman, R. and Valkama, M.},
journal=cma,
title={{Recent Advances in Antenna Design and Interference Cancellation Algorithms for In-Band Full Duplex Relays}},
year={2015},
volume={53},
number={5},
pages={91-101},
month={May}}

@ARTICLE{6862895,
author={Young Yun Kang and Byung-Jae Kwak and Joon Ho Cho},
journal=com,
title={{An Optimal Full-Duplex AF Relay for Joint Analog and Digital Domain Self-Interference Cancellation}},
year={2014},
volume={62},
number={8},
pages={2758-2772},
month=aug}

@ARTICLE{6832471,
author={Debaillie, B. and van den Broek, D.-J. and Lavin, C. and van Liempd, B. and Klumperink, E.A.M. and Palacios, C. and Craninckx, J. and Nauta, B. and Parssinen, A.},
journal=sel,
title={{Analog/RF Solutions Enabling Compact Full-Duplex Radios}},
year={2014},
volume={32},
number={9},
pages={1662-1673},
month=sep}

@ARTICLE{6832439,
author={Korpi, D. and Anttila, L. and Syrjala, V. and Valkama, M.},
journal=sel,
title={{Widely Linear Digital Self-Interference Cancellation in Direct-Conversion Full-Duplex Transceiver}},
year={2014},
volume={32},
number={9},
pages={1674-1687},
month=sep}

@ARTICLE{6782415,
author={Korpi, D. and Riihonen, T. and Syrjala, V. and Anttila, L. and Valkama, M. and Wichman, R.},
journal=wc,
title={{Full-Duplex Transceiver System Calculations: Analysis of ADC and Linearity Challenges}},
year={2014},
volume={13},
number={7},
pages={3821-3836},
month=jul}


@ARTICLE{6832592,
author={Cirik, A.C. and Yue Rong and Yingbo Hua},
journal=sip,
title={{Achievable Rates of Full-Duplex MIMO Radios in Fast Fading Channels With Imperfect Channel Estimation}},
year={2014},
volume={62},
number={15},
pages={3874-3886},
month=aug}

@ARTICLE{7051286,
author={Ahmed, E. and Eltawil, A.M.},
journal=wc,
title={{All-Digital Self-Interference Cancellation Technique for Full-Duplex Systems}},
year={2015},
volume={14},
number={7},
pages={3519-3532},
month=jul}

@ARTICLE{7182305,
author={Tong, Z. and Haenggi, M.},
journal=com,
title={{Throughput Analysis for Full-Duplex Wireless Networks With Imperfect Self-Interference Cancellation}},
year={2015},
volume={63},
number={11},
pages={4490-4500},
month=nov}


@ARTICLE{841172,
author={M. Medard},
journal=inf,
title={{The Effect Upon Channel Capacity in Wireless Communications of Perfect and Imperfect Knowledge of the Channel}},
year={2000},
volume={46},
number={3},
pages={933-946},
month={May}}




@ARTICLE{zlatanov_fd_cap,
  title={{Capacity of the Gaussian  Two-Hop Full-Duplex Relay Channel with Self-Interference}},
  author={Nikola Zlatanov and Erik Sippel and Vahid Jamali   and   Robert
Schober},
  journal={Submitted in IEEE Trans. on Commun. Theory},
url={http://arxiv.org/abs/1510.07394},
year=2016
}


@ARTICLE{6408173,
author={N. Zlatanov and R. Schober},
journal=inf,
title={{Buffer-Aided Relaying With Adaptive Link Selection -- Fixed and Mixed Rate Transmission}},
year={2013},
volume={59},
number={5},
pages={2816-2840},
month={May},}


@ARTICLE{7523270,
author={K. T. Phan and T. Le-Ngoc},
journal={IEEE Access},
title={{Power Allocation for Buffer-Aided Full-Duplex Relaying With Imperfect Self-Interference Cancelation and Statistical Delay Constraint}},
year={2016},
volume={4},
pages={3961-3974},
month={}}

@ARTICLE{7560604,
author={N. Zlatanov and D. Hranilovic and J. S. Evans},
journal={IEEE Commun. Letters},
title={{Buffer-Aided Relaying Improves Throughput of Full-Duplex Relay Networks with Fixed-Rate Transmissions}},
year={2016},
volume={PP},
number={99},
pages={1-1},
month={}}

@ARTICLE{eh_zlatanov,
author={N. Zlatanov and R. Schober and Z. Hadzi-Velkov},
journal={Submitted to IEEE TVT},
title={{Asymptotically Optimal Power Allocation for Energy Harvesting Communication Networks}},
year={2016},
url={https://arxiv.org/abs/1308.2833}}

